Minimum-Violation Temporal Logic Planning for Heterogeneous Robots under Robot Skill Failures

In this paper, we consider teams of robots with heterogeneous skills (e.g., sensing and manipulation) tasked with collaborative missions described by Linear Temporal Logic (LTL) formulas. These LTL-encoded tasks require robots to apply their skills to specific regions and objects in a temporal and logical order. While existing temporal logic planning algorithms can synthesize correct-by-construction plans, they typically lack reactivity to unexpected failures of robot skills, which can compromise mission performance. This paper addresses this challenge by proposing a reactive LTL planning algorithm that adapts to unexpected failures during deployment. Specifically, the proposed algorithm reassigns sub-tasks to robots based on their functioning skills and locally revises team plans to accommodate these new assignments and ensure mission completion. The main novelty of the proposed algorithm is its ability to handle cases where mission completion becomes impossible due to limited functioning robots. Instead of reporting mission failure, the algorithm strategically prioritizes the most crucial sub-tasks and locally revises the team's plans, as per user-specified priorities, to minimize mission violations. We provide theoretical conditions under which the proposed framework computes the minimum-violation task reassignments and team plans. We provide numerical and hardware experiments to demonstrate the efficiency of the proposed method.

==> algorithm2e.tex <==
%  algorithm2e.sty --- style file for algorithms
%                      almost everything can be customized by users. See the document for more explanations
%% Copyright 1996-2015 Christophe Fiorio
%
% This work may be distributed and/or modified under the conditions of the LaTeX Project
% Public License, either version 1.3 of this license or (at your option) any later version.
% The latest version of this license is in http://www.latex-project.org/lppl.txt and
% version 1.3 or later is part of all distributions of LaTeX version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
% 
% The Current Maintainer of this work is M. Christophe Fiorio
%
% This work consists of the files algorithm2e.sty and algorithm2e.tex 
% and the associated example files algorithm2e_exAlgoDisjdecomp.tex,
% algorithm2e_exIR.tex, algorithm2e_ex01.tex, algorithm2e_exProg.tex,
% algorithm2e_ex02.tex, algorithm2e_exfor.tex, algorithm2e_ex03.tex,
% algorithm2e_exgeneric.tex, algorithm2e_ex04.tex,  algorithm2e_exgeneric2.tex,
% algorithm2e_ex05.tex, algorithm2e_exnlsty.tex, algorithm2e_ex06.tex,
% algorithm2e_exrepeat.tex, algorithm2e_ex07.tex, algorithm2e_exswitch.tex
%  
%  Report bugs and comments to:
%  - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
%  - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
%  subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
%
%  $Id: algorithm2e.sty,v 5.1 2015/10/18 21:37:30 cfiorio Exp $
%
%  PACKAGES REQUIRED:
%
%  - float   (in contrib/supported/float)
%  - ifthen  (in base)
%  - xspace  (in packages/tools)
%  - relsize (in contrib/misc/relsize.sty)
%
%%%%%%%%%%%%%%%  Release 5.1
%
%   Package options: 
%   ---------------
%   - oldcommands                      : to use old command names
%   - french, english, german, ngerman
%      portuguese, czech, italiano,
%      slovak, croatian, spanish       : for the name of the algorithm and some keyword code
%   - onelanguage                      : to simply switch keyword from one language to another without changing
%                                        keyword commands
%   - boxed, boxruled, ruled, tworuled, 
%     algoruled, plain                 : layout of the algorithm
%   - algo2e                           : environment is algorithm2e instead of algorithms and \listofalgorithmes
%                                        instead of \listofalgorithms
%   - slide                            : to use when making slides
%   - noline,lined,vlined              : how block are designed.
%   - shortend, longend, noend         : short or long end keyword as endif for e.g.
%   - linesnumbered                    : auto numbering of the algorithm's lines
%   - linesnumberedhidden              : to hide autonumbered lines (show number on a line with \ShowLn
%   - commentsnumbered, inoutnumbered  : to autonumber comments and inout keywords (by defaut not numbered)
%   - rightnl                          : to have line number on the right instead of on the left as default
%   - algonl                           : line numbers preceded by algo number
%   - scright, scleft                  : right or left justified side comments
%   - fillcomment, nofillcomment       : end mark of comment is flushed to the right so comments fill the line
%   - dotocloa                         : add an entry in the toc for list of algorithms (require tocbibind package)
%   - endfloat                         : add algoendfloat environment pushing algorithm so written to the end of document
%   - resetcount, noresetcount         : start value of line numbers.
%   - algopart,algochapter,algosection : algo numbering within part, chapter or section
%   - titlenumbered,titlenotnumbered   : numbering of title set by \Titleofalgo
%   - figure                           : algorithms are figures, numbered as figures, and put in the list of figures.
%   - procnumbered                     : procedure or function are numbered as algorithm
%   - nokwfunc                         : procedure or function name doens't become a command
%   - norelsize                        : don't use relsize package (useful if it breaks the compatibily)
%   - displayblockmarkers              : display begin, end keywords at start of each block
%  
%   defaults are; english,plain,resetcount,titlenotnumbered
%
%%%%%%%%%%%%%%
%
%   Short summary  
%   -------------
%  
%   algorithm is an environment for writing algorithm in LaTeX2e.
%   Almost all is customizable. You can add keywords, change style, change the layout, ...
%   It provide macros that allow you to create differents sorts of key words, therefore a set of predefined key
%   word is gived.
%
%   IT should be used as follows
%
%   \begin{algorithm}
%       ...
%       ...
%   \end{algorithm}
%
%
%   IMPORTANT : each line MUST end with \;
%
%   Note that if you define macros outside algorithm environment they
%   are avaible in all the document and particulary you can use then
%   inside all algorithms without re-define them.
%  
%   an example:
%
%   \begin{algorithm}
%     \SetAlgoLined
%     \KwIn{this text}
%     \KwOut{how to write algorithm with \LaTeX2e }
%     
%     initialization\;
%     \While{not at end of this document}{
%       read current section\;
%       \eIf{understand}{
%         go to next section\;
%         current section becomes this one\;
%         }{
%         go back to the beginning of current section\;
%         }
%       }
%     \caption{How to write algorithm}
%   \end{algorithm}
%
%
%%%%%%%%%%%%%%         predefined keywords
%
%     \KwIn{input}
%     \KwOut{output}
%     \KwData{input}
%     \KwResult{output}
%     \KwTo                                       % a simple keyword
%     \KwFrom                                     % a simple keyword
%     \KwRet{[value]}
%     \Return{[value]}
%     \Begin{block inside}
%     \eIf{condition}{Then Block}{Else block}     % in blocks
%     \If{condition}{Then block}                  % in a block
%     \uIf{condition}{Then block}                 % in a block unended
%     \lIf{condition}{Else text}                  % on the same line
%     \Else{inside Else}                          % in a block
%     \lElse{Else text}                           % on the same line        
%     \uElse{Else text}                           % in a block unended
%     \ElseIf{inside Elseif}                      % in a block
%     \lElseIf{Elseif text}                       % on the same line        
%     \uElseIf{Elseif text}                       % in a block unended
%     \Switch{Condition}{Switch block}
%     \Case{a case}{case block}                   % in a block
%     \lCase{a case}{case text}                   % on the same line
%     \Other{otherwise block}                     % in a block
%     \lOther{otherwise block}                    % on the same line
%     \For{condition}{text loop}                  % in a block
%     \lFor{condition}{text}                      % on the same line
%     \ForEach{condition}{text loop}              % in a block
%     \lForEach{condition}{text}                  % on the same line
%     \ForPar{condition}{text loop}               % in a block
%     \lForPar{condition}{text}                   % on the same line
%     \While{condition}{text loop}                % in a block
%     \lWhile{condition}{text loop}               % on the same line
%     \Repeat{End condition}{text loop}           % in a block
%     \lRepeat{condition}{text}                   % on the same line
%
%%%%%%%%%%%%%%
%
%   History: 
%
%   -  October 19 2015 - revision 5.1
%                   * CHANGE/ADD: l commands  (the ones as \lIf) can now be used with a
%                              star. If done, no end of line are done, so you can enclose
%                              l command into another one. For example, you can write:
%                              \lForEach{$i$}{\lIf*{foo}{bar}}.
%                               Note that when you use a star, side comments are not allowed.
%                   * CHANGE/ADD: Now you can have a side comment at end of macros which
%                               have a block. For example you can do : 
%                               \Begin(\tcc*[h]{side comment for begin}{text}(\tcc*[h]{side comment after end})
%                               Note: there are some side effects for some commands:
%                              \SetKwProg : macro defined thanks to \SetKwProg are allowed
%                                                   to have no end marker. In this case,
%                                                   beware to end side comment, this can
%                                                   do weird output (but no error)
%                   * CHANGE: \SetKwSwitch defines also an \uOther command which was not
%                               the case until this release.
%                   * CHANGE: \SetStartEndCondition{typo1}{typo2}{typo3} defined two end
%                               conditions (type2 and typo3) : typo3 is no more used for
%                               case condition as typo2 is used which is more consistent
%                               since there is a condition followed by a keyword as for
%                               if-then or other command that are defined using typo2.
%                   * CHANGE: keywords was not language dependant to allow to use multiple
%                               languages in the same document, but some keywords in
%                               different language were having the same keyword that lead
%                               last one declared to replace first one and so you could have some
%                               spanish keywords printed as you were in portuguese. So
%                               this behavior is changed from now:
%                               - localized keywords are defined if according language
%                                  option is defined ; 
%                               - if you want to keep old behaviour and use localized
%                                  keywords without using language option (keep old
%                                  behavior), you can use languagekw option
%                                  (e.g. frenchkw, germankw, ...). Note that you can use
%                                  multiple languagekw options at the same time, in
%                                  contrary of language option. Note also that if you use
%                                  multiple languagekw options, you can get back the same
%                                  problem as previously when keywords was not language
%                                  dependant.
%                   * ADD: new typo styles:
%                               - Arguments of functions have now their own style. By
%                                  default, FuncArgSty is the same as ArgSty. 
%                               - Name of KwProg have now their own sty (they used ArgSty
%                                  previously). By default, ProgSty is still ArgSty.
%                               As usual, \SetFuncArgSty{}, FuncArgSty{} and
%                               \SetProgSty{}, ProgSty{} are macros to set and use these
%                               typo styles.
%                   * ADD: Options to manage algorithm hangindent
%                            Until this revision, long statement acts as classical text and
%                            continue on next line starting from the same point. This makes
%                            difficult to notice that the new lines of text is not a new
%                            statement. Now, hangindent is managed and when a long
%                            statement continue on next lines, lines, except the first,
%                            are indented.
%                            Option: noalgohanging
%                               By default, long statement are indented on subsequent
%                               lines; with this option you get old behavior and lines are
%                               no more indented
%                            Option: hangingcomment 
%                               Comment that are alone on a line (not side comment) are
%                               not driven by algo hanging: subsequent lines of long
%                               comments are indented according to width of start comment
%                               marker. With this option, comment are indented like normal
%                               statement.
%                            Option: hanginginout
%                               As for comment, by default, in/out keywords and input
%                               keywords (defined by \SetKwInOut or \SetKwInput) are not
%                               indented by algorithm hangindent. They are indented
%                               according to width of input keyword. If you want that these
%                               keywords acts like normal statement, use this option.
%                            \SetAlgoHangIndent{length}
%                               This macro allows you to set your own indent length. By
%                               default, \SetAlgoHangIndent{0.5em}
%                   * ADD: Group markers. 
%                            This option is related to block markers of release 5.0. Some
%                            have ask to put also block markers for single line
%                            command. This new feature has been implemented to do this.
%                            So, you can now ask package to put begin and end keywords
%                            automatically at start and end of single line command (see
%                            example in documentation).
%                            These new group markers macros are:
%                            - \AlgoDisplayGroupMarkers and \AlgoDontDisplayGroupMarkers
%                            Note that a new option has also been added: displaygroupmarkers
%                   * ADD: \SetCustomAlgoRuledWidth{length}
%                             set a custom ruled width of ruled and algoruled options ;
%                             note that by the moment you use this macro, rules will have
%                             this fixed length: this can cause strange behavior in
%                             multicolumn mode or other layout that change the line
%                             width. 
%                   * ADD: turkish language option
%                   * FIX: a spurious whitespace which results in a spurious indent in the
%                            user's text right after the end of the algorithm environment
%                            was introduced  in release 5.0. This is fixed now thanks to
%                            Alexander Malkis.
%                   * FIX: there was a problem with margins in caption when option figure
%                            was use with caption package. This is fixed.
%                   * FIX: when changing font size in caption with, interline skip stayed
%                            unchanged and so with a small font was to large. This is fixed.
%                   * FIX: in contrary of that is written in the documentation, ':' what
%                            not in KwSty typo for KwIn and KwOut command. This is fixed. 
%                   * FIX: strange behaviour with label and lines numbered: @currentlabel
%                            was updated according to algo line number not in all
%                            situation. For e.g, with hyperref package, always updated ;
%                            with \nlset also updated, but with \nl or linesnumbered
%                            option, not updated. This "feature" causes different output
%                            with \label command according to options used which is not
%                            that one want. This is solved now, and @currentlabel is
%                            always updated so \label command works always is the same way.
%                   * FIX: some czech keywords
%                   * FIX: some spanish keywords
%                   * FIX: some croatian keywords
%                   * FIX: krantz class changes definition of chapter and get one more
%                            option that classical classes as book.cls or report.cls and
%                            broke fix for hyperref on chapter definition. This is now
%                            fixed and algorithm detects use of krantz class and use then
%                            a definition of chapter working with krantz class.
%                   * FIX: an issue with internal macro which causes ([Q]) use as argument
%                            of some environment to be misprinted (thanks to Martin Schr?der).
%                   * FIX: mispelled name of hyperrefcounter inside internal macro.
%
%   - January 06 2013 - revision 5.0
%                     * CHANGE: SetKwSwitch takes now 9 args: 9th arg is the same as
%                                previous 8th arg ('end of switch' keyword). New 8th arg is
%                                'end of case' keyword. This is due to change of release
%                                3.2 which introduce end after case block... as I never
%                                test with longend option, I never see that the 'end
%                                switch' used for case was not good.
%                     * CHANGE: when no end keyword is defined in a block macro, then
%                                algorithm2e does no more try to print it. So even with lined or noline
%                                option, no empty line is printed (before: a blank end was
%                                printed, so a blank line appeared)
%                     * Internal Change: add some internal function to improve readibility
%                                        (thanks to Philip K. F. H\?lzenspies)
%                     * ADD: Block markers. 
%                            You can now ask package to put begin and end keywords automatically at begin
%                            and end of blocks, it means each group of commands shifted and enclosed in
%                            braces.
%                            This is tricky to use but, combined with \SetStartEndCondition and
%                            redefinition of keywords, you should be abble to simulate any syntax. See
%                            examples in documentation where a generic example is derived in pseudo-code,
%                            python and C by keeping code and changing only style using block markers
%                            macros, \SetStartEndCondition and some redefinition of keywords.
%                            These new block markers macros are:
%                            - \AlgoDisplayBlockMarkers and \AlgoDontDisplayBlockMarkers
%                            - \SetAlgoBlockMarkers{begin marker}{end marker}
%                            - \BlockMarkersSty{text} and \SetBlockMarkersSty
%                            Note that a new option has also been added: displayblockmarkers
%                     * ADD: \leIf macro automatically defined by \SetKwIF: allow to define
%                            an if-then-else on a single line.
%                     * ADD: new macro \SetStartEndCondition{typo1}{typo2}{typo3} which
%                            sets typo around condition in For, If, Switch, Case and
%                            Repeat macros. First two are used around For, If, Swith
%                            conditions, First and third are used for Case and Repeat
%                            condition where condition ends the line. Default definition
%                            is \SetStartEndCondition{ }{ }{}. 
%                            A common alternative is \SetStartEndCondition{ (}{) }{)}
%                            Can also be used to remove space around condition, for
%                            example if you want python style commands:
%                            \SetStartEndCondition{ }{}{} and \SetKwFor{For}{for}{:}{}
%                     * ADD: new environment algomathdisplay which allow display math (like inside \[ \] or $$ $$) 
%                            handling end line and line number
%                     * ADD: new command \SetKwProg{Env}{Title}{is}{end} which defines a macro
%                            \Env{args}{text}. Env is a block with 'Title' (in \CapSty) at the beginning
%                            followed by args followed by 'is' then 'text' is put below inside a block ended
%                            by 'end'. If no 'end' is specified, nothing is written (no
%                            blank line is inserted). Useful to typeset function or prog for example:
%                            \SetKwProg{Fn}{Function}{ is}{end} makes \Fn{afunc(i: int) : int}{return 0\;}                    
%                            writes: 
%                            Function afunc(i: int) : int is
%                            | return 0;
%                            end
%                            or \SetKwProg{Def}{def}{:}{} makes \Def{afunc(i: int)}{return 0\;} writes:
%                            def afunc(i: int):
%                            | return 0
%                            Tip: combine it with \SetKwFunction to write recursive function algorithm. With
%                            example above, you could define \SetKwFunction{\Afunc}{afunc} and then write:
%                            \Def{\Afunc{i:int}{\eIf{i>0}{\KwRet \Afunc{i-1}}{\KwRet 0\;}} that writes:
%                            def afunc(i: int):
%                            | if(i>0):
%                            |     return afunc(i-1)
%                            | else:
%                            |     return 0
%                            with appropriate typo.
%                     * ADD: option croatian: croatian keywords (thanks to Ivan Gavran)
%                     * ADD: option ngerman: same as german option but so can be used with global option ngerman
%                            of babel
%                     * ADD: option spanish: Spanish support (thanks to Mario Abarca)
%                     * ADD: unterminated block: useful to add part separator that doesn't necessary need an end
%                            keyword.  
%                            Designed on the pattern of unterminated if (see \uIf macro) allowing to
%                            add a block that is not terminated by a keyword. Such block are defined in the same
%                            time as a block is defined by adding a macro beginning with u. So, for example,
%                            predefined \SetKwBlock{Begin}{begin}{end} defines now two commands:
%                            - \Begin{} as previously which print a begin - end block
%                            - \uBegin{} that defines a begin only block
%                     * FIX: problem when numbering line inside until condition of
%                            \SetKwRepeat macro: line number was not correctly aligned.
%                     * FIX: dotocloa option which was broken
%                     * FIX: uIf and uCase didn't have same behavior when used with
%                            noline, vlined or lined option. This is fixed. Side effect: no empty
%                            line after an uIf or uCase when used with options lined or vlined
%                     * FIX: a bug with Repeat Until command when use with side comment on Until
%                     * FIX: a bug with side text -- text put into () -- of command macro (SetKwIf and so on)
%                            which was always setting a ';' even after a \DontPrintSemicolon
%                     * FIX: a bug with hyperref and chapter definition (thanks to Hubert Meier)
%                     * FIX: bugs with l macro and side comment
%                     * FIX: revision number
%                     * FIX: fix non ascii character (utf8 not yet recognized by all latex engine)
%                     * FIX: fnum@algocf had an useless parameter which sometimes broke expansion and output an error
%                     * FIX: works now with multicol package
%
%   - december 14 2009 - revision 4.1
%                     * ADD: new command \SetKwHangingKw{Name}{text} (hanging indent with keyword): This creates a
%                            hanging indent much like \texttt{SetKwInput}, except that it removes the trailing `:'
%                            and does not reset numbering (thanks to Nathan Tallent)
%
%   - november 17 2009  - revision 4.00 -
%
%                      * CHANGE: IMPORTANT: some commands have been renamed to have consistent naming (CamlCase
%                                syntax) and old commands are no more available. If you doesn't want to change
%                                your mind or use old latex files, you can use oldcommands option to enable old
%                                commands back.
%                                text. Here are these commands:
%                                - \SetNoLine becomes \SetAlgoNoLine
%                                - \SetVline  becomes \SetAlgoVlined
%                                - \Setvlineskip  becomes \SetVlineSkip
%                                - \SetLine   becomes \SetAlgoLined
%                                - \dontprintsemicolon becomes \DontPrintSemicolon
%                                - \printsemicolon becomes \PrintSemicolon
%                                - \incmargin becomes \IncMargin
%                                - \decmargin becomes \DecMargin
%                                - \setnlskip becomes \SetNlSkip
%                                - \Setnlskip becomes \SetNlSkip
%                                - \setalcapskip becomes \SetAlCapSkip
%                                - \setalcaphskip becomes \SetAlCapHSkip
%                                - \nlSty becomes \NlSty
%                                - \Setnlsty becomes \SetNlSty
%                                - \linesnumbered becomes \LinesNumbered
%                                - \linesnotnumbered becomes \LinesNotNumbered
%                                - \linesnumberedhidden becomes \LinesNumberedHidden
%                                - \showln becomes \ShowLn
%                                - \showlnlabel becomes \ShowLnLabel
%                                - \nocaptionofalgo becomes \NoCaptionOfAlgo
%                                - \restorecaptionofalgo becomes \RestoreCaptionOfAlgo
%                                - \restylealgo becomes \RestyleAlgo
%                                - gIf macros and so on do no more exist
%                      * NEW: - Compatibily with other packages improven by changing name of internal
%                               macros. Algorithm2e can now be used with arabtex for example, if this last is
%                               loaded after algorithm2e package.
%                      * ADD: - OPTION endfloat: endfloat packages doesn't allow float environment inside other
%                               environment. So using it with figure option of algorithm2e makes error. This
%                               option enables a new environment algoendfloat to be used instead of algorithm
%                               environment that put algorithm at the end. algoendfloat environment make
%                               algorithm acting as endfloat figures. This option requires endfloat packages.
%                      * ADD: - OPTION norelsize: starting from this release (v4.00), algorithm2e package uses
%                               relsize package in order to get relative size for lines numbers; but it seems
%                               that some rare classes (such as inform1.cls) are not compatible with relsize; to
%                               have algorithm2e working, this option makes algorithm2e not to load relsize
%                               package and go back to previous definition by using \scriptsize font for lines
%                               numbers.
%                      * ADD: - OPTION onelanguage: allow, if using standard keywords listed below, to switch
%                               from one language to another without changing keywords by using appropriate
%                               language option:
%                               . KwIn, KwOut, KwData, KwResult
%                               . KwTo KwFrom
%                               . KwRet, Return
%                               . Begin
%                               . Repeat
%                               . If, ElseIf, Else
%                               . Switch, Case, Other
%                               . For, ForPar, ForEach, ForAll, While
%                               .
%                      * ADD: - OPTION rightnl: put lines numbers to the right of the algorithm instead of left.
%                      * ADD:   new commands \setRightLinesNumbers and \setLeftLinesNumbers which sets the lines
%                               numbers to the right or to the left of the algorithm.
%                      * ADD: - new kind of keywords: KwArray used to define arrays:
%                               \SetKwArray{Kw}{array} defines an array keywords Kw called array and printed in
%                               DataSty style when call with \Kw. It can be used with one argument which
%                               denotes the element index: \Kw{n} prints array[n] with array in DataSty and n in
%                               ArgSty.
%                      * ADD/FIX: rules of ruled, algoruled, tworuled styles used rules of different sizes! This
%                                 is now fixed. Moreover size of the rules is now controlled by a length and so
%                                 can be customized by the user.
%                                 \algoheightrule is the height of the rules and can be changed via \setlength
%                                 \algoheightruledefault is the default height of he rules (0.8pt)
%                                 \algotitleheightrule is the height of the rule that comes just after the
%                                 caption in ruled and algoruled style; it can be changed via \setlength
%                                 \algotitleheightruledefault is the default height of this rules (0.8pt)
%                                 Thanks to Philippe Dumas who reports the bug and make the suggestion.
%                      * ADD: - \SetAlgoCaptionSeparator which sets the separator between Algorithm 1 and the
%                               title. By default it's ':' and caption looks like "Algorithm 2: title" but now
%                               you can change it by using for example \SetAlgoCaptionSeparator{.} which will
%                               give "Algorithm 3. title"
%                      * ADD: - \SetAlgoLongEnd and \SetAlgoShortEnd and \SetAlgoNoEnd commands which act as
%                               corresponding package options
%                      * ADD: - OPTIONS italiano and slovak as new language (thanks to Roberto Posenato and
%                               Miroslav Binas) 
%                      * CHANGE: - Fnt and Sty macro to have consistent use and naming (see below)
%                      * ADD: - \AlCapSty, \AlCapNameSty, \AlCapFnt, \AlCapNameFnt, \ProcSty, \ProcFnt,
%                               \ProcNameSty, \ProcNameFnt, \ProcArgSty, ProcArgFnt and corresponding "set macro" 
%                               \SetAlCapSty, \SetAlCapNameSty, \SetAlCapFnt, \SetAlCapNameFnt, \SetProcSty,
%                               \SetProcFnt, \SetProcNameSty, \SetProcNameFnt, \SetProcArgSty, \SetProcArgFnt which
%                               control the way caption is printed. Sty macro use command taking one parameter as
%                               argument, Fnt macros use directly command. In Fact caption is printed as follow:
%                               \AlCapSty{\AlCapFnt Algorithm 1:}\AlCapNameSty{\AlCapNameFnt my algorithm}
%                               By default, \AlCapSty is textbf and \AlCapFnt is nothing. \AlCapNameSty keep text 
%                               as it is, and \AlCapNameFnt do nothing also.
%                               You can redefine \AlCapFnt and \AlCapNameFnt by giving macro to \Set commands. For
%                               example, you can do \SetAlCapFnt{\large} to see Algorithm printed in \large font.
%                               You can redefine \AlCapSty, \AlCapFnt, \AlCapNameSty and \AlCapNameFnt with the
%                               corresponding \Set command. For the Sty commands, you have to give in parameter
%                               name of a macro (whithout \)  which takes one argument. For example,
%                               \SetAlCapFnt{textbf} defines the default behaviour. If you want to do more
%                               complicated thing, you should define your own macro and give it to \SetAlCapFnt or
%                               \SetAlCapNameFnt. Here are two examples:
%                               - \newcommand{\mycapsty}[1]{\tiny #1}\SetAlCapNameSty{mycapsty}
%                               - \newcommand{\mycapsty}[1]{\textsl{\small #1}}\SetAlCapNameSty{mycapsty}
%                               Or you can combine the two, for the last example you can also do:
%                               \SetAlCapNameSty{textsl}\SetAlCapNameFnt{\small}
%                               Thanks to Jan Stilhammer who gives me the idea of \AlCapNameFnt.
%                      * CHANGE \AlTitleFnt to match definition of all other Fnt macros and add a \AlTitleSty 
%                               macro (see below) . Now you set \AlTitleFnt by calling \SetAlTitleFnt with 
%                               directly a macro without parameter in argument:
%                               Example: \SetAlTitleFnt{\small} to set title in small font.
%                      * ADD: - \AlTitleSty and \SetAlTitleSty commands to set a style for title. These commands
%                               are defined from a macro taking the text in argument, as \textbf for example. 
%                               To set the TitleSty you have to give name of the macro (without the '\') 
%                               to \SetAlTitleSty. For example \SetAlTitleSty{textbf} to set \textbf style.
%                      * ADD: - new command \SetAlgorithmName{algorithmname}{list of algorithms name} which
%                               redefines name of the algorithms and the sentence list of algorithms. Second
%                               argument is the name that \autoref, from hyperref package, will use. Example:
%                               \SetAlgorithmName{Protocol}{List of protocols} if you prefer protocol than
%                               algorithm.
%                      * ADD: - new \SetAlgoRefName{QXY} which change the default ref (number of the algorithm) by
%                               the name given in parameter (QXY in the example). 
%                      * ADD: - new command \SetAlgoRefRelativeSize{-2} which sets the output size of refs, defined
%                               by \SetAlgoRefName, used in list of algorithms.
%                      * ADD: - two dimensions to control the layout of caption in ruled, algoruled and boxruled
%                               algorithms:
%                               - interspacetitleruled (2pt by defaut) which controls the vertical space between
%                                 rules and title in ruled and algoruled algorithms.
%                               - interspaceboxruled (2\lineskip by default) which controls the vertical space
%                                 between rules and title in boxruled algorithms.
%                               These two dimensions can be changed by using \setlength command.
%                      * ADD: - With the fix (see below) of procedure and function environments, a new feature has
%                               been added: the name of the procedure or function set in caption is automatically
%                               defined as a KwFunction and so can be used as a macro. For example, if inside a
%                               procedure environment you set \caption{myproc()}, you can use \myproc macro in you
%                               main text. Beware that the macro is only defined after the \caption!
%                      * ADD: - OPTION nokwfunc to unable the new feature described above in function and
%                               procedure environment. Useful if you use name of procedure or function that cannot
%                               be a command name as a math display for example.
%                      * ADD: - \SetAlgoNlRelativeSize{number} command which sets the relative size of line
%                               numbers. By default, line numbers are two size smaller than algorithm text. Use
%                               this macro to change this behavior. For example, \SetAlgoNlRelativeSize{0} sets it
%                               to the same size, \SetAlgoNlRelativeSize{-1} to one size smaller and
%                               \SetAlgoNlRelativeSize{1} to one size bigger
%                      * ADD: - \SetAlgoProcName{aname} command which sets the name of Procedure printed by
%                               procedure environment (the environment prints Procedure by default). Second
%                               argument is the name that \autoref, from hyperref package, will use.
%                      * ADD: - \SetAlgoFuncName{aname} command which sets the name of Function printed by
%                               procedure environment (the environment prints Function by default). Second
%                               argument is the name that \autoref, from hyperref package, will use. 
%                      * ADD: - \SetAlgoCaptionLayout{style} command which sets style of the caption; style must
%                               be the name of a macro taking one argument (the text of the caption). Examples
%                               below show how to use it:
%                               . \SetAlgoCaptionLayout{centerline} to have centered caption
%                               . \SetAlgoCaptionLayout{textbf} to have bold caption
%                               If you want to apply two styles in the same time, such as centered bold, you have
%                               to define you own macro and then use \SetAlgoCaptionLayout with its name.
%                      * ADD: - OPTION procnumbered: which makes the procedure and function to be numbered as
%                               algorithm
%                      * ADD: - OPTIONS tworuled and boxruled
%                               these are two new layouts: tworuled acts like ruled but doesn't put a line after
%                               caption ; boxruled surround algorithm by a box, puts caption above and add a line
%                               after caption.
%                      * REMOVE: - SetKwInParam has been deleted since not useful itself because of different
%                                macros which can do the same in a better and a more consistent way as
%                                SetKwFunction or SetKw.
%                      * FIX: - line number is now correctly vertically aligned with math display.
%                      * FIX: - references with hyperref. No more same identifier or missing name error. BUT now
%                               you must NOT use naturalnames option of hyperref packages if you do PdfLaTeX
%                      * FIX: - autoref with hyperref package (thanks to J?rg Sommer who notices the problem).
%                      * FIX: - titlenumbered was not working! fixed.
%                      * FIX: - Else(){} acted like uElse. Corrected.
%                      * FIX: - noend management: when a block was inside another and end of block was following
%                               each other, a blank line was added: it's now corrected.
%                      * FIX: - Function and Procedure environment was no more working as defined originally: the
%                               label was no more name of the procedure, it acts always as if procumbered option
%                               has been used.
%                      * FIX: - line numbers had a fixed size which can be bigger than algorithm text accordingly
%                               to \AlFnt set (see also new command \SetAlgoNlRelativeSize above)
%                      * FIX: - semicolon in comments when dontprintsemicolon is used.
%                      * FIX: - listofalgorithms adds a vertical space before first algo of a chapter as for
%                               listoffigures or listoftables
%                      * FIX: - listofalgorithms with twocolumns mode and some classes which don't allow onecolumn
%                               and so don't define \if@restonecol as prescribed in LaTeX (sig-alternate for
%                               example)
%                      * FIX: - algorithm2e now works with elsart cls and some more classes.
%                      * FIX: - blocks defined by SetKwBlock act now as other blocks (if for instance) and don't
%                               write end in vlined mode, instead they print a small horizontal line as required
%                               by the option.
%                      * FIX: - underfull hbox warning at each end of algorithm environment removed.
%
%                      * INTERNAL CHANGE: - short end keyword are deduce from long end keyword by keeping the
%                                           first one. Allows to avoid double definition.
%                      * INTERNAL CHANGE: - procedure, function and algorithm are now resolved by the same
%                               environment to avoid code duplication. 
%
%   - October  04 2005  - revision 3.9 -
%                      * ADD: - \setalcaphskip command which sets the horizontal skip before Algorithm: in caption
%                               when used in ruled algorithm.
%                      * ADD: - \SetAlgoInsideSkip command which allows to add an extra vertical space before and
%                               after the core of the algorithm (ie: \SetAlgoInsideSkip{bigskip}) 
%                      * CHANGE: - caption, when used with figure option, is no more controlled by algorithm2e
%                                  package and so follows the exact behaviour of figures. The drawback is that you
%                                  cannot change the typo with AlTitleFnt or CapFnt. The avantage is that if you
%                                  use caption package, it works.
%                      * FIX: - problem with numbering line and pdflatex
%                      * FIX: - error when algorithm2e package was used with beamer and listings together
%   - February 12 2005  - revision 3.8 -
%                      * FIX: - extra line with noend option.
%   - February 10 2005  - revision 3.7 -
%                      * ADD: - sidecomment: different macros allowing to put text right after code on the same
%                               line. They are defined in the same time comment macros are defined with a star
%                               after the macro name. By default comments are right justified but this can be
%                               change with appropriate option in the macro. Ex:
%                               . default: \tcc*{side comment}
%                               . same as previous: \tcc*[r]{side comment}
%                               . left justify: \tcc*[l]{side comment}
%                               . here: \tcc*[h]{side comment} don't put the end of line mark before
%                                       comment (; by default) and don't end the line.
%                               . flushed: \tcc*[f]{side comment} same as the precedent but right
%                                 justified
%                      * ADD: - OPTION scright (default): right justified side comments (side comments
%                               are flushed to the righr)
%                      * ADD: - OPTION scleft: left justified side comments (side comments are put right after the
%                               code line)
%                      * ADD: - \SetSideCommentLeft acts as scleft option
%                      * ADD: - \SetSideCommentRight acts as scright option
%                      * ADD: - block like macro side text: all macro defining a block allows now to put text right
%                               after key words by putting text into (). Done to be used with sidecomment macros,
%                               but all text can be used. 
%                               Ex: \eIf(\tcc*[f]{then comment}){test}{then text}(else side text){else text}
%                      * ADD: - OPTION fillcomment (default): end mark of comment is flushed to the right so
%                               comments fill all the width of text.
%                      * ADD: - OPTION nofillcomment: end mark of comment is put right after the comment.
%                      * ADD: - \SetNoFillComment acts as nofillcomment option.
%                      * ADD: - \SetFillComment acts as fillcomment option.
%                      * ADD: - OPTION dotocloa: which adds an entry in the toc for the list of algorithms. This
%                               option load package tocbibind if not already done and so list of figures and list
%                               of tables are also added in the toc. If you want to control which ones of the lists
%                               will be added in the toc, please load package tocbibind before package algorithm
%                               and give it the options you want.
%                      * FIX: - vertical spacing for uif macro with noend option
%                      * FIX: - all the compatibility problems between caption and other packages
%                      * FIX: - typographical differences between list of algorithms and other lists  when in
%                               report or book 
%
%   - January 24 2005  - revision 3.6 -
%                      * FIX: - vertical spacing and space characters at the beginning or end of comments.
%                               line numbers of comments not in the NlSty.
%                               Thanks to Arnaud Giersch for his comments and suggestions.
%                      * FIX: - Set*Sty macro: the styles defined was not protected and was modified by surrounding
%                               context. For example KwTo in a \For{}{} was in bold AND italic instead of just in
%                               bold.
%                      * FIX: - line number misplacement after \Indp
%
%   - January 21 2005  - revision 3.5 -
%                      * ADD: - hidden numbering of the lines. Lines are auto-numbered but numbers are shown only
%                               on lines you specify:
%                               * linesnumberedhidden option or \LinesNumberedHidden macro activate this
%                                 functionnality.
%                               * \ShowLn and \ShowLnLabel{lab} macros make the number visible on the
%                               line. \ShowLnLabel{lab} allows to set a label for this line. 
%                               Thanks to Samson de Jager who makes this suggestion and provides the macros.
%                      * ADD: - \AlCapFnt and \SetAlCapFnt which allow to have a different font for
%                               caption. Works like \AlFnt and \SetAlFnt and by default is the same.
%                      * ADD: - \AlCapSkip skip length. This vertical space is added before caption in plain ou
%                               boxed mode. It allows to change distance between text and caption.
%                      * FIX: - caption compatible with IEEEtran class. 
%                      * FIX: - some vertical spacing error with \uIf macros (Thanks to Arnaud Giersch)
%                      * FIX: - Procedure and Function: lines are also numbered like algorithms
%                      * FIX: - CommentSty was not used for Comments
%
%   - January 10 2005  - revision 3.4 -
%                      * FIX: - caption compatible with new release of Beamer class. 
%
%   - June 16 2004     - revision 3.3 - 
%                      * FIX: - Hyperlink references of Hyperref package works now if compiled with pdflatex 
%                               and [naturalnames] option of hyperref package is used.
%                      * FIX: - algorithm[H] had problem in an list environment - corrected
%                      * FIX: - interline was not so regular in nested blocks - corrected
%                      * ADD  - \SetVlineSkip macro which sets the vertical skip after the little horizontal 
%                               rule which closes a block in Vlined mode. By default 0.8ex
%
%   - June 11 2004     - revision 3.2 - AUTO NUMBERING LINES !!!
%                      * ADD: auto numbering of the lines (the so asked and so long awaiting feature)
%                             this feature is managed by 3 options and 3 commands:
%                             - linesnumbered option: lines of the algo are numbered except for comments and
%                               input/output (KwInput and KwInOut)
%                             - commentsnumbered option: makes comments be numbered
%                             - inoutnumbered option: makes data input/output be numbered
%                             - \nllabel{lab} labels the line so you can cite with \ref{lab}
%                             - \LinesNumbered make the following algorithms having auto-numbered lines
%                             - \linesnotnumbered make the following algorithms having no auto-numbered lines
%                      * Change: algo2e option renames listofalgorithms in listofalgorithmes
%                      * FIX: new solution for compatibility with color package, more robust and not tricky.
%                             Many thanks to David Carlisle for his advices
%
%   - June 09 2004     - revision 3.1 -
%                      * Change: \SetKwSwitch command defines an additionnal macro \uCase and \Case prints end
%                      * Change: now macros SetKw* do a renewcommand if the keyword is already defined. So you can
%                                redefine default definition at your own convenience or change your definition
%                                without introducing a new macro and changing your text.
%                      * ADD: new macro \SetKwIF which do \SetKwIf and
%                             \SetKwIfElseIf.The following default definition has been added:
%                             \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
%                             and so you get the macros;
%                             \If \eIf \lIf \uIf \ElseIf \uElseIf \lElseIf \Else \uElse \lElse
%                      * ADD: new macro \SetAlgoSkip which allow to fix the vertical skip before and after the
%                             algorithms. Default is smallskip, do \SetAlgoSkip{} if you don't want an extra space
%                             or \SetAlgoSkip{medskip} or \SetAlgoSkip{bigskip} if you want bigger space.
%                      * ADD: macro \SetKwIf defines in addition a new macro \uElse  (depending on wat name you
%                             have given in #2 arg).
%                      * ADD: macro \SetKwIfElseIf defines in addition a new macro \uElse and \ugElseIf (depending
%                             on what name you have given in #2 and #3 arg).
%                      * Change: baseline of algorithm is now top, so two algorithms can be put side by side.
%                      * FIX: Compatibility with color package solved. The problem was due to a redefinition of
%                             standard macros by color package. This solves compatibility problem with other
%                             packages as pstcol or colortbl. (notified by Dirk Fressmann, Antti Tarvainen and Koby
%                             Crammer)
%                      * Fix: extra little shift to the right with boxed style algorithm removed (notified by
%                             P. Tanovski)
%                      * Fix: algoln option was buggy (notified bye Jiaying Shen)
%                      * Fix: german and portuges option didn't work due to bad typo (notified by Martin Sievers,
%                             Thorsten Vitt and Jeronimo Pellegrini)
%                      
%   - February 13 2004 - revision 3.0 -
%                      * Major revision which makes the package independent from float.sty, so now
%                        - algorithm* works better, in particular can be used in multicols environments
%                        - (known bug corrected)
%                          [H] works now for all sort of environment but is handled differently for classic
%                          environment and star environment (algorithm, figure, procedure and function). For star
%                          environment, H acts like for classical figure environment, so it doesn't stay here
%                          absolutely.
%                        - (known bug corrected)
%                          you can use now floatflt package with algorithm package and even with figure
%                          option. Beware that if you want to put an algorithm inside a floatingfigure, it cannot
%                          be floating, so [H] is required and then figure option should not be used, since
%                          standard figure[H] are still floating with LaTeX.
%                      * boxruled: a new style added. Possible now since no style no more defined by the float
%                        package.
%                      * nocaptionofalgo: dosen't print Algorithm #: in the caption for algorithm in ruled or
%                        algoruled style.
%                        note: this is just documentation of a macro which was already in the package.
%   - December 14 2003 - revision 2.52 -
%                      * output message shorter
%                      * French keyword macro \PourTous was missing for longend option, it has been added.
%                      * TitleofAlgo prints Function or Procedure in corresponding environments.
%
%   - October 27 2003  - revision 2.51 - Revision submitted to CTAN archive
%                      * correction of a minor which make caption in procedure
%                        and function to be blanck with pdfscreen package
%                        (thanks to Joel Gossens for the notification)
%                      * add two internal definition to avoid some errors when
%                        used with Hyperref package (Hyperref package need to
%                        define new counter macro from existing ones, and
%                        don't do it for algorithm2e package, so we do it)
%
%   - October 17 2003  - revision 2.50 - first revision for CTAN archive
%                      * add \AlFnt and \SetAlFnt{font} macros: \AlFnt is used at the beginning of the caption and
%                        the body of algorithm in order to define the fonts used for typesetting algorithms. You
%                        can use it elsewhere you want to typeset text as algorithm. For example you can do
%                        \SetAlFnt{\small\sf} to have algorithms typeset in small sf font. Default is nothing so
%                        algorithm is typeset as the text of the document.
%                      * add \AlTitleFnt{text} and \SetAlTitleFnt{font} macros: The {Algorithm: } in the caption is
%                        typeset with \AlTitleFnt{Algorithm:}. You can use it to have text typeset as {Algorithm:}
%                        of captions. Default is textbf.  Default can be redefined by \SetAlTitleFnt{font}, for
%                        example you can do \SetAlTitleFnt{emph}
%                      * add CommentSty typo for text comment.  
%                      * add some compatibility with hyperref package (still an error on multiply defined refs but
%                        pdf correctly generated)
%                      * flush text to left in order to have correct indentation even with class as amsart which
%                        center all figures
%                      * add german, portuguese and czech options for title of algorithms and typo.
%                      * add portuguese translation of predefined keywords * add czech translation of some
%                        predefined keywords
%
%   - December 23 2002 - revision 2.40
%                      * add some French keyword missing
%                      * add function* and procedure* environment like algorithme* environment: print in one column
%                        even if twocolumn option is specified for the document.
%                      * add a new macro \SetKwComment to define macro which writes comments in the text. First
%                        argument is the name of the macro, second is the text put before the comment, third is the
%                        text put at the end of the comment.Default are \tcc and \tcp
%                      * add new options to change the way algo are numbered:
%                        [algopart] algo are numbered within part (counter must exist)
%                        [algochapter] algo are numbered within chapter
%                        [algosection] algo are numbered within section
%
%   - March 27 2002   - revision 2.39
%                      * Gilles Geeraerts: added the \SetKwIfElseIf to manage
%                        if (c)
%                             i;
%                        else if (c)
%                             i;
%                        ...
%                        else
%                             i;
%                        end
%                      * Also added \gIf \gElseIf \gElse.
%
%   - January 02 2001 - revision 2.38
%                      * bugs related to the caption in procedure and function
%                        environment are corrected.
%                      * bug related to option noend (extra vertical space added
%                        after block command as If or For) is corrected.
%                      * czech option language added (thanks to Libor Bus: l.bus@sh.cvut.cz).
%  
%   - October 16 2000 - revision 2.37
%                      * option algo2e added: change the name of environment
%                        algorithm into algorithm2e. So allow to use the package
%                        with some journal style which already define an algorithm
%                        environment.
%  
%   - September 13 2000 - revision 2.36
%                      * option slide added: require package color
%                      * Hack for slide class in order to have correct
%                        margins
%  
%   - November 25 1999 - revision 2.35
%                      * revision number match RCS number
%                      * Thanks to David A. Bader, a new option is added:
%                        noend: no end keywords are printed.
%  
%   - November 19 1999 - revision 2.32
%                      * minor bug on longend option corrected.
%  
%   - August 26 1999 - revision 2.31
%                      * add an option: figure
%                        this option makes algorithms be figure and so are numbered
%                        as figures, have Figure as caption and are put in 
%                        the \listoffigures
%  
%   - January 21 1999 - revision 2.3 beta
%                    add 2 new environments: procedure and function.
%                    These environments works like algorithm environment but:
%                    - the ruled (or algoruled) style is imperative.
%                    - the caption now writes Procedure name....
%                    - the syntax of the \caption command is restricted as
%                      follow: you MUST put a name followed by 2 braces like
%                      this ``()''. You can put arguments inside the braces and
%                      text after. If no argument is given, the braces will be
%                      removed in the title. 
%                    - label now puts the name (the text before the braces in the
%                      caption) of the procedure or function as reference (not
%                      the number like a classic algorithm environment).
%                    There are also two new styles: ProcNameSty and
%                    ProcArgSty. These style are by default the same as FuncSty
%                    and ArgSty but are used in the caption of a procedure or a
%                    function.
%                    
%   - November 28 1996 - revision 2.22
%                    add a new macro \SetKwInParam{arg1}{arg2}{arg3}:
%                    it defines a macro \arg1{name}{arg} which prints name in keyword
%                    style followed byt arg surrounded by arg2 and arg3. The main
%                    application is to a function working as \SetKwInput to be used
%                    in the head of the algorithm. For example
%                    \SetKwInParam{Func}{(}{)} allows
%                    \Func{functionname}{list of arguments} which prints:
%                    \KwSty{functioname(}list of arguments\KwSty{)}
%       
%
%   - November 27 1996 - revision 2.21:
%                    minor bug in length of InOut boxes fixed.
%                    add algorithm* environment.
%
%   - July 12 1996 - revision 2.2: \SetArg and \SetKwArg macros removed.
%                        
%                    \SetArg has been removed since it never has been
%                    documented.
%                    \SetKwArg has been removed since \SetKw can now
%                    take an argument in order to be consistent with
%                    \SetKwData and \SetKwFunction macros.
%
%   - July 04 1996 - revision 2.1: still more LaTeX2e! Minor compatibility break
%
%                    Macros use now \newcommand instead of \def, use of \setlength, 
%                    \newsavebox, ... and other LaTeX2e specific stuff.
%                    The compatibility break:
%                    - \SetData becomes \SetKwData to be more consistent. So the old 
%                      \SetKwData becomes \SetKwInput
%                    - old macros \titleofalgo, \Freetitleofalgo and \freetitleofalgo
%                      from LaTeX209 version which did print a warning message and call 
%                      \Titleofalgo in version 2.0 are now removed!
%
%   - March 13 1996 - revision 2.0: first official major revision.
%   
%
%%%%%%%%%%%%%%
%
%   Known bugs: 
%   -----------
%   - horizontal spacing (indent) doesn't work with revtex4 class.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% for more complete informations you can see algorithm2e.tex
%
%
%%%%%%%%%%%%%%%%%%%%%%%% Identification Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
%
\ProvidesPackage{algorithm2e}[2013/01/06 v5.00 algorithms environments]
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Initial Code %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\@makeother\*% some package redefined it as a letter (as color.sty)
\def\@firstword#1 #2\@nil{#1}% an useful fonction
%%%%%%% Utilities:
% \ifArgumentEmpty<c><t><e> ; if c is empty, i.e. {}, then t, else e.
%    Function used internally, but may as well expose it to the user; it's useful
\begingroup
\catcode`\Q=3
\catcode`\T=3
\long\gdef\ALGOCF@argemptyaux#1#2Q#3#4#5T{#4}
\long\gdef\ifArgumentEmpty#1{%
  \begingroup\long\edef\@tempa{\endgroup
    \ALGOCF@argemptyaux#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T%
  }\@tempa
}
\endgroup
% \long\def\ifArgumentEmpty#1{\bgroup
% 	\catcode`\Q=3
% 	\catcode`\T=3
% 	\long\def\@tempa##1##2Q##3##4##5T{##4}%
% 	\xdef\@tempa{\@tempa#1QQ{\noexpand\@secondoftwo}{\noexpand\@firstoftwo}T}%
% \egroup\@tempa}
%%%%%%%%%%%
%
% \algocf@longdef -> shorthand to reduce
%    \expandafter\long\expandafter\def
% to
%    \expandafter\algocf@longdef
% may look insignificant, but reads that much better ;)
\def\algocf@longdef{\long\def}
%
% \algocf@newcommand (and helper \algocf@new@command) behaves like LaTeX's newcommand,
% with two differences:
%  - the argument is not "\<name>", but rather "<name>"; i.e. one level of indirection
%  - if the command exists already, then \renewcommand, rather than \newcommand
\def\algocf@newcommand#1{\expandafter\algocf@new@command\csname#1\endcsname}
\def\algocf@new@command#1{%
	\begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
	\expandafter\@ifundefined\@gtempa\newcommand\renewcommand#1}%
%
% \algocf@newcmdside<name><arity><body>
%   The largest time-saver; many commands we define have the pattern:
%     \<name>(<side_text>)<argX><argY>...
%   where "(<side_text>)" is optional. By defining them with this function,
%   the arguments are parsed and renumbered, i.e. the body works as if the
%   command was:
%     \<name><side_text><argX><argY>...
%   and can use \ifArgumentEmpty to see whether its #1 exists (default case
%   for the side text is (), so there's no difference between calling
%     \foo{bar}
%   or
%     \foo(){bar}
%   Technically this is new behaviour, but it shouldn't really occur...
\algocf@longdef\algocf@newcmdside#1#2#3{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3}%
}
%
% a serie of newcmdside macro for block that allows a comment after the end
%     \<name>(<side_text>)<argX><argY>...(<side_text>)% 
%
% 1. kind of begin-end : for command with only one block as begin-end 
\algocf@longdef\algocf@newcmdside@kobe#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2{\csname algocf@#1checkcomfol\endcsname{##1}{##2}}%
  % now check for last side comment; args are : <first side com (could be empty)>, <body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}}{\csname algocf@#1noendcom\endcsname{##1}{##2}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2(##3){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2{%
    \csname algocf@#1main\endcsname{##1}{##2}{}}%
  \algocf@newcommand{algocf@#1main}[3]{#2}%
}%
%
% 2. kind of if-else : for command with two blocks as if-then-else 
\algocf@longdef\algocf@newcmdside@koif#1#2{% <name of cmd><body of cmd>
  % command starts by checking for side comment at beginning
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
  }%
  % next we strip comment and include it in cmd that get body and check last side comment
  \expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1)##2##3{\csname algocf@#1checkcomfol\endcsname{##1}{##2}{##3}}%
  % now check for last side comment; args are : <1st side com>, <1st body of cmd>, <2nd body of cmd>
  \expandafter\algocf@longdef\csname algocf@#1checkcomfol\endcsname##1##2##3{\@ifnextchar({\csname algocf@#1withendcom\endcsname{##1}{##2}{##3}}{\csname algocf@#1noendcom\endcsname{##1}{##2}{##3}}}% call macro that manages end of command, with or without last side comment
  % finally manage end of macro... with end side comment...
  \expandafter\algocf@longdef\csname algocf@#1withendcom\endcsname##1##2##3(##4){%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{##4}}%
  % ... or without end side comment
  \expandafter\algocf@longdef\csname algocf@#1noendcom\endcsname##1##2##3{%
    \csname algocf@#1main\endcsname{##1}{##2}{##3}{}}%
  \algocf@newcommand{algocf@#1main}[4]{#2}%
}%
%
% \algocf@newcmdsides<name><arity><body><tail><closing>
%   Like the command above, but with an optional side text at the end
%   of the command as well, i.e.:
%     \<name>(<side_text>)<argX><argY>(<end_text>)
%   It may be a bit confusing that <arity> doesn't count <end_text>,
%   but since it is for internal use, the naming can be a little more
%   fuzzy. This function behaves as if:
%     <body'> = <body><if end_text: tail{end_text}><closing>
\algocf@longdef\algocf@newcmdsides#1#2#3#4#5{%
	\expandafter\def\csname#1\endcsname{%
		\@ifnextchar({\csname algocf@#1strip\endcsname}{\csname algocf@#1strip\endcsname()}%
	}%
	\expandafter\algocf@longdef\csname algocf@#1strip\endcsname(##1){\csname algocf@#1main\endcsname{##1}}%
	\algocf@newcommand{algocf@#1main}[#2]{#3\@ifnextchar({\csname algocf@#1end\endcsname}{#4#5}}%
	\expandafter\algocf@longdef\csname algocf@#1end\endcsname(##1){#4{##1}\strut\par}%
}%
%
% definition of commands which can be redefined in options of the package.
%
\newcounter{AlgoLine}%
\setcounter{AlgoLine}{0}%
%
\newcommand{\algocf@algocfref}{\relax}%
\newcommand{\listalgorithmcfname}{}%
\newcommand{\algorithmcfname}{}%
\@ifundefined{algorithmautorefname}{\newcommand{\algorithmautorefname}{algorithm}}{\renewcommand{\algorithmautorefname}{algorithm}}%
\newcommand{\algorithmcflinename}{}%
\newcommand{\algocf@typo}{}%
\newcommand{\@algocf@procname}{}\newcommand{\procedureautorefname}{}%
\newcommand{\SetAlgoProcName}[2]{\renewcommand{\@algocf@procname}{#1}\renewcommand{\procedureautorefname}{#2}}%
\newcommand{\@algocf@funcname}{}\newcommand{\functionautorefname}{}%
\newcommand{\SetAlgoFuncName}[2]{\renewcommand{\@algocf@funcname}{#1}\renewcommand{\functionautorefname}{#2}}%
\newcommand{\@algocf@titleofalgoname}{\algorithmcfname}%
\newcommand{\@algocf@algotitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algorithmcfname}}%
\newcommand{\@algocf@proctitleofalgo}{%
  \renewcommand{\@algocf@titleofalgoname}{\algocf@procname}}%
%
\newcommand{\algocf@style}{plain}%
\newcommand{\@ResetCounterIfNeeded}{}%
\newcommand{\@titleprefix}{}%
%
\newcommand{\algocf@numbering}[1]{\newcommand{\algocf@within}{#1}}%
%
\newcommand{\defaultsmacros@algo}{\algocf@defaults@shortend}%
%
\newcommand{\algocf@list}{loa}%
\newcommand{\algocf@float}{algocf}%
%
\newcommand{\algocf@envname}{algorithm}%
\newcommand{\algocf@listofalgorithms}{listofalgorithms}%
%
%
%% redefine chapter so that it adds a vspace in the loa as the original does for lof and lot
% \let\algocf@original@chapter=\chapter%
% \def\chapter{\expandafter\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}%
%
% bug correction with hyperref submitted by Hubert Meier
\begingroup\expandafter\expandafter\expandafter\endgroup 
\expandafter\ifx\csname @chapter\endcsname\relax\else 
% \let\algocf@original@chapter=\chapter% 
% \def\chapter{\addtocontents{loa}{\protect\addvspace{10\p@}}\algocf@original@chapter}% 
\let\algocf@original@chapter=\@chapter%
\@ifclassloaded{krantz}{%
\def\@chapter[#1][#2]#3{\algocf@original@chapter[#1][#2]{#3}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}{%
\def\@chapter[#1]#2{\algocf@original@chapter[#1]{#2}\addtocontents{loa}{\protect\addvspace{10\p@}}}% 
}%
\fi
%
%% if@restonecol is defined in article and book but some other classes don't define it and we need it, so we do
\ifx\if@restonecol\relax\else\newif\if@restonecol\fi%
%
%
%%%%%%%%%%%%%%%%%%%%%% Declaration of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\RequirePackage{ifthen}%
%
\newboolean{algocf@displayblockmarkers}\setboolean{algocf@displayblockmarkers}{false}%
\DeclareOption{displayblockmarkers}{%
  \setboolean{algocf@displayblockmarkers}{true}%
}
\newboolean{algocf@displaygroupmarkers}{\setboolean{algocf@displaygroupmarkers}{false}
\DeclareOption{displaygroupmarkers}{%
  \setboolean{algocf@displaygroupmarkers}{true}%
}
%
\newboolean{algocf@nokwfunc}\setboolean{algocf@nokwfunc}{false}%
\DeclareOption{nokwfunc}{%
  \setboolean{algocf@nokwfunc}{true}%
}%
%
\newboolean{algocf@oldcommands}\setboolean{algocf@oldcommands}{false}%
\DeclareOption{oldcommands}{%
  \setboolean{algocf@oldcommands}{true}%
}%
%
\newboolean{algocf@leftlinenumber}\setboolean{algocf@leftlinenumber}{true}%
\newcommand{\setLeftLinesNumbers}{\setboolean{algocf@leftlinenumber}{true}}%
\newcommand{\setRightLinesNumbers}{\setboolean{algocf@leftlinenumber}{false}}%
\DeclareOption{rightnl}{%
  \setRightLinesNumbers%
}%
%
\newboolean{algocf@endfloat}\setboolean{algocf@endfloat}{false}%
\DeclareOption{endfloat}{%
  \setboolean{algocf@endfloat}{true}%
  \newcounter{postalgo}\setcounter{postalgo}{0}%
}%
%
\newboolean{algocf@procnumbered}\setboolean{algocf@procnumbered}{false}%
\DeclareOption{procnumbered}{%
  \setboolean{algocf@procnumbered}{true}%
}%
%
\DeclareOption{algo2e}{%
  \renewcommand{\algocf@envname}{algorithm2e}%
  \renewcommand{\algocf@listofalgorithms}{listofalgorithmes}%
}%
%
\newboolean{algocf@slide}\setboolean{algocf@slide}{false}%
\DeclareOption{slide}{%
  \setboolean{algocf@slide}{true}%
}%
%
\newboolean{algocf@figurecaption}\setboolean{algocf@figurecaption}{false}%
\DeclareOption{figure}{%
\renewcommand{\algocf@list}{lof}%
\renewcommand{\algocf@float}{figure}%
\AtBeginDocument{\@ifpackageloaded{caption}{\setboolean{algocf@figurecaption}{true}}{}}%
}%
%
\newboolean{algocf@optonelanguage}\setboolean{algocf@optonelanguage}{false}%
\DeclareOption{onelanguage}{\setboolean{algocf@optonelanguage}{true}}%
%
\newcommand{\algocf@languagechoosen}{english}%
\newboolean{algocf@localkw@english}\setboolean{algocf@localkw@english}{true}%
\DeclareOption{englishkw}{%
\setboolean{algocf@localkw@english}{true}%
}%
%
\DeclareOption{english}{%
\renewcommand{\listalgorithmcfname}{List of Algorithms}%
\renewcommand{\algorithmcfname}{Algorithm}%
\renewcommand{\algorithmautorefname}{algorithm}%
\renewcommand{\algorithmcflinename}{line}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedure}%
\renewcommand{\@algocf@funcname}{Function}%
\renewcommand{\procedureautorefname}{procedure}%
\renewcommand{\functionautorefname}{function}%
\renewcommand{\algocf@languagechoosen}{english}%
}%
%
%----
\newboolean{algocf@localkw@french}\setboolean{algocf@localkw@french}{false}%
\DeclareOption{frenchkw}{%
\setboolean{algocf@localkw@french}{true}%
}%
%
\DeclareOption{french}{%
\renewcommand{\listalgorithmcfname}{Liste des Algorithmes}%
\renewcommand{\algorithmcfname}{Algorithme}%
\renewcommand{\algorithmautorefname}{algorithme}%
\renewcommand{\algorithmcflinename}{ligne}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Proc\'edure}%
\renewcommand{\@algocf@funcname}{Fonction}%
\renewcommand{\procedureautorefname}{proc\'edure}%
\renewcommand{\functionautorefname}{fonction}%
\renewcommand{\algocf@languagechoosen}{french}%
}%
%
%----
\newboolean{algocf@localkw@czech}\setboolean{algocf@localkw@czech}{false}%
\DeclareOption{czechkw}{%
\setboolean{algocf@localkw@czech}{true}%
}%
%
\DeclareOption{czech}{%
\renewcommand{\listalgorithmcfname}{Seznam algoritm\r{u}}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkce}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{czech}%
}%
%
%----
\newboolean{algocf@localkw@german}\setboolean{algocf@localkw@german}{false}%
\DeclareOption{germankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{german}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\DeclareOption{ngermankw}{%
\setboolean{algocf@localkw@german}{true}%
}%
%
\DeclareOption{ngerman}{%
\renewcommand{\listalgorithmcfname}{Liste der Algorithmen}%
\renewcommand{\algorithmcfname}{Algorithmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Zeile}%
\renewcommand{\algocf@typo}{\ }%
\renewcommand{\@algocf@procname}{Prozedur}%
\renewcommand{\@algocf@funcname}{Funktion}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{german}%
}%
%
%----
\newboolean{algocf@localkw@portuguese}\setboolean{algocf@localkw@portuguese}{false}%
\DeclareOption{portuguesekw}{%
\setboolean{algocf@localkw@portuguese}{true}%
}%
%
\DeclareOption{portuguese}{%
\renewcommand{\listalgorithmcfname}{Lista de Algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{linha}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimento}%
\renewcommand{\@algocf@funcname}{Fun\c{c}\~{a}o}%
\renewcommand{\procedureautorefname}{procedimento}%
\renewcommand{\functionautorefname}{fun\c{c}\~{a}o}%
\renewcommand{\algocf@languagechoosen}{portuguese}%
}%
%
%----
\newboolean{algocf@localkw@italiano}\setboolean{algocf@localkw@italiano}{false}%
\DeclareOption{italianokw}{%
\setboolean{algocf@localkw@italiano}{true}%
}%
%
\DeclareOption{italiano}{%
\renewcommand{\listalgorithmcfname}{Elenco degli algoritmi}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{riga}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funzione}%
\renewcommand{\procedureautorefname}{procedura}%
\renewcommand{\functionautorefname}{funzione}%
\renewcommand{\algocf@languagechoosen}{italiano}%
}%
%----
\newboolean{algocf@localkw@spanish}\setboolean{algocf@localkw@spanish}{false}%
\DeclareOption{spanishkw}{%
\setboolean{algocf@localkw@spanish}{true}%
}%
%
\DeclareOption{spanish}{%
\renewcommand{\listalgorithmcfname}{\'Indice de algoritmos}%
\renewcommand{\algorithmcfname}{Algoritmo}%
\renewcommand{\algorithmautorefname}{algoritmo}%
\renewcommand{\algorithmcflinename}{l\'inea}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedimiento}%
\renewcommand{\@algocf@funcname}{Funci\'on}%
\renewcommand{\procedureautorefname}{procedimiento}%
\renewcommand{\functionautorefname}{funci\'on}%
\renewcommand{\algocf@languagechoosen}{spanish}%
}%
%----
\newboolean{algocf@localkw@slovak}\setboolean{algocf@localkw@slovak}{false}%
\DeclareOption{slovakkw}{%
\setboolean{algocf@localkw@slovak}{true}%
}%
%
\DeclareOption{slovak}{%
\renewcommand{\listalgorithmcfname}{Zoznam algoritmov}%
\renewcommand{\algorithmcfname}{Algoritmus}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{Radek}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Proced\'{u}ra}%
\renewcommand{\@algocf@funcname}{Funkcia}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{slovak}%
}%
%
%----
\newboolean{algocf@localkw@croatian}\setboolean{algocf@localkw@croatian}{false}%
\DeclareOption{croatiankw}{%
\setboolean{algocf@localkw@croatian}{true}%
}%
%
\DeclareOption{croatian}{%
\renewcommand{\listalgorithmcfname}{Popis algoritama}%
\renewcommand{\algorithmcfname}{Algoritam}%
\renewcommand{\algorithmautorefname}{\algorithmcfname}%
\renewcommand{\algorithmcflinename}{redak}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Procedura}%
\renewcommand{\@algocf@funcname}{Funkcija}%
\renewcommand{\procedureautorefname}{\@algocf@procname}%
\renewcommand{\functionautorefname}{\@algocf@funcname}%
\renewcommand{\algocf@languagechoosen}{croatian}%
}%
%%% adding 'turkish' option customization
%
%----
\newboolean{algocf@localkw@turkish}\setboolean{algocf@localkw@turkish}{false}%
\DeclareOption{turkishkw}{%
\setboolean{algocf@localkw@turkish}{true}%
}%
\DeclareOption{turkish}{%
\renewcommand{\listalgorithmcfname}{Algoritma Listesi}%
\renewcommand{\algorithmcfname}{Algoritma}%
\renewcommand{\algorithmautorefname}{algoritma}%
\renewcommand{\algorithmcflinename}{?izgi}%
\renewcommand{\algocf@typo}{}%
\renewcommand{\@algocf@procname}{Prosed?r}%
\renewcommand{\@algocf@funcname}{Fonksiyon}%
\renewcommand{\procedureautorefname}{prosed?r}%
\renewcommand{\functionautorefname}{fonksiyon}%
\renewcommand{\algocf@languagechoosen}{turkish}%
}%
%
% OPTIONs plain, boxed, ruled, algoruled & boxruled
%
\newcommand{\algocf@style@plain}{\renewcommand{\algocf@style}{plain}}%
\newcommand{\algocf@style@boxed}{\renewcommand{\algocf@style}{boxed}}%
\newcommand{\algocf@style@ruled}{\renewcommand{\algocf@style}{ruled}}%
\newcommand{\algocf@style@algoruled}{\renewcommand{\algocf@style}{algoruled}}%
\newcommand{\algocf@style@boxruled}{\renewcommand{\algocf@style}{boxruled}}%
\newcommand{\algocf@style@tworuled}{\renewcommand{\algocf@style}{tworuled}}%
\newcommand{\algocf@style@plainruled}{\renewcommand{\algocf@style}{plainruled}}%
\newcommand{\RestyleAlgo}[1]{\csname algocf@style@#1\endcsname}%
\DeclareOption{plain}{\algocf@style@plain}%
\DeclareOption{plainruled}{\algocf@style@plainruled}%
\DeclareOption{boxed}{\algocf@style@boxed}%
\DeclareOption{ruled}{\algocf@style@ruled}%
\DeclareOption{algoruled}{\algocf@style@algoruled}%
\DeclareOption{boxruled}{\algocf@style@boxruled}%
\DeclareOption{tworuled}{\algocf@style@tworuled}%
%
% OPTIONs algopart,algochapter & algosection
%
\DeclareOption{algopart}{\algocf@numbering{part}}%       %algo part numbered
\DeclareOption{algochapter}{\algocf@numbering{chapter}}% %algo chapter numbered
\DeclareOption{algosection}{\algocf@numbering{section}}% %algo section numbered
%
% OPTIONs resetcount & noresetcount
%
\DeclareOption{resetcount}{\renewcommand{\@ResetCounterIfNeeded}{\setcounter{AlgoLine}{0}}}%
\DeclareOption{noresetcount}{\renewcommand{\@ResetCounterIfNeeded}{}}%
%
% OPTIONs algorithm hanging for long lines
%
\newlength{\algocf@hangindent}\setlength{\algocf@hangindent}{.5em}
\newcommand{\SetAlgoHangIndent}[1]{\setlength{\algocf@hangindent}{#1}}
%
\newboolean{algocf@hanging}\setboolean{algocf@hanging}{true}% hanging is handle by default
\newboolean{algocf@hanginginout}\setboolean{algocf@hanginginout}{false}% inout are managed as previously: hanging set by inout keywords
\newboolean{algocf@hangingcomment}\setboolean{algocf@hangingcomment}{false}% comment that are not side comment are indented accordingly to comment mark, not as normal text
\newcommand{\algocf@everyparnl}{\relax}%
\newcommand{\algocf@everyparhanging}{\hangafter=1\hangindent=\algocf@hangindent\relax}%
\newcommand{\algocf@everypar}{\algocf@everyparnl\algocf@everyparhanging}%
\newcommand{\algocf@seteverypar}{%
  \ifthenelse{\boolean{algocf@hanging}}{\everypar{\algocf@everypar}}{\relax}%
}%
%
\newcommand{\algocf@seteveryparnl}[1]{\renewcommand{\algocf@everyparnl}{#1}\everypar{\algocf@everypar}}%
\newcommand{\algocf@seteveryparhanging}[1]{%
\let\algocf@oldeveryparhanging=\algocf@everyparhanging%
\renewcommand{\algocf@everyparhanging}{#1}\everypar{\algocf@everypar}%
}%
\newcommand{\algocf@reseteveryparhanging}{%
\let\algocf@everyparhanging=\algocf@oldeveryparhanging%
\everypar{\algocf@everypar}%
}%
\DeclareOption{hanginginout}{\setboolean{algocf@hanginginout}{true}}%
\DeclareOption{hangingcomment}{\setboolean{algocf@hangingcomment}{true}}%
\DeclareOption{noalgohanging}{%
  \setboolean{algocf@hanginginout}{false}%
  \setboolean{algocf@hangingcomment}{false}%
  \setboolean{algocf@hanging}{false}%
}%
%\newcommand{
%
%
% OPTION linesnumbered
%
\newboolean{algocf@linesnumbered}\setboolean{algocf@linesnumbered}{false}%
\newcommand{\algocf@linesnumbered}{\relax}%
\DeclareOption{linesnumbered}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}%
}%
%
% OPTION linesnumberedhidden
%
\DeclareOption{linesnumberedhidden}{%
  \setboolean{algocf@linesnumbered}{true}%
  \renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}%
}%
%
% OPTION commentsnumbered inoutnumbered
%
\newboolean{algocf@commentsnumbered}\setboolean{algocf@commentsnumbered}{false}%
\DeclareOption{commentsnumbered}{\setboolean{algocf@commentsnumbered}{true}}%
\newboolean{algocf@inoutnumbered}\setboolean{algocf@inoutnumbered}{false}%
\DeclareOption{inoutnumbered}{\setboolean{algocf@inoutnumbered}{true}}%
%
% OPTIONs titlenumbered & titlenotnumbered
%
\DeclareOption{titlenumbered}{%
  \renewcommand{\@titleprefix}{%
    \refstepcounter{\algocf@float}%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\ \expandafter\csname the\algocf@float\endcsname\algocf@typo: }%
  }%
}%
%
\DeclareOption{titlenotnumbered}{\renewcommand{\@titleprefix}{%
    \AlTitleSty{\AlTitleFnt\@algocf@titleofalgoname\algocf@typo: }}%
}%
%
% OPTIONs algonl
% line numbered with the counter of the algorithm
%
\DeclareOption{algonl}{\renewcommand{\theAlgoLine}{\expandafter\csname the\algocf@float\endcsname.\arabic{AlgoLine}}}%
%
% OPTIONs lined, vlined & noline
%
\DeclareOption{lined}{\AtBeginDocument{\SetAlgoLined}}%   \SetAlgoLined (default)
\DeclareOption{vlined}{\AtBeginDocument{\SetAlgoVlined}}% \SetAlgoVlined
\DeclareOption{noline}{\AtBeginDocument{\SetAlgoNoLine}}%\SetAlgoNoLine
%
% OPTIONs longend, shotend & noend
%
\DeclareOption{longend}{\AtBeginDocument{\SetAlgoLongEnd}}%  \SetAlgoLongEnd
\DeclareOption{shortend}{\AtBeginDocument{\SetAlgoShortEnd}}%\SetAlgoShortEnd
\DeclareOption{noend}{\AtBeginDocument{\SetAlgoNoEnd}}%      \SetAlgoNoEnd
%
\DeclareOption{nosemicolon}{\AtBeginDocument{\DontPrintSemicolon}}%      \SetAlgoNoEnd
%
% OPTION dotoc
%
\newboolean{algocf@dotocloa}\setboolean{algocf@dotocloa}{false}%
\DeclareOption{dotocloa}{%
  \setboolean{algocf@dotocloa}{true}%
}
%
% OPTION comments
%
\newboolean{algocf@optfillcomment}\setboolean{algocf@optfillcomment}{true}%
\DeclareOption{nofillcomment}{%
  \setboolean{algocf@optfillcomment}{false}%
}%
\DeclareOption{fillcomment}{%
  \setboolean{algocf@optfillcomment}{true}%
}%
%
% OPTION sidecommments
%
\newboolean{algocf@scleft}\setboolean{algocf@scleft}{false}%
\DeclareOption{scleft}{%
  \setboolean{algocf@scleft}{true}%
}%
\DeclareOption{sright}{% default
  \setboolean{algocf@scleft}{false}%
}%
%
% OPTION norelsize
%
\newboolean{algocf@norelsize}\setboolean{algocf@norelsize}{false}%
\DeclareOption{norelsize}{%
  \setboolean{algocf@norelsize}{true}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%% Execution of Options %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\ExecuteOptions{english,plain,resetcount,titlenotnumbered,lined,shortend}%
%
\ProcessOptions%
%
\@algocf@algotitleofalgo% fix name for \TitleOfAlgo to \algorithmcfname by default
%
%%%%%%%%%%%%%%%%%%%%%%%%%% Package Loading %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\RequirePackage{xspace}%
%
\ifthenelse{\boolean{algocf@endfloat}}{%
  \RequirePackage{endfloat}%
}{\relax}%
%
\ifthenelse{\boolean{algocf@norelsize}}{%
  \newcommand{\relsize}[1]{\scriptsize}%
}{%
  \RequirePackage{relsize}%
}%
%
\ifthenelse{\boolean{algocf@slide}}{\RequirePackage{color}}{}%
%
%
\AtEndOfPackage{%
  \ifthenelse{\boolean{algocf@dotocloa}}{%
    \renewcommand{\listofalgorithms}{\tocfile{\listalgorithmcfname}{loa}}%
  }{\relax}%
}%
%
% if loa in toc required, load tocbibind package if not already done.
\ifthenelse{\boolean{algocf@dotocloa}}{%
  \ifx\@tocextra\undefined%
  \RequirePackage{tocbibind}%
  \fi%
}{\relax}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Main Part %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\algocf@name}{algorithm2e}%
\newcommand{\algocf@date}{october 19 2015}%
\newcommand{\algocf@version}{Release 5.1}%
\newcommand{\algocf@id}{\algocf@version\space -- \algocf@date\space --}%
\typeout{********************************************************^^JPackage `\algocf@name'\space\algocf@id^^J%
         - algorithm2e-announce@lirmm.fr  mailing list for announcement about releases^^J%
         - algorithm2e-discussion@lirmm.fr mailing list for discussion about package^^J%
         subscribe by emailing sympa@lirmm.fr with 'subscribe <list> <firstname name>'^^J%
         - Author: Christophe Fiorio (christophe.fiorio@umontpellier.fr)^^J********************************************************}%
%%
%%
%%
%%
%%
%%
%%%% hyperref compatibility tricks: Hyperref package defines H counters from
   % standard counters (i.e \theHpage from \thepage) and check some particular
   % counters of some packages, unfortunately it doesn't do the same for
   % algorithm2e package but act as Hcounter was defined. To avoid errors we
   % defined \theHalgocf ourself
%%%%
%
\@ifundefined{theHalgocf}{\def\theHalgocf{\thealgocf}}{}%
\@ifundefined{theHAlgoLine}{\def\theHAlgoLine{\theAlgoLine}}{}%
\@ifundefined{theHalgocfproc}{\def\theHalgocfproc{0}}{}%
\@ifundefined{theHalgocffunc}{\def\theHalgocffunc{0}}{}%
\@ifundefined{toclevel@algocf}{\def\toclevel@algocf{0}}{}%
%
% autoref from hyperref needs an autorefname, so we give it.
\def\AlgoLineautorefname{\algorithmcflinename}%
\def\algocfautorefname{\algorithmautorefname}%
\def\algocfprocautorefname{\procedureautorefname}%
\def\algocffuncautorefname{\functionautorefname}%
%%
%%
%%
\newcommand{\@defaultskiptotal}{0.5em}%
\newskip\skiptotal\skiptotal=0.5em%
\newskip\skiplinenumber\skiplinenumber=\hsize\advance\skiplinenumber by-\skiptotal%
\newskip\skiprule%
\newskip\skiphlne%
\newskip\skiptext%
\newskip\skiplength%
\newskip\algomargin%
\newskip\skipalgocfslide\skipalgocfslide=1em%
\newdimen\algowidth%
\newdimen\inoutsize%
\newdimen\inoutindent%
\newdimen\interspacetitleruled\setlength{\interspacetitleruled}{2pt}%
\newdimen\interspacealgoruled\setlength{\interspacealgoruled}{2pt}%
\newdimen\interspacetitleboxruled\setlength{\interspacetitleboxruled}{2\lineskip}%
%
\newcommand{\@algoskip}{\smallskip}%
\newcommand{\SetAlgoSkip}[1]{\renewcommand{\@algoskip}{\csname#1\endcsname}}%
\newcommand{\@algoinsideskip}{\relax}%
\newcommand{\SetAlgoInsideSkip}[1]{\renewcommand{\@algoinsideskip}{\csname#1\endcsname}}%
%
% ruledwidth
%
\newlength{\algocf@ruledwidth}\setlength{\algocf@ruledwidth}{\linewidth}%
\newboolean{algocf@customruledwidth}\setboolean{algocf@customruledwidth}{false}%
\newcommand{\SetCustomAlgoRuledWidth}[1]{%
  \setboolean{algocf@customruledwidth}{true}%
  \ifthenelse{\boolean{algocf@customruledwidth}}{\setlength{\algocf@ruledwidth}{#1}}{\relax}%
}%
%
\newsavebox{\algocf@inoutbox}%
\newsavebox{\algocf@inputbox}%
%%
%%
\newcommand{\arg@e}{}%
\newcommand{\arg@space}{\ }%
\newcommand{\BlankLine}{\vskip 1ex}%
%%
\newcommand{\vespace}{1ex}%
\newcommand{\SetInd}[2]{%
\skiprule=#1%
\skiptext=#2%
\skiplength=\skiptext\advance\skiplength by \skiprule\advance\skiplength by 0.4pt}%
\SetInd{0.5em}{1em}
\algomargin=\leftskip\advance\algomargin by \parindent%
\newcommand{\IncMargin}[1]{\advance\algomargin by #1}%
\newcommand{\DecMargin}[1]{\advance\algomargin by -#1}%
\newcommand{\SetNlSkip}[1]{%
  \renewcommand{\@defaultskiptotal}{#1}%
  \setlength{\skiptotal}{#1}}%
%%
\newskip\AlCapSkip\AlCapSkip=0ex%
\newskip\AlCapHSkip\AlCapSkip=0ex%
\newcommand{\SetAlCapSkip}[1]{\setlength{\AlCapSkip}{#1}}%
\newcommand{\SetAlCapHSkip}[1]{\setlength{\AlCapHSkip}{#1}}%
\SetAlCapHSkip{.5\algomargin}%
%%
%%
\newskip\algoskipindent
\newcommand{\algocf@adjustskipindent}{%
  \algoskipindent=\skiprule%
  \advance\algoskipindent by \skiptext\advance\algoskipindent by 0.4pt}
\algocf@adjustskipindent%
%
\newcommand{\Indentp}[1]{\advance\leftskip by #1}%
\newcommand{\Indp}{\algocf@adjustskipindent\advance\leftskip by \algoskipindent}
\newcommand{\Indpp}{\advance\leftskip by 0.5em}%
\newcommand{\Indm}{\algocf@adjustskipindent\advance\leftskip by -\algoskipindent}
\newcommand{\Indmm}{\advance\leftskip by -0.5em}%
%
%%
%%
%% Line Numbering
%%
%%
% number line style
\newcommand{\algocf@nlrelsize}{-2}\newcommand{\SetAlgoNlRelativeSize}[1]{\renewcommand{\algocf@nlrelsize}{#1}}%
\newcommand{\NlSty}[1]{\textnormal{\textbf{\relsize{\algocf@nlrelsize}#1}}}% default definition
\newcommand{\SetNlSty}[3]{\renewcommand{\NlSty}[1]{\textnormal{\csname#1\endcsname{\relsize{\algocf@nlrelsize}#2##1#3}}}}%
%
% nl definitions
%
\newsavebox{\algocf@nlbox}%
\newcommand{\algocf@printnl}[1]{%
  \ifthenelse{\boolean{algocf@leftlinenumber}}{%
    \skiplinenumber=\skiptotal\advance\skiplinenumber by\leftskip%
    \strut\raisebox{0pt}{\llap{\NlSty{#1}\kern\skiplinenumber}}\ignorespaces%
  }{%
    \sbox\algocf@nlbox{\NlSty{#1}}%
    \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip\advance\skiplinenumber by-\skiptext%
    \advance\skiplinenumber by\algomargin\advance\skiplinenumber by.3em\advance\skiplinenumber by-\wd\algocf@nlbox%
    % to handle particular case of until: printnl is after 'until' keyword has been writen, so we need to substract length of this keyword
    \advance\skiplinenumber by-\algocf@skipuntil%
    \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\NlSty{#1\ignorespaces}}}\ignorespaces%
  }%
}%
\newcommand{\algocf@nl@sethref}[1]{%
  \renewcommand{\theHAlgoLine}{\thealgocfproc.#1}%
  \hyper@refstepcounter{AlgoLine}\gdef\@currentlabel{#1}%
}%
\newcommand{\nl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \algocf@printnl{\theAlgoLine}%
}%
%
\newcommand{\nllabel}[1]{\label{#1}}%
%
\newcommand{\enl}{%
  \@ifundefined{hyper@refstepcounter}{% if not hyperref then do a simple refstepcounter
    \refstepcounter{AlgoLine}\gdef\@currentlabel{\theAlgoLine}%
  }{% else if hyperref, do the anchor so 2 lines in two differents algorithms cannot have the same href
    \stepcounter{AlgoLine}\algocf@nl@sethref{\theAlgoLine}%
  }% now we can do the line numbering
  \skiplinenumber=\hsize\advance\skiplinenumber by-\leftskip%
  \strut\raisebox{0pt}{\rlap{\kern\skiplinenumber\strut\NlSty{\theAlgoLine}}}\ignorespaces%
}%
%% nlset
\newcommand{\nlset}[1]{%
  \@ifundefined{hyper@refstepcounter}{\protected@edef\@currentlabel{#1}}{\algocf@nl@sethref{#1}}\algocf@printnl{#1}%
}%
%
%% lnl definitions
\newcommand{\lnl}[1]{\nl\label{#1}\ignorespaces}%
%
%% lnlset
\newcommand{\lnlset}[2]{\nlset{#2}\label{#1}}%
%
% set char put at end of each line
%
\newcommand{\algocf@endline}{\string;}
\newcommand{\SetEndCharOfAlgoLine}[1]{\renewcommand{\algocf@endline}{#1}}
%
% end of line definition
%
\newcommand{\@endalgocfline}{\algocf@endline}% default definition: printsemicolon
\newcommand{\DontPrintSemicolon}{\renewcommand{\@endalgocfline}{\relax}}%
\newcommand{\PrintSemicolon}{\renewcommand{\@endalgocfline}{\algocf@endline}}%
\newcommand{\@endalgoln}{\@endalgocfline\hfill\strut\par}%
%
% line numbering
%
\newcommand{\LinesNumbered}{\setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\nl}}}%
\newcommand{\LinesNotNumbered}{%
  \setboolean{algocf@linesnumbered}{false}%
  \renewcommand{\algocf@linesnumbered}{\relax}%
}%
%
\newcommand{\LinesNumberedHidden}{%
  \setboolean{algocf@linesnumbered}{true}\renewcommand{\algocf@linesnumbered}{\algocf@seteveryparnl{\stepcounter{AlgoLine}}}}%
\newcommand{\ShowLn}{\nlset{\theAlgoLine}\ignorespaces}% display the line number on this line (without labelling)
\newcommand{\ShowLnLabel}[1]{\lnlset{#1}{\theAlgoLine}\ignorespaces}% display the line number and label this line
%
%%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Styling text commands
%
\newcommand{\AlFnt}{\relax}% default definition
\newcommand{\SetAlFnt}[1]{\renewcommand{\AlFnt}{#1}}%
\newcommand{\AlTitleFnt}{\relax}% default definition
\newcommand{\SetAlTitleFnt}[1]{\renewcommand{\AlTitleFnt}{#1}}%
%
\newcommand{\AlCapFnt}{\relax}% default definition
\newcommand{\SetAlCapFnt}[1]{\renewcommand{\AlCapFnt}{#1}}%
\newcommand{\AlCapNameFnt}{\relax}% default definition
\newcommand{\SetAlCapNameFnt}[1]{\renewcommand{\AlCapNameFnt}{#1}}%
%
\newcommand{\ProcFnt}{\relax}% default definition
\newcommand{\SetProcFnt}[1]{\renewcommand{\ProcFnt}{#1}}%
\newcommand{\ProcNameFnt}{\relax}% default definition
\newcommand{\SetProcNameFnt}[1]{\renewcommand{\ProcNameFnt}{#1}}%
\newcommand{\ProcArgFnt}{\relax}% default definition
\newcommand{\SetProcArgFnt}[1]{\renewcommand{\ProcArgFnt}{#1}}%
%
\newcommand{\AlTitleSty}[1]{\textbf{#1}\unskip}% default definition
\newcommand{\SetAlTitleSty}[1]{\renewcommand{\AlTitleSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetAlCapSty}[1]{\renewcommand{\AlCapSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\AlCapNameSty}[1]{\textnormal{#1}\unskip}% default definition
\newcommand{\SetAlCapNameSty}[1]{\renewcommand{\AlCapNameSty}[1]{\textnormal{\csname #1\endcsname{##1}}\unskip}}%
%
\newcommand{\ProcSty}[1]{\AlCapSty{#1}}%
\newcommand{\SetProcSty}[1]{\renewcommand{\ProcSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcNameSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcNameSty}[1]{\renewcommand{\ProcNameSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProcArgSty}[1]{\AlCapNameSty{#1}}%
\newcommand{\SetProcArgSty}[1]{\renewcommand{\ProcArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
\newcommand{\KwSty}[1]{\textnormal{\textbf{#1}}\unskip}% default definition
\newcommand{\SetKwSty}[1]{\renewcommand{\KwSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetArgSty{emph}
\newcommand{\SetArgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncArgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetFuncArgSty{emph}
\newcommand{\SetFuncArgSty}[1]{\renewcommand{\FuncArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\FuncSty}[1]{\textnormal{\texttt{#1}}\unskip}%\SetFuncSty{texttt}
\newcommand{\SetFuncSty}[1]{\renewcommand{\FuncSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\ProgSty}[1]{\textnormal{\emph{#1}}\unskip}%\SetProgSty{emphg}
\newcommand{\SetProgSty}[1]{\renewcommand{\ArgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\DataSty}[1]{\textnormal{\textsf{#1}}\unskip}%%\SetDataSty{textsf}
\newcommand{\SetDataSty}[1]{\renewcommand{\DataSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\CommentSty}[1]{\textnormal{\texttt{#1}}\unskip}%%\SetDataSty{texttt}
\newcommand{\SetCommentSty}[1]{\renewcommand{\CommentSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
\newcommand{\TitleSty}[1]{#1\unskip}%\SetTitleSty{}{}
\newcommand{\SetTitleSty}[2]{\renewcommand{\TitleSty}[1]{%
\csname#1\endcsname{\csname#2\endcsname##1}}\unskip}%
\newcommand{\BlockMarkersSty}[1]{\KwSty{#1}}%
\newcommand{\SetBlockMarkersSty}[1]{\renewcommand{\BlockMarkersSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}%
%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Block basic commands
%
\newcommand{\algocf@push}[1]{\advance\skiptotal by #1\moveright #1}%
\newcommand{\algocf@pop}[1]{\advance\skiptotal by -#1}%
\newcommand{\algocf@addskiptotal}{\advance\skiptotal by 0.4pt\advance\hsize by -0.4pt\advance\hsize by -\skiplength}% 0.4 pt=width of \vrule
\newcommand{\algocf@subskiptotal}{\advance\skiptotal by -0.4pt\advance\hsize by 0.4pt\advance\hsize by \skiplength}% 0.4 pt=width of \vrule
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% group of instructions definition
%
\skiphlne=.8ex%
\newcommand{\SetVlineSkip}[1]{\skiphlne=#1}%
\newcommand{\algocf@bblock}{\BlockMarkersSty{begin}}%
\newcommand{\algocf@eblock}{\BlockMarkersSty{end}}%
\newcommand{\AlgoDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{true}}%
\newcommand{\AlgoDontDisplayBlockMarkers}{\setboolean{algocf@displayblockmarkers}{false}}%
\newcommand{\AlgoDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{true}}%
\newcommand{\AlgoDontDisplayGroupMarkers}{\setboolean{algocf@displaygroupmarkers}{false}}%
\newcommand{\algocf@bblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@bblock\par}{\relax}%
}%
\newcommand{\algocf@eblockcode}{%
  \ifthenelse{\boolean{algocf@displayblockmarkers}}{\algocf@eblock\par}{\relax}%
}%
\newcommand{\algocf@bgroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@bblock}{\relax}%
}%
\newcommand{\algocf@egroupcode}{%
  \ifthenelse{\boolean{algocf@displaygroupmarkers}}{\algocf@eblock}{\relax}%
}%
\newcommand{\SetAlgoBlockMarkers}[2]{%
  \ifArgumentEmpty{#1}{%
    \renewcommand{\algocf@bblock}{\relax}%
  }{%
    \renewcommand{\algocf@bblock}{\BlockMarkersSty{#1}}%
  }% begin marker set
  \ifArgumentEmpty{#2}{%
    \renewcommand{\algocf@eblock}{\relax}%
  }{%
    \renewcommand{\algocf@eblock}{\BlockMarkersSty{#2}}%
  }% end marker set
}
%
%%%%%%%%% block with a vertical line end by a little horizontal line
\newcommand{\algocf@Vline}[1]{%     no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}\Hlne}}\vskip\skiphlne% inside the block
  \algocf@pop{\skiprule}%\algocf@subskiptotal% restore indentation
  \nointerlineskip}% no vskip after
%
%%%%%%%%% block with a vertical line
\newcommand{\algocf@Vsline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%        move to the right before the vertical rule
  \hbox{\vrule%               the vertical rule
    \vtop{\algocf@push{\skiptext}%move the right after the rule
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}% restore indentation
  \algocf@eblockcode%
}
%
\newcommand{\algocf@Hlne}{\hrule height 0.4pt depth 0pt width .5em}%
%
%%%%%%%%%  block without line
\newcommand{\algocf@Noline}[1]{%    no vskip in between boxes but a strut to separate them, 
  \strut\par\nointerlineskip% then interblock space stay the same whatever is inside it
  \algocf@bblockcode%
  \algocf@push{\skiprule}%
  \hbox{%
    \vtop{\algocf@push{\skiptext}%
      \vtop{\algocf@addskiptotal #1}}}% inside the block
  \algocf@pop{\skiprule}%
  \algocf@eblockcode%
  % \nointerlineskip% no vskip after
}%
%%%%%%%%%
%
%% default=NoLine
%
\newcommand{\algocf@group}[1]{\algocf@Noline{#1}}% group: set of instruction depending from another (ex: then part of the If)
\newcommand{\algocf@@@eblock}[2]{#1\ifArgumentEmpty{#2}{\relax}{\KwSty{\@algocf@endoption{#2}}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@@block}[3]{#1\ifArgumentEmpty{#2}{\ifArgumentEmpty{#3}{\relax}{ #3\relax}}{\KwSty{\@algocf@endoption{#2}}\ifArgumentEmpty{#3}{\relax}{ #3}\strut\par}}% block: group with a end keyword.
\newcommand{\algocf@@block}[3]{\algocf@@@block{#1}{#2}{#3}}% block: group with a end keyword.
\newcommand{\algocf@block}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
%\newcommand{\algocf@nblock}[3]{\algocf@@block{#1}{#2}{#3}}% command that will be used and redefined accordingly to noend option
\newcommand{\algocf@setBlock}{%
  \ifthenelse{\boolean{algocf@optnoend}}{%     if no end option
    \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%     block will be a group
  }{%                                          else
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}% block stays a block
  }%
}%
%
\newcommand{\Hlne}{}% little hrizontal line ending a block in vline mode
%
\newcommand{\@algocf@endoption}[1]{#1}%
\newboolean{algocf@optnoend}\setboolean{algocf@optnoend}{false}%
%
\newcommand{\SetAlgoLongEnd}{%%%%%%%%%%%%%%%%%%%%%%%%% Long End
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{##1}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoShortEnd}{%%%%%%%%%%%%%%%%%%%%%%%% ShortEnd
  \setboolean{algocf@optnoend}{false}%
  \renewcommand{\@algocf@endoption}[1]{\@firstword##1 \@nil}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoEnd}{%%%%%%%%%%%%%%%%%%%%%%%%%%% NoEnd
  \setboolean{algocf@optnoend}{true}%
  \renewcommand{\@algocf@endoption}[1]{}%
  \algocf@setBlock}%
%
\newcommand{\SetAlgoNoLine}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\algocf@Noline{##1}}{##2}}%
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetAlgoVlined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Vline
\renewcommand{\algocf@@block}[2]{\algocf@Vline{##1}}%
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{\algocf@Hlne}}%
%
\newcommand{\SetAlgoLined}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Line
\renewcommand{\algocf@@block}[2]{\algocf@@@block{\strut\algocf@Vsline{##1}}{##2}}% no skip after a block so garantie at least one line
\renewcommand{\algocf@group}[1]{\algocf@Vsline{##1}}%\ifthenelse{\boolean{algocf@optnoend}}{\relax}{\strut\ignorespaces}}%
\renewcommand{\Hlne}{}}%
%
\newcommand{\SetNothing}{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Noline
\renewcommand{\algocf@@block}[2]{\algocf@Noline{##1}\par}%
%\long
\renewcommand{\algocf@group}[1]{\algocf@Noline{##1}}%
\renewcommand{\Hlne}{}}%
%
%%
%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% ``Input:'''s like command 
%
%%%
% text staying at the right of the longer keyword of KwInOut commands 
% (text of KwInOut commands are all vertically aligned)
%
\newcommand{\algocf@newinout}{\par\parindent=\inoutindent}% to put right indentation after a \\ in the KwInOut
\newcommand{\SetKwInOut}[2]{%
  \sbox\algocf@inoutbox{\KwSty{#2\algocf@typo:}}%
  \expandafter\ifx\csname InOutSizeDefined\endcsname\relax% if first time used
    \newcommand\InOutSizeDefined{}\setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
  \else% else keep the larger dimension
    \ifdim\wd\algocf@inoutbox>\inoutsize%
    \setlength{\inoutsize}{\wd\algocf@inoutbox}%
    \sbox\algocf@inoutbox{\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~}\setlength{\inoutindent}{\wd\algocf@inoutbox}%
    \fi%
  \fi% the dimension of the box is now defined.
  \algocf@newcommand{#1}[1]{%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
%     {\let\\\algocf@newinout\hangindent=\wd\algocf@inoutbox\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2}\algocf@typo\hfill:}~##1\par}%
    {\let\\\algocf@newinout\hangindent=\inoutindent\hangafter=1\parbox[t]{\inoutsize}{\KwSty{#2\algocf@typo\hfill:}}~##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
%
%% allow to ajust the skip size of InOut
%%
\newcommand{\ResetInOut}[1]{%
  \sbox\algocf@inoutbox{\hbox{\KwSty{#1\algocf@typo:}\ }}%
  \setlength{\inoutsize}{\wd\algocf@inoutbox}%
  }%
%
% 
%%%
% text staying at the right of the keyword.
%
\newcommand{\algocf@newinput}{\par\parindent=\wd\algocf@inputbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwInput}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@inputbox{\hbox{\KwSty{#2\algocf@typo:} }}%
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@seteveryparhanging{\relax}}%
    \ifthenelse{\boolean{algocf@inoutnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
    {\let\\\algocf@newinput\hangindent=\wd\algocf@inputbox\hangafter=1\unhbox\algocf@inputbox##1\par}%
    \algocf@linesnumbered% reset the numbering of the lines
    \ifthenelse{\boolean{algocf@hanginginout}}{\relax}{\algocf@reseteveryparhanging}%
  }}%
\newcommand{\SetKwData}[2]{%
  \algocf@newcommand{@#1}[1]{\DataSty{#2(}\ArgSty{##1}\DataSty{)}}%
  \algocf@newcommand{#1}{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
  }%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% tallent:
%
% Add following macros:
%   \SetKwHangingKw:  [kw] ------------   <= hanging determined by [kw]
%                          ------------
% Should act like a combination of \SetKwInput and \SetKw.
% Based on \SetKwInput:
%   - remove ':' at end of keyword
%   - do not reset numbering
%   - use separate savebox
\newsavebox{\algocf@hangingbox}
\newcommand{\algocf@newhanging}{\par\parindent=\wd\algocf@hangingbox}% to put right indentation after a \\ in the KwInput
\newcommand{\SetKwHangingKw}[2]{%
  \algocf@newcommand{#1}[1]{%
    \sbox\algocf@hangingbox{\hbox{\KwSty{#2}\algocf@typo\ }}%
    {\let\\\algocf@newhanging\hangindent=\wd\algocf@hangingbox\hangafter=1\unhbox\algocf@hangingbox##1\;}%
  }%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Comments macros
%
%%%%
% comment in the text, first argument is the name of the macro, second is
% the text put before the comment, third is the text put at the end of the
% comment.
%
% first side comment justification
\newcommand{\SetSideCommentLeft}{\setboolean{algocf@scleft}{true}}%
\newcommand{\SetSideCommentRight}{\setboolean{algocf@scleft}{false}}%
\newcommand{\SetNoFillComment}{\setboolean{algocf@optfillcomment}{false}}%
\newcommand{\SetFillComment}{\setboolean{algocf@optfillcomment}{true}}%
%
% next comment and side comment
%
\newcommand{\algocf@endmarkcomment}{\relax}%
\newcommand{\algocf@fillcomment}{%
  \ifthenelse{\boolean{algocf@optfillcomment}}{\hfill}{\relax}}%
%
\newcommand{\algocf@startcomment}{%
  \hangindent=\wd\algocf@inputbox\hangafter=1\usebox\algocf@inputbox}%
\newcommand{\algocf@endcomment}{\algocf@fillcomment\algocf@endmarkcomment\ignorespaces\par}%
\newcommand{\algocf@endstartcomment}{\algocf@endcomment\algocf@startcomment\ignorespaces}%
%
\newboolean{algocf@sidecomment}%
\newboolean{algocf@altsidecomment}\setboolean{algocf@altsidecomment}{false}%
\newcommand{\algocf@scpar}{\ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\par}}%
\newcommand{\algocf@sclfill}{\ifthenelse{\boolean{algocf@scleft}}{\algocf@fillcomment}{\relax}}%
\newcommand{\algocf@scrfill}{\ifthenelse{\boolean{algocf@scleft}}{\relax}{\hfill}}%
\newcommand{\algocf@startsidecomment}{\usebox\algocf@inputbox}%
\newcommand{\algocf@endsidecomment}{\algocf@endmarkcomment\algocf@scpar}%
\newcommand{\algocf@endstartsidecomment}{%
  \algocf@sclfill\algocf@endsidecomment%
  \algocf@scrfill\algocf@startsidecomment\ignorespaces}%
%
\newcommand{\SetKwComment}[3]{%
  \algocf@newcommand{#1}{\@ifstar{\csname algocf@#1@star\endcsname}{\csname algocf@#1\endcsname}}%
	\algocf@newcommand{algocf@#1}[1]{%
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@seteveryparhanging{\relax}}%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {\renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartcomment%
        \algocf@startcomment\CommentSty{%
          \strut\ignorespaces##1\strut\algocf@fillcomment#3}\par}%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifthenelse{\boolean{algocf@hangingcomment}}{\relax}{\algocf@reseteveryparhanging}%
    }%
  %%% side comment definitions
	\algocf@newcommand{algocf@#1@star}[2][]{%
      \ifArgumentEmpty{##1}\relax{% TODO: Is this even necessary, with all those \ifx's?
        \ifthenelse{\boolean{algocf@scleft}}{\setboolean{algocf@sidecomment}{true}}{\setboolean{algocf@sidecomment}{false}}%
        \ifx##1h\setboolean{algocf@altsidecomment}{true}\SetSideCommentLeft\fi%
        \ifx##1f\setboolean{algocf@altsidecomment}{true}\SetSideCommentRight\fi%
        \ifx##1l\setboolean{algocf@altsidecomment}{false}\SetSideCommentLeft\fi%
        \ifx##1r\setboolean{algocf@altsidecomment}{false}\SetSideCommentRight\fi%
      }%
      \sbox\algocf@inputbox{\CommentSty{\hbox{#2}}}%
      \ifthenelse{\boolean{algocf@commentsnumbered}}{\relax}{\algocf@seteveryparnl{\relax}}%
      {%
        \renewcommand{\algocf@endmarkcomment}{#3}%
        \let\\\algocf@endstartsidecomment%
        % here is the comment
        \ifthenelse{\boolean{algocf@altsidecomment}}{\relax}{\@endalgocfline\ }%
        \algocf@scrfill\algocf@startsidecomment\CommentSty{%
          \strut\ignorespaces##2\strut\algocf@sclfill#3}\algocf@scpar%
      }%
      \algocf@linesnumbered% reset the numbering of the lines
      \ifArgumentEmpty{##1}\relax{%
        \ifthenelse{\boolean{algocf@sidecomment}}{\setboolean{algocf@scleft}{true}}{\setboolean{algocf@scleft}{false}}%
        \setboolean{algocf@altsidecomment}{false}%
      }%
	}%
  }%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwProg
%
\newcommand{\SetKwProg}[4]{%\SetKwProg{Env}{Title}{is}{end} 
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\ifArgumentEmpty{#2}\relax{\ }\ProgSty{##2}\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode\@endalgocfline\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2} \ProgSty{##2}\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Kw
%
\newcommand{\SetKw}[2]{%
	\algocf@newcommand{@#1}[1]{\KwSty{#2} \ArgSty{##1}}
	\algocf@newcommand{#1}{\@ifnextchar\bgroup{\csname @#1\endcsname}{\KwSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwFunction
%
\newcommand{\SetKwFunction}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\FuncSty{#2(}\FuncArgSty{##1}\FuncSty{)}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\FuncSty{#2}\xspace}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwTab
%
\newcommand{\SetKwArray}[2]{%
%%% use of gdef since newcommand doesn't manage to define the macro when SetKwFunction is used in \algocf@caption@proc
  \expandafter\gdef\csname @#1\endcsname##1{\DataSty{#2[}\ArgSty{##1}\DataSty{]}}%
  \expandafter\gdef\csname#1\endcsname{%
    \@ifnextchar\bgroup{\csname @#1\endcsname}{\DataSty{#2}\xspace}}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% KwBlock
%
\newcommand{\SetKwBlock}[3]{%
	\algocf@newcmdside@kobe{#1}%
    {\KwSty{#2}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#3}{##3}\par}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% condition typo
%
\newcommand{\algocf@scond}{\ }
\newcommand{\algocf@econd}{\ }
\newcommand{\algocf@ucond}{}
\newcommand{\SetStartEndCondition}[3]{%
  \renewcommand{\algocf@scond}{#1}\renewcommand{\algocf@econd}{#2}\renewcommand{\algocf@ucond}{#3}}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For Switch
%
\newcommand{\SetKwSwitch}[9]{% #1=\Switch #2=\Case #3=\Other #4=switch #5=do #6=case #7=otherwise #8=endcase #9=endsw
%	\algocf@newcmdside{#1}{3}%
	\algocf@newcmdside@koif{#1}%
		{\KwSty{#4}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#9} {##4\relax}}%
%%%% Case
	\algocf@newcmdside@koif{#2}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#8}{##4\relax}}%
    %uCase
	\algocf@newcmdside{u#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##3}}%
    %lcase
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\ \relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\KwSty{#6}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#5}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
%%%% Other 
	\algocf@newcmdside@kobe{#3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##2}{#8}{##3\relax}}%
    %lOther
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\KwSty{#7} \KwSty{#5}\algocf@bgroupcode\ ##2\algocf@egroupcode}%
    %uOther
	\algocf@newcmdside{u#3}{3}{\KwSty{#7} \KwSty{#5}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@group{##2}}%
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% If macros
%
\newcommand{\SetKwIF}[8]{% #1=\If #2=\ElseIf #3=\Else #4=if #5=then #6=elseif #7=else #8=endif
% 
% common text
	\algocf@newcommand{#1@ifthen}[1]{\KwSty{#4}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#1@endif} [2]{\algocf@block{##1}{#8}{##2}}%
	\algocf@newcommand{#1@noend} [1]{\algocf@group{##1}}%
	\algocf@newcommand{#1@else}  [1]{\algocf@group{##1}\KwSty{#7}}%
	\algocf@newcommand{#2@elseif}[1]{\KwSty{#6}\algocf@scond\ArgSty{##1}\algocf@econd\KwSty{#5}}%
	\algocf@newcommand{#3@else}     {\KwSty{#7}}%
%%%% If then { } endif
	\algocf@newcmdside@koif{#1}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% If then {} else {} endif
    % first command to handle optional side comment of else (so just after first braces)
 	\algocf@newcmdside@kobe{algocf@e#1thenelse}{\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##2}{##3}}%
    % the definition of if-then-else command using command above 
	\algocf@newcmdside{e#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@else\endcsname{##3}\csname algocf@e#1thenelse\endcsname}%
    %%% leif
    \algocf@newcommand{le#1}{\@ifstar{\csname algocf@le#1star\endcsname}{\csname algocf@le#1\endcsname}}%
    \algocf@newcmdside{algocf@le#1}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\@endalgocfline\ \algocf@egroupcode\ifArgumentEmpty{##1}\relax{##1}\strut\par}%
    \algocf@newcmdside{algocf@le#1star}{4}{\csname #1@ifthen\endcsname{##2} \algocf@bgroupcode##3 \csname #3@else\endcsname\ ##4\algocf@egroupcode}%
%%%% If then 
	% \algocf@newcmdside{l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\
    % ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\csname #1@ifthen\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#1}{3}{\csname #1@ifthen\endcsname{##2}\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@noend\endcsname{##3}}%
%%%% ElseIf {} endif
	\algocf@newcmdside@koif{#2}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{ ##1}\csname #1@endif\endcsname{##3}{##4\relax}}%
%%%% ElseIf
    \algocf@newcommand{l#2}{\@ifstar{\csname algocf@l#2star\endcsname}{\csname algocf@l#2\endcsname}}%
	\algocf@newcmdside{algocf@l#2}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#2star}{3}{\csname #2@elseif\endcsname{##2}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
	\algocf@newcmdside{u#2}{3}{\csname #2@elseif\endcsname{##2}\relax\ifArgumentEmpty{##1}\relax{##1}\csname #1@noend\endcsname{##3}}%
%%%% Else {} endif
	\algocf@newcmdside@kobe{#3}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ ##1\csname #1@endif\endcsname{##2}{##3\relax}}%
%%%% Else 
    \algocf@newcommand{l#3}{\@ifstar{\csname algocf@l#3star\endcsname}{\csname algocf@l#3\endcsname}}%
	\algocf@newcmdside{algocf@l#3}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#3star}{2}{\csname #3@else\endcsname\algocf@bgroupcode\ ##2\algocf@egroupcode}%
	\algocf@newcmdside{u#3}{2}{\csname #3@else\endcsname\ifArgumentEmpty{##1}\relax\ {##1\relax}\csname #1@noend\endcsname{##2}}%
}% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% For macros
%
\newcommand{\SetKwFor}[4]{%
	\algocf@newcmdside@koif{#1}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\ifArgumentEmpty{##1}\relax{ ##1}\algocf@block{##3}{#4}{##4\relax}}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\@endalgocfline\algocf@egroupcode\ifArgumentEmpty{##1}\relax\ {##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@scond\ArgSty{##2}\algocf@econd\KwSty{#3}\algocf@bgroupcode\ ##3\algocf@egroupcode}%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Repeat macros
%
\newsavebox{\algocf@untilbox}% to handle width of until keyword needed to have good skip
  % for line numbers
\newskip\algocf@skipuntil
\newcommand{\SetKwRepeat}[3]{%
	\algocf@newcmdsides{#1}{3}{%
      \sbox\algocf@untilbox{\KwSty{#3}\algocf@scond}\algocf@skipuntil=\wd\algocf@untilbox%
      \KwSty{#2}\ifArgumentEmpty{##1}\relax{##1}\algocf@group{##3}%
      \KwSty{#3}\algocf@scond% until keyword and start condition typo
      %\advance\skiptotal by\algocf@skipuntil%
      \ArgSty{##2}%
      %\advance\skiptotal by-\algocf@skipuntil%
      \algocf@ucond%
      \algocf@skipuntil=0pt% reset counter
    }{\@endalgocfline}{\strut\par}%
    \algocf@newcommand{l#1}{\@ifstar{\csname algocf@l#1star\endcsname}{\csname algocf@l#1\endcsname}}%
	\algocf@newcmdside{algocf@l#1}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond\@endalgocfline\ifArgumentEmpty{##1}\relax{ ##1}\strut\par}%
	\algocf@newcmdside{algocf@l#1star}{3}{\KwSty{#2}\algocf@bgroupcode\ ##3\algocf@egroupcode\ \KwSty{#3}\algocf@scond\ArgSty{##2}\algocf@ucond}%
}%
%
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%        Environments definitions     %%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%
%% Caption management
%%
% for the following macros:
% #1 is given by caption and is equal to fnum@algocf
% #2 is the text given in argument by the user in the \caption macro
%
%%%%% text of caption
\newcommand{\algocf@captionlayout}[1]{#1}%
\newcommand{\SetAlgoCaptionLayout}[1]{%
  \renewcommand{\algocf@captionlayout}[1]{\csname #1\endcsname{##1}}}%
\newcommand{\algocf@capseparator}{:}%
\newcommand{\SetAlgoCaptionSeparator}[1]{\renewcommand{\algocf@capseparator}{#1}}%
\newcommand{\algocf@captiontext}[2]{%
  \algocf@captionlayout{\AlCapSty{\AlCapFnt #1\algocf@typo\algocf@capseparator}\nobreakspace%
    \AlCapNameSty{\AlCapNameFnt{}#2\endgraf}}}% text of caption
%
%%%%% default caption of algorithm: used if no specific style caption is defined
\newcommand{\algocf@makecaption}[2]{%
  \addtolength{\hsize}{\algomargin}%
  \sbox\@tempboxa{\algocf@captiontext{#1}{#2}}%
  \ifdim\wd\@tempboxa >\hsize%     % if caption is longer than a line
    \hskip .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}% then caption is not centered
  \else%
    \global\@minipagefalse%
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}% else caption is centered
  \fi%
  \addtolength{\hsize}{-\algomargin}%
}%
%
\newsavebox\algocf@capbox%
\newcommand{\algocf@makecaption@plain}[2]{%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}}%
\newcommand{\algocf@makecaption@boxed}[2]{%
  \addtolength{\hsize}{-\algomargin}%
  \global\sbox\algocf@capbox{\algocf@makecaption{#1}{#2}}%
  \addtolength{\hsize}{\algomargin}%
 }%
%
\newcommand{\algocf@makecaption@plainruled}[2]{\algocf@makecaption@plain{#1}{#2}}%
\newcommand{\algocf@makecaption@tworuled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@algoruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@boxruled}[2]{\algocf@makecaption@ruled{#1}{#2}}%
\newcommand{\algocf@makecaption@ruled}[2]{%
  \global\sbox\algocf@capbox{\hskip\AlCapHSkip% .5\algomargin%
    \parbox[t]{\hsize}{\algocf@captiontext{#1}{#2}}}% then caption is not centered
}%
%
\newlength{\algoheightruledefault}\setlength{\algoheightruledefault}{0.8pt}%
\newlength{\algoheightrule}\setlength{\algoheightrule}{\algoheightruledefault}%
\newlength{\algotitleheightruledefault}\setlength{\algotitleheightruledefault}{0.8pt}%
\newlength{\algotitleheightrule}\setlength{\algotitleheightrule}{\algotitleheightruledefault}%
\newcommand{\algocf@caption@plain}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@plainruled}{\algocf@caption@plain}%
\newcommand{\algocf@caption@boxed}{\vskip\AlCapSkip\box\algocf@capbox}%
\newcommand{\algocf@caption@ruled}{\box\algocf@capbox\kern\interspacetitleruled\hrule
  width\algocf@ruledwidth height\algotitleheightrule depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@tworuled}{\box\algocf@capbox\hrule  height0pt depth0pt\kern\interspacealgoruled}%
\newcommand{\algocf@caption@algoruled}{\algocf@caption@ruled}%
\newcommand{\algocf@caption@boxruled}{%
  \addtolength{\hsize}{-0.8pt}%
  \hbox to\hsize{%
    \vrule%\hskip-0.35pt%
    \vbox{%
      \hrule\vskip\interspacetitleboxruled%
      \hbox to\hsize{\unhbox\algocf@capbox\hfill}\vskip\interspacetitleboxruled%
    }% 
    %\hskip-0.35pt%
    \vrule%
  }\nointerlineskip%
  \addtolength{\hsize}{0.8pt}%
}%
%
%
%%%% set caption for the environment
\newcommand{\algocf@captionref}{%
  \renewcommand{\fnum@algocf}[1]{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\algocf@algocfref}}%
  \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
  \let\old@thealgocf=\thealgocf\renewcommand{\thealgocf}{{\relsize{\algocf@refrelsize}\algocf@algocfref}}%
  \gdef\@currentlabel{\algocf@algocfref}% let the label use the new ref
}%
%
% Unfortunatly, we also need our own caption to set some specific stuff for special references. But after these
% settings, we call the original caption.
%
\long\def\algocf@caption@algo#1[#2]#3{%
  \ifthenelse{\equal{\algocf@algocfref}{\relax}}{}{\algocf@captionref}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\equal{\algocf@algocfref}{\relax}}{\renewcommand{\theHalgocf}{\thealgocf}}{% take algocf as Href
      \renewcommand{\theHalgocf}{\algocf@algocfref}}%else if SetAlgoRefName done, take this name as ref.
    \hyper@refstepcounter{algocf}%set algocf as category of ref
  }%
   \algocf@latexcaption{#1}[{#2}]{{#3}}% call original caption
}%
%
% beamer define is own caption overrinding latex caption!
% as we need it, we have put here the original definition
% to handle manual ref, unfortunately we have to add one line to handle algocf@algocfref
\long\def\algocf@latexcaption#1[#2]#3{% original definition of caption
  \par%
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
  {\protect\numberline{\csname the#1\endcsname}{\ignorespaces #2}}%
  \begingroup%
  \@parboxrestore%
  \if@minipage%
    \@setminipage%
  \fi%
  \normalsize%
  \@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par%
  \endgroup%
}%
%
% \ifx\beamer@makecaption\undefined%
% \else% beamer detected
\ifx\@makecaption\undefined%
\newcommand{\@makecaption}[2]{\relax}%
\fi%
%%

%
% more and more packages redefine \@caption instead of just \@makecaption which makes algorithm2e
% caption not works since based on standard \@caption. So we force the definition of \@caption to be
% the standard one (the one from LaTeX) inside algorithm environment.
%
% unfortunately, makecaption is called with \ignorespace #3 so 
% we can't do the @currentlabel definition inside \algocf@captionproctext
\long\def\algocf@caption@proc#1[#2]#3{%
  \ifthenelse{\boolean{algocf@nokwfunc}}{\relax}{%
    \SetKwFunction{\algocf@captname#3@}{\algocf@captname#3@}%
  }%
  % we tell hyperref to use algocfproc as category and to take the appropriate ref.
  \ifthenelse{\boolean{algocf@func}}{\def\@proc@func{algocffunc}}{\def\@proc@func{algocfproc}}%
  \@ifundefined{hyper@refstepcounter}{\relax}{% if hyper@refstepcounter undefind, no hyperref, else...
    \ifthenelse{\boolean{algocf@procnumbered}}{% 
      \expandafter\def\csname theH\@proc@func\endcsname{\thealgocf}%if procnumbered, take \thealgocf as ref
    }{%
      \expandafter\def\csname theH\@proc@func\endcsname{\algocf@captname#3@}%else take procedure or function name
    }%
    \hyper@refstepcounter{\@proc@func}%
  }%
  \ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
    \addtocounter{algocf}{-1}% \caption do a refstepcounter, so we restore the precedent value
    \gdef\@currentlabel{\algocf@captname#3@}% let the label be the name of the function, not the counter
  }%
  \ifthenelse{\equal{\algocf@captparam#2@}{\arg@e}}{% if no paramater, we remove the ()
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace\algocf@captname#2@]{#3}%
  }{%                                                 else we give the complete name
    \algocf@latexcaption{#1}[\algocf@procname\nobreakspace#2]{#3}%
  }%
}%
%%
%%% setcaption
\newcommand{\algocf@setcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment, caption text must be changed
    \let\algocf@oldcaptiontext=\algocf@captiontext%
    \renewcommand{\algocf@captiontext}[2]{%
      \algocf@captionproctext{##1}{##2}%
    }%
  }{}%
  \let\algocf@savecaption=\@caption%
  \ifthenelse{\boolean{algocf@procenvironment}}{\let\@caption=\algocf@caption@proc}{\let\@caption=\algocf@caption@algo}%
  \let\algocf@oldmakecaption=\@makecaption%
  \renewcommand{\@makecaption}[2]{%
    \expandafter\csname algocf@makecaption@\algocf@style\endcsname{##1}{##2}%
  }%
}%
%
%%%%% reset caption
%
% since we have force the LaTeX caption for algorithm environment, we must go back to the caption
% used in the text.
\newcommand{\algocf@resetcaption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if proc environment
    \let\thealgocf=\old@thealgocf% restore normal counter printing
    \let\algocf@captiontext=\algocf@oldcaptiontext% restore normal caption text
  }{}%
  \let\@caption=\algocf@savecaption% now restore caption outside algo/proc/func environment
  \let\@makecaption=\algocf@oldmakecaption% and restore makecaption outside outside algo/proc/func environment
  \algocf@resetfnum%
}%
%
%%%%% nocaptionofalgo and restorecaptionofalgo --
\newcommand{\NoCaptionOfAlgo}{%
  \let\@old@algocf@captiontext=\algocf@captiontext%
  \renewcommand{\algocf@captiontext}[2]{\AlCapNameSty{\AlCapNameFnt{}##2}}%
}%
\newcommand{\RestoreCaptionOfAlgo}{%
  \let\algocf@captiontext=\@old@algocf@captiontext%
}%
%
% ----------------------  algocf environment
%
\newcounter{algocfline}%                    % new counter to make lines numbers be internally 
\setcounter{algocfline}{0}%                 % different in different algorithms
\newcounter{algocfproc}% counter to count all algo environment (proc, func), just used by hyperref to avoir "same
\setcounter{algocfproc}{0}% identifier" error caused by algocf being set to '-' for procedure or function or not
  % changed if no caption is given.
%
\expandafter\ifx\csname algocf@within\endcsname\relax% if \algocf@within doesn't exist
\newcounter{algocf}%                        % just define a new counter
\renewcommand{\thealgocf}{\@arabic\c@algocf}% and the way it is printed
\else%                                     else
\newcounter{algocf}[\algocf@within]%        % counter is numbered within \algocf@within
\renewcommand\thealgocf{\csname the\algocf@within\endcsname.\@arabic\c@algocf}%
\fi%
%
\def\fps@algocf{htbp}%        % default
\def\ftype@algocf{10}%        % float type
\def\ext@algocf{\algocf@list} % loa by default, lof if figure option used
\newcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}%
\newcommand{\algocf@resetfnum}{\renewcommand{\fnum@algocf}{\AlCapSty{\AlCapFnt\algorithmcfname\nobreakspace\thealgocf}}}%
\newenvironment{algocf}%      % float environment for algorithms
               {\@float{algocf}}%
               {\end@float}%
\newenvironment{algocf*}%     % float* environment for algorithms
               {\@dblfloat{algocf}}%
               {\end@dblfloat}%
%
\def\algocf@seclistalgo{}%
\ifx\l@chapter\undefined\let\algocf@seclistalgo=\section\else\let\algocf@seclistalgo=\chapter\fi%
\@ifundefined{if@restonecol}{\newif\if@restonecol}\relax%
\newcommand\listofalgocfs{%
     \ifx\algocf@seclistalgo\chapter%
      \if@twocolumn\@restonecoltrue\onecolumn\else\@restonecolfalse\fi%
    \fi%
     \algocf@seclistalgo*{\listalgorithmcfname}%
       \@mkboth{\MakeUppercase\listalgorithmcfname}%
               {\MakeUppercase\listalgorithmcfname}%
     \@starttoc{loa}%
    \ifx\algocf@seclistalgo\chapter%
      \if@restonecol\twocolumn\fi%
    \fi%
}
%
\newcommand*\l@algocf{\@dottedtocline{1}{1em}{2.3em}}% line of the list
%
% ----------------------  algorithm environment
%
%%%%%%%
%%
%% Algorithm environment definition
%%
%%%%%%%
%%
%
\newsavebox\algocf@algoframe%
\def\@algocf@pre@plain{\relax}%  action to be done before printing the algo.
\def\@algocf@post@plain{\relax}% action to be done after printing the algo.
\def\@algocf@capt@plain{bottom}% where the caption should be localized.
\def\@algocf@pre@boxed{\noindent\begin{lrbox}{\algocf@algoframe}}
\def\@algocf@post@boxed{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxed{under}%
\def\@algocf@pre@ruled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@ruled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@ruled{top}%
\def\@algocf@pre@algoruled{\hrule width\algocf@ruledwidth height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@algoruled{\kern\interspacealgoruled\hrule width\algocf@ruledwidth height\algoheightrule \relax}%
\def\@algocf@capt@algoruled{top}%
\def\@algocf@pre@tworuled{\hrule height\algoheightrule depth0pt\kern\interspacetitleruled}%
\def\@algocf@post@tworuled{\kern\interspacealgoruled\hrule height\algoheightrule\relax}%
\def\@algocf@capt@tworuled{top}%
\def\@algocf@pre@boxruled{\noindent\begin{lrbox}{\algocf@algoframe}}%
\def\@algocf@post@boxruled{\end{lrbox}\framebox[\hsize]{\box\algocf@algoframe}\par}%
\def\@algocf@capt@boxruled{above}%
\def\@algocf@pre@plainruled{\@algocf@pre@ruled}%  action to be done before printing the algo.
\def\@algocf@post@plainruled{\@algocf@post@ruled\kern\interspacealgoruled}%  action to be done before printing the algo.
\def\@algocf@capt@plainruled{under}%
%
\newcommand{\noalgocaption}{\def\@algocf@capt@ruled{none}}
%
%% before algocf environment (not figure environment)
\newcommand{\@algocf@init@caption}{%
  \ifthenelse{\boolean{algocf@procenvironment}}{% if we are inside a procedure/function environment
    \@algocf@proctitleofalgo% set Titleofalgo to Procedure: or Function:
                            % accordingly to the environment
    \let\old@thealgocf=\thealgocf\ifthenelse{\boolean{algocf@procnumbered}}{\relax}{%
      \renewcommand{\thealgocf}{-}}%
  }{% else inside environment algorithm
    \@algocf@algotitleofalgo% fix name for \Titleofalgo to \algorithmcfname
  }%
  \algocf@setcaption%       set caption to our caption style
}%
%
\newcommand{\@algofloatboxreset}{\@setminipage}
\newcommand{\@algocf@init}{%
  \refstepcounter{algocfline}%
  \stepcounter{algocfproc}%to have a different counter for each environment and being abble to make the difference
    %between href of algoline in different algorithms.
  \ifthenelse{\boolean{algocf@optnoend}}{%
      \renewcommand{\algocf@block}[3]{\algocf@group{##1}}%
    }{%
      \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
    }%
}%
%% after the end of algocf or figure environment
\newcommand{\@algocf@term@caption}{%
  \algocf@resetcaption% restore original caption
}%
%
\newcommand{\@algocf@term}{%
  \setboolean{algocf@algoH}{false}% no H by default
  \ifthenelse{\boolean{algocf@optnoend}}{%
    \renewcommand{\algocf@block}[3]{\algocf@@block{##1}{##2}{##3}}%
  }{%
    \renewcommand{\algocf@block}[2]{\algocf@group{##1}}%
  }%
  \SetAlgoRefName{\relax}%
}%
%
%%%%%%%%%%%%%%%%%
%% makethealgo: macro which print effectively the algo in its box
%% 
\newsavebox\algocf@algobox%
\newcommand{\algocf@makethealgo}{%
  \vtop{%
    % place caption above if needed  bye the style
    \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{above}}%
    {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    % precommand according to the style
    \csname @algocf@pre@\algocf@style\endcsname%
    % place caption at top if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{top}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    %
    \box\algocf@algobox% the algo
    % place caption at bottom if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{bottom}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
    % postcommand according to the style
    \csname @algocf@post@\algocf@style\endcsname%
    % place caption under if needed  bye the style
     \ifthenelse{\equal{\csname @algocf@capt@\algocf@style\endcsname}{under}}%
     {\csname algocf@caption@\algocf@style\endcsname}{}%
  }%
}%
%%%%%%%%%%%%%%%%%%%
%
%% at the beginning of algocf or figure environment
\newenvironment{algomathdisplay}{\[}{\@endalgocfline\]\ifthenelse{\boolean{algocf@linesnumbered}}{\nl}{\relax}}%
\newcommand{\@algocf@start}{%
  \@algoskip%
  \begin{lrbox}{\algocf@algobox}%
  \setlength{\algowidth}{\hsize}%
  \vbox\bgroup% save all the algo in a box
  \hbox to\algowidth\bgroup\hbox to \algomargin{\hfill}\vtop\bgroup%
  \ifthenelse{\boolean{algocf@slide}}{\parskip 0.5ex\color{black}}{}%
  % initialization
  \addtolength{\hsize}{-1.5\algomargin}%
  \let\@mathsemicolon=\;\def\;{\ifmmode\@mathsemicolon\else\@endalgoln\fi}%
  \raggedright\AlFnt{}%
  \ifthenelse{\boolean{algocf@slide}}{\IncMargin{\skipalgocfslide}}{}%
  \@algoinsideskip%
%   \let\@emathdisplay=\]\def\]{\algocf@endline\@emathdisplay\nl}%
}%
%
%% at the end of algocf or figure environment
\newcommand{\@algocf@finish}{%
  \@algoinsideskip%
  \egroup%end of vtop which contain all the text
  \hfill\egroup%end of hbox wich contains [margin][vtop]
  \ifthenelse{\boolean{algocf@slide}}{\DecMargin{\skipalgocfslide}}{}%
  %
  \egroup%end of main vbox
  \end{lrbox}%
  \algocf@makethealgo% print the algo
  \@algoskip%
  % restore dimension and macros
  \setlength{\hsize}{\algowidth}%
  \lineskip\normallineskip\setlength{\skiptotal}{\@defaultskiptotal}%
  \let\;=\@mathsemicolon%  
  \let\]=\@emathdisplay%
}%
%
%%%%%%%%%%%%%%%%%%%%
%% basic definition of the environment algorithm
%%
%
\newboolean{algocf@procenvironment}\setboolean{algocf@procenvironment}{false}%
\newboolean{algocf@func}\setboolean{algocf@func}{false}%
\newboolean{algocf@algoH}\setboolean{algocf@algoH}{false}%
\newboolean{algocf@algostar}\setboolean{algocf@algostar}{false}%
%
%%% environment for {algorithm}[H]
\newenvironment{algocf@Here}{\noindent%
  \def\@captype{algocf}% if not defined, caption exit with an error
  \begin{minipage}{\hsize}%
}{%
  \end{minipage}%\par%
}%
%%% real algorithm environment which manages H and * option
%    \let\algocf@originalfloatboxreset=\@floatboxreset%
%    \let\@floatboxreset=\@algofloatboxreset%
\newenvironment{algocf@algorithm}[1][htbp]{%
   \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@figurecaption}}{\captionsetup{margin={-\algomargin,\algomargin}}}{}%
   }{}%
   \@algocf@init%
   \ifthenelse{\equal{\algocf@float}{figure}}{% if option figure set
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \begin{figure*}[#1]% call figure*
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else algorithm environment with figure option
       \begin{figure}[#1]%  call figure
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
          \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }%
   }{% else normal algorithm environment
     \@algocf@init@caption%
     \ifthenelse{\equal{#1}{H}}{% if [H] algorithm
       \if@twocolumn\@latex@error{[H] in two columns mode is not allowed for algorithms}\fi% TODO: SCREAM if H in two colums!
       \setboolean{algocf@algoH}{true}\begin{algocf@Here}% call corresponding environment
         \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
         \let\algocf@oldeverypar=\everypar%
         \algocf@seteverypar%
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \begin{algocf*}[#1]% call algocf*
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }{% else algorithm environment
         \begin{algocf}[#1]%  call algcf
           \ifthenelse{\boolean{algocf@customruledwidth}}{\relax}{\setlength{\algocf@ruledwidth}{\linewidth}}%
           \let\algocf@oldeverypar=\everypar%
           \algocf@seteverypar%
       }%
     }%
   }% fin test option figure ou pas
   \@algocf@start% 
   \@ResetCounterIfNeeded%
   \algocf@linesnumbered\ignorespaces%
}{%
  \@algocf@finish%
  \ifthenelse{\equal{\algocf@float}{figure}}{%
     \ifthenelse{\boolean{algocf@algostar}}{% if algorithm* with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure*}% call figure*
     }{% else algorithm environment with figure option
       \let\everypar=\algocf@oldeverypar%
       \end{figure}%  call figure
     }%
  }{%
    \@algocf@term@caption%
    \ifthenelse{\boolean{algocf@algoH}}{% if [H] algorithm
      \let\everypar=\algocf@oldeverypar%
      \end{algocf@Here}\par% call corresponding environment
     }{% else floating algorithm environment
       \ifthenelse{\boolean{algocf@algostar}}{% if algorithm*
         \let\everypar=\algocf@oldeverypar%
         \end{algocf*}% call algocf*
       }{% else algorithm environment
         \let\everypar=\algocf@oldeverypar%
         \end{algocf}%  call algocf
       }%
     }%
  }%
  \@algocf@term\ignorespacesafterend%
}%
%
%%% user algorithm environment
\newenvironment{\algocf@envname}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%%% user algorithm* environment
\newenvironment{\algocf@envname*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{false}\gdef\algocfautorefname{\algorithmautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%%%%%%%%%%%%%%%%%%%%%%%
%%%
%
\expandafter\newcommand\csname\algocf@listofalgorithms\endcsname{%
  \ifthenelse{\equal{\algocf@float}{figure}}{\listoffigures}{\listofalgocfs}%
}%
%%%
%%%
%
% ----------------------  procedure and function environments
%
%
% -- new style (used in particular in the caption of function and procedure environments)
%
% three macros to extract parts of the caption
\gdef\algocf@captname#1(#2)#3@{#1}  % keep characters before the first brace
\gdef\algocf@captparam#1(#2)#3@{#2} % keep character in between the braces
\gdef\algocf@captother#1(#2)#3@{#3} % keep character after the braces
%
%%% Text of caption for Procedure or Function
\newcommand{\algocf@captionproctext}[2]{%
  {%
    \ProcSty{\ProcFnt\algocf@procname\ifthenelse{\boolean{algocf@procnumbered}}{\nobreakspace\thealgocf\algocf@typo\algocf@capseparator}{\relax}}%
    \nobreakspace\ProcNameSty{\ProcNameFnt\algocf@captname #2@}% Name of the procedure in ProcName Style. 
    \ifthenelse{\equal{\algocf@captparam #2@}{\arg@e}}{}{% if no argument, write nothing
      \ProcNameSty{\ProcNameFnt(}\ProcArgSty{\ProcArgFnt\algocf@captparam #2@}\ProcNameSty{\ProcNameFnt)}%else put arguments in ProcArgSty:
    }% endif
    \algocf@captother #2@%
  }%
}%
%
%
% -- procedure and function environments are defined from algocf@algorithm environment
%
\newenvironment{procedure}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function}[1][htbp]{%
  \setboolean{algocf@algostar}{false}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
\newenvironment{procedure*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{false}%
  \newcommand{\algocf@procname}{\@algocf@procname}\gdef\algocfprocautorefname{\procedureautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
\newenvironment{function*}[1][htbp]{%
  \setboolean{algocf@algostar}{true}%
  \setboolean{algocf@procenvironment}{true}\setboolean{algocf@func}{true}%
  \newcommand{\algocf@procname}{\@algocf@funcname}\gdef\algocffuncautorefname{\functionautorefname}%
  \begin{algocf@algorithm}[#1]\ignorespaces%
}{%
  \end{algocf@algorithm}\ignorespacesafterend%
}%
%
%
%%%%%%%%%%%%%%%%%%%%
%% definition of algondfloat environment
%%
\ifthenelse{\boolean{algocf@endfloat}}{% if endfloat option then
\newcommand{\algoplace}{% macro which is used to writhe algorithm about there
   \begin{center}%
     [\algorithmcfname~\thepostfig\ about here.]%
   \end{center}%
}%
\newcommand{\algoendfloat}{% use as a \begin{algoendfloat} environment to start scanning of line
%  \immediate\openout\@mainfff\jobname.fff%
  \efloat@condopen{fff}
  \efloat@iwrite{fff}{\string\begin{\algocf@envname}}%
    \if@domarkers%
       \ifthenelse{\equal{\algocf@list}{lof}}{%
         \addtocounter{postfig}{1}%
       }{%
         \addtocounter{postalgo}{1}%
       }%
       \algoplace%
    \fi%
    \bgroup%
    \let\do\ef@makeinnocent\dospecials%
    \ef@makeinnocent\^^L% and whatever other special cases
    \endlinechar`\^^M \catcode`\^^M=12 \ef@xalgocfendfloat}%
}{\relax}%%%% end of endfloat option ifthenelse
%% some macros useful for endfloat option that cannot be defined inside the ifthenelse
%scan algoendfloat algorithm and write the text into .fff file
{\catcode`\^^M=12 \endlinechar=-1 %
 \gdef\ef@xalgocfendfloat#1^^M{% scan the lines inside algoendfloat environment being read by latex
   \def\test{#1}% test is the line being currently scan by latex
   \ifx\test\ef@endalgocftest% if it is \end{algoendfloat}
     \def\next{% define next as to not continue the scan and write \end{algorithm} into .fff file
       \egroup\end{algoendfloat}%
       \efloat@iwrite{fff}{\string\end{\algocf@envname}}%
       \efloat@iwrite{fff}{\string\efloatseparator}%
       \efloat@iwrite{fff}{ }%
     }%
     \else% else write the current line being scanned by latex and set next to continue the scan
       \efloat@iwrite{fff}{#1}%
       \let\next\ef@xalgocfendfloat%
     \fi% endif
     \next}% next is continue if it was else condition, else it does not continue the scan and write end to file
}%
% test if the scan is finish by looking at the string \end{algoendfloat}
{\escapechar=-1%
 \xdef\ef@endalgocftest{\string\\end\string\{algoendfloat\string\}}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
\newcommand{\TitleOfAlgo}[1]{\@titleprefix\ 
  \TitleSty{#1}\par\smallskip}%
%
\newcommand{\SetAlgorithmName}[3]{%
  \renewcommand{\listalgorithmcfname}{#3}%
  \renewcommand{\algorithmcfname}{#1}%
  \renewcommand{\algorithmautorefname}{#2}%
}%
%
\newcommand{\algocf@refrelsize}{-2}\newcommand{\SetAlgoRefRelativeSize}[1]{\renewcommand{\algocf@refrelsize}{#1}}%
\newcommand{\SetAlgoRefName}[1]{%
  \renewcommand{\algocf@algocfref}{#1}%
}%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 
% -------------------------   Default Definitions
%
%%
%%
%
\SetKwComment{tcc}{/* }{ */}%
\SetKwComment{tcp}{// }{}%
%
%\newcommand{\algocf@defaults@common}{
%
%
% english keywords (default)
%
\SetKwHangingKw{KwHData}{Data$\rightarrow$}
\SetKwInput{KwIn}{Input}%
\SetKwInput{KwOut}{Output}%
\SetKwInput{KwData}{Data}%
\SetKwInput{KwResult}{Result}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
%
% French keywords
%
\ifthenelse{\boolean{algocf@localkw@french}\OR\equal{\algocf@languagechoosen}{french}}{%
%\SetKwInOut{AlgDonnees}{Donn\'ees}\SetKwInOut{AlgRes}{R\'esultat}
\SetKwHangingKw{HDonnees}{Donnees$\rightarrow$}
\SetKwInput{Donnees}{Donn\'ees}%
\SetKwInput{Res}{R\'esultat}%
\SetKwInput{Entree}{Entr\'ees}%
\SetKwInput{Sortie}{Sorties}%
\SetKw{KwA}{\`a}%
\SetKw{Retour}{retourner}%
\SetKwBlock{Deb}{d\'ebut}{fin}%
\SetKwRepeat{Repeter}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{Si}{SinonSi}{Sinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Suivant}{Cas}{Autre}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{Pour}{pour}{faire}{fin pour}%
\SetKwFor{PourPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{PourCh}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{PourTous}{pour tous les}{faire}{fin pour tous}%
\SetKwFor{Tq}{tant que}{faire}{fin tq}%
}{}%
%
% --- German keywords
%
\ifthenelse{\boolean{algocf@localkw@german}\OR\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{Ein}{Eingabe}%KwIn
\SetKwInput{Aus}{Ausgabe}%KwOut
\SetKwInput{Daten}{Daten}%KwData
\SetKwInput{Ergebnis}{Ergebnis}%KwResult
\SetKw{Bis}{bis}%KwTo
\SetKw{KwZurueck}{zur\"uck}%KwRet
\SetKw{Zurueck}{zur\"uck}%Return
\SetKwBlock{Beginn}{Beginn}{Ende}%Begin
\SetKwRepeat{Wiederh}{wiederhole}{bis}%Repeat
%
\SetKwIF{Wenn}{SonstWenn}{Sonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Unterscheide}{Fall}{Anderes}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{Fuer}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{FuerPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{FuerJedes}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{FuerAlle}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{Solange}{solange}{tue}{Ende solange}%While
}{}%
%
% --- Czech keywords
%
\ifthenelse{\boolean{algocf@localkw@czech}\OR\equal{\algocf@languagechoosen}{czech}}{%
\SetKwInput{Vst}{Vstup}%
\SetKwInput{Vyst}{V\'{y}stup}%
\SetKwInput{Vysl}{V\'{y}sledek}%
}{}%
%
% --- Portuguese keywords
%
\ifthenelse{\boolean{algocf@localkw@portuguese}\OR\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{Entrada}{Entrada}%
\SetKwInput{Saida}{Sa\'{i}da}%
\SetKwInput{Dados}{Dados}%
\SetKwInput{Resultado}{Resultado}%
\SetKw{Ate}{at\'{e}}
\SetKw{KwRetorna}{retorna}%
\SetKw{Retorna}{retorna}%
\SetKwBlock{Inicio}{in\'{i}cio}{fim}%
\SetKwRepeat{Repita}{repita}{at\'{e}}%
%
\SetKwIF{Se}{SenaoSe}{Senao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Selec}{Caso}{Outro}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{Para}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ParaPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ParaCada}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ParaTodo}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{Enqto}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
%
% --- Italian keywords
%
\ifthenelse{\boolean{algocf@localkw@italiano}\OR\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIng}{Ingresso}%
\SetKwInput{KwUsc}{Uscita}%
\SetKwInput{KwDati}{Dati}%
\SetKwInput{KwRisult}{Risultato}%
\SetKw{KwA}{a}%
\SetKw{KwRitorna}{ritorna}%
\SetKw{Ritorna}{ritorna}%
\SetKwBlock{Inizio}{inizio}{fine}%
\SetKwRepeat{Ripeti}{ripeti}{finch\'e}%
%
\SetKwIF{Sea}{AltSe}{Altrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{Per}{per}{fai}{fine per}%
\SetKwFor{PerPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{PerCiascun}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{PerTutti}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{Finche}{finch\'e}{fai}{fine finch\'e}%
}{}%
%
% --- Spanish keywords
%
\ifthenelse{\boolean{algocf@localkw@spanish}\OR\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{Datos}{Datos}
\SetKwInput{Resultado}{Resultado}
\SetKwInput{Entrada}{Entrada}
\SetKwInput{Salida}{Salida}
\SetKw{KwA}{a}
\SetKw{KwDevolver}{devolver}
\SetKw{Devolver}{devolver}
\SetKwBlock{Inicio}{inicio}{fin}
\SetKwIF{SSi}{EnOtroCasoSi}{EnOtroCaso}{si}{entonces}{sin\'o, si}{sin\'o}{fin si}
\SetKwSwitch{Seleccionar}{Caso}{Otro}{seleccionar}{hacer}{caso}{sin\'o}{fin caso}{fin seleccionar}
\SetKwFor{Para}{para}{hacer}{fin para}
\SetKwFor{ParaPara}{par}{hacer en paralelo}{fin para}
\SetKwFor{EnParalelo}{para}{hacer en paralelo}{fin para}
\SetKwFor{Mientras}{mientras}{hacer}{fin mientras}
\SetKwFor{ParaCada}{para cada}{hacer}{fin para cada}
\SetKwFor{ParaTodo}{para todo}{hacer}{fin para todo}
\SetKwRepeat{Repetir}{repetir}{hasta que}
}{}%
%
% Croatian keywords
%
\ifthenelse{\boolean{algocf@localkw@croatian}\OR\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwUlaz}{Ulaz}%KwIn
\SetKwInput{KwIzlaz}{Izlaz}%KwOut
\SetKwInput{KwPodaci}{Podaci}%KwData
\SetKwInput{KwRezultat}{Rezultat}%KwResult
\SetKw{KwDo}{do}%KwTo
\SetKw{KwVrati}{vrati}%KwRet
\SetKw{Vrati}{vrati}%Return
\SetKwBlock{Pocetak}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Ponavljaj}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{Ako}{InaceAko}{Inace}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Granaj}{Slucaj}{OstaliSlucajevi}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{Za}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ZaPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ZaSvaki}{za svaki}{\v{c}ini}{kraj za svaki}%mForEach
\SetKwFor{ZaSvaku}{za svaku}{\v{c}ini}{kraj za svaku}%fForEach
\SetKwFor{ZaSvako}{za svako}{\v{c}ini}{kraj za svako}%nForEach
\SetKwFor{ZaSve}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{Dok}{dok}{\v{c}ini}{kraj dok}%While
}{}%

%
% --- Turkish keywords
%
\ifthenelse{\boolean{algocf@localkw@turkish}\OR\equal{\algocf@languagechoosen}{turkish}}{%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
% %
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
% --- End 
%}
%
%\algocf@defaults@common
%
% option onelanguage redefinition
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{french}}{%
\SetKwInput{KwIn}{Entr\'ees}%
\SetKwInput{KwOutSortie}{Sorties}%
\SetKwInput{KwData}{Donn\'ees}%
\SetKwInput{KwResult}{R\'esultat}%
\SetKw{KwTo}{\`a}%
\SetKw{KwRet}{retourner}%
\SetKw{Return}{retourner}%
\SetKwBlock{Begin}{d\'ebut}{fin}%
\SetKwRepeat{Repeat}{r\'ep\'eter}{jusqu'\`a}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwSwitch{Switch}{Case}{Other}{suivant}{faire}{cas o\`u}{autres cas}{fin cas}{fin d'alternative}%
\SetKwFor{For}{pour}{faire}{fin pour}%
\SetKwFor{ForPar}{pour}{faire en parall\`ele}{fin pour}%
\SetKwFor{ForEach}{pour chaque}{faire}{fin pour chaque}%
\SetKwFor{ForAll}{pour tous}{faire}{fin pour tous}%
\SetKwFor{While}{tant que}{faire}{fin tq}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{german}}{%
\SetKwInput{KwIn}{Eingabe}%KwIn
\SetKwInput{KwOut}{Ausgabe}%KwOut
\SetKwInput{KwData}{Daten}%KwData
\SetKwInput{KwResult}{Ergebnis}%KwResult
\SetKw{KwTo}{bis}%KwTo
\SetKw{KwRet}{zur\"uck}%KwRet
\SetKw{Return}{zur\"uck}%Return
\SetKwBlock{Begin}{Beginn}{Ende}%Begin
\SetKwRepeat{Repeat}{wiederhole}{bis}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwSwitch{Switch}{Case}{Other}{unterscheide}{tue}{Fall}{sonst}{Ende Fall}{Ende Unt.}%Switch
\SetKwFor{For}{f\"ur}{tue}{Ende f\"ur}%For
\SetKwFor{ForPar}{f\"ur}{tue gleichzeitig}{Ende gleichzeitig}%ForPar
\SetKwFor{ForEach}{f\"ur jedes}{tue}{Ende f\"ur}%ForEach
\SetKwFor{ForAll}{f\"ur alle}{tue}{Ende f\"ur}%ForAll
\SetKwFor{While}{solange}{tue}{Ende solange}%While
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{portuguese}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Sa\'{i}da}%
\SetKwInput{KwData}{Dados}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{at\'{e}}
\SetKw{KwRet}{retorna}%
\SetKw{Return}{retorna}%
\SetKwBlock{Begin}{in\'{i}cio}{fim}%
\SetKwRepeat{Repeat}{repita}{at\'{e}}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwSwitch{Switch}{Case}{Other}{selecione}{fa\c{c}a}{caso}{sen\~{a}o}{fim caso}{fim selec}%
\SetKwFor{For}{para}{fa\c{c}a}{fim para}%
\SetKwFor{ForPar}{para}{fa\c{c}a em paralelo}{fim para}
\SetKwFor{ForEach}{para cada}{fa\c{c}a}{fim para cada}%
\SetKwFor{ForAll}{para todo}{fa\c{c}a}{fim para todo}%
\SetKwFor{While}{enquanto}{fa\c{c}a}{fim enqto}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{italiano}}{%
\SetKwInput{KwIn}{Ingresso}%
\SetKwInput{KwOut}{Uscita}%
\SetKwInput{KwData}{Dati}%
\SetKwInput{KwResult}{Risultato}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{ritorna}%
\SetKw{Return}{ritorna}%
\SetKwBlock{Begin}{inizio}{fine}%
\SetKwRepeat{Repeat}{ripeti}{finch\'e}%
%
\SetKwIF{If}{ElseIf}{Else}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end case}{endsw}%
\SetKwFor{For}{per}{fai}{fine per}%
\SetKwFor{ForPar}{per}{fai in parallelo}{fine per}%
\SetKwFor{ForEach}{per ciascun}{fai}{fine per ciascun}%
\SetKwFor{ForAll}{per tutti i}{fai}{fine per tutti}%
\SetKwFor{While}{finch\'e}{fai}{fine finch\'e}%
}{}%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{spanish}}{%
\SetKwInput{KwIn}{Entrada}%
\SetKwInput{KwOut}{Salida}%
\SetKwInput{KwData}{Datos}%
\SetKwInput{KwResult}{Resultado}%
\SetKw{KwTo}{a}%
\SetKw{KwRet}{devolver}%
\SetKw{Return}{devolver}%
\SetKwBlock{Begin}{inicio}{fin}%
\SetKwRepeat{Repeat}{repetir}{hasta que}%
%
\SetKwIF{If}{ElseIf}{Else}{si}{entonces}{si no, si}{en otro caso}{fin si}
\SetKwSwitch{Switch}{Case}{Other}{seleccionar}{hacer}{caso}{si no}{fin caso}{fin seleccionar}
\SetKwFor{For}{para}{hacer}{fin para}%
\SetKwFor{ForPar}{para}{hacer in paralelo}{fin para}%
\SetKwFor{ForEach}{para cada}{hacer}{fin para cada}
\SetKwFor{ForAll}{para todo}{hacer}{fin para todo}
\SetKwFor{While}{mientras}{hacer}{fin mientras}
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{croatian}}{%
\SetKwInput{KwIn}{Ulaz}%KwIn
\SetKwInput{KwOut}{Izlaz}%KwOut
\SetKwInput{KwData}{Podaci}%KwData
\SetKwInput{KwResult}{Rezultat}%KwResult
\SetKw{KwTo}{do}%KwTo
\SetKw{KwRet}{vrati}%KwRet
\SetKw{Return}{vrati}%Return
\SetKwBlock{Begin}{po\v{c}etak}{kraj}%Begin
\SetKwRepeat{Repeat}{ponavljaj}{dok ne bude}%Repeat
%
\SetKwIF{If}{ElseIf}{Else}{ako}{onda}{ina\v{c}e ako}{ina\v{c}e}{kraj ako}%gIf
\SetKwSwitch{Switch}{Case}{Other}{granaj}{\v{c}ini}{slu\v{c}aj}{ostali slu\v{c}ajevi}{kraj slu\v{c}aj}{kraj granaj}%Switch
\SetKwFor{For}{za}{\v{c}ini}{kraj za}%For
\SetKwFor{ForPar}{za}{\v{c}ini paralelno}{kraj za paralelno}%ForPar
\SetKwFor{ForEach}{za svaki}{\v{c}ini}{kraj za svaki}%ForEach
\SetKwFor{ForAll}{za sve}{\v{c}ini}{kraj za sve}%ForAll
\SetKwFor{While}{dok}{\v{c}ini}{kraj dok}%While
}{}%
%
\ifthenelse{\boolean{algocf@optonelanguage}\AND\equal{\algocf@languagechoosen}{turkish}}{%
%
\SetKwInput{KwIn}{Girdi}%
\SetKwInput{KwOut}{\c{C}{\i}kt{\i}}%
\SetKwInput{KwData}{Veri}%
\SetKwInput{KwResult}{Sonu\c{c}}%
\SetKw{KwTo}{to}
\SetKw{KwRet}{return}%
\SetKw{Return}{return}%
\SetKwBlock{Begin}{begin}{end}%
\SetKwRepeat{Repeat}{repeat}{until}%
%
\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{end if}%
\SetKwSwitch{Switch}{Case}{Other}{switch}{do}{case}{otherwise}{end switch}%
\SetKwFor{For}{for}{do}{end for}%
\SetKwFor{ForPar}{for}{do in parallel}{end forpar}
\SetKwFor{ForEach}{foreach}{do}{end foreach}%
\SetKwFor{ForAll}{forall}{do}{end forall}%
\SetKwFor{While}{while}{do}{end while}%
}{}%
%
%
%%%% old commands compatibility
%
\ifthenelse{\boolean{algocf@oldcommands}}{%
\newcommand{\SetNoLine}{\SetAlgoNoLine}%
\newcommand{\SetNoline}{\SetAlgoNoLine}%
\newcommand{\SetVline}{\SetAlgoVlined}%
\newcommand{\SetLine}{\SetAlgoLined}%
%
\newcommand{\dontprintsemicolon}{\DontPrintSemicolon}%
\newcommand{\printsemicolon}{\PrintSemicolon}%
\newcommand{\incmargin}[1]{\IncMargin{#1}}%
\newcommand{\decmargin}[1]{\DecMargin{-#1}}%
\newcommand{\setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\Setnlskip}[1]{\SetNlSkip{#1}}%
\newcommand{\setalcapskip}[1]{\SetAlCapSkip{#1}}%
\newcommand{\setalcaphskip}[1]{\SetAlCapHSkip{#1}}%
\newcommand{\nlSty}[1]{\NlSty{#1}}%
\newcommand{\Setnlsty}[3]{\SetNlSty{#1}{#2}{#3}}%
\newcommand{\linesnumbered}{\LinesNumbered}%
\newcommand{\linesnotnumbered}{\LinesNotNumbered}%
\newcommand{\linesnumberedhidden}{\LinesNumberedHidden}%
\newcommand{\showln}{\ShowLn}%
\newcommand{\showlnlabel}[1]{\ShowLnLabel{#1}}%
\newcommand{\nocaptionofalgo}{\NoCaptionOfAlgo}%
\newcommand{\restorecaptionofalgo}{\RestoreCaptionOfAlgo}%
\newcommand{\restylealgo}[1]{\RestyleAlgo{#1}}%
%
\newcommand{\Titleofalgo}[1]{\TitleOfAlgo{#1}}%
% \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
\newcommand{\SetKwIf}[6]{\SetKwIF{#1}{#2#1}{#2}{#3}{#4}{#5 #1}{#5}{#6}}
%
\SetKwIF{gSi}{gSinonSi}{gSinon}{si}{alors}{sinon si}{sinon}{fin si}%
\SetKwIF{gIf}{gElsIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gIf}{gElseIf}{gElse}{if}{then}{else if}{else}{end if}%
\SetKwIF{gWenn}{gSonstWenn}{gSonst}{wenn}{dann}{sonst wenn}{sonst}{Ende wenn}%gIf
\SetKwIF{gSe}{gSenaoSe}{gSenao}{se}{ent\~{a}o}{sen\~{a}o se}{sen\~{a}o}{fim se}%
\SetKwIF{gSea}{gAltSe}{gAltrimenti}{se}{allora}{altrimenti se}{allora}{fine se}%
\SetKw{Ret}{return}%
\SetKwInput{Data}{Data}%
\SetKwInput{Result}{Result}%
}{%
  \relax%
}%
%
%
%
%%
%%%
%%%% END

==> files/Intro.tex <==
\IEEEPARstart{M}{otion} planning is a fundamental problem in robotics that has garnered considerable research attention over the years. This problem traditionally involves generating robot trajectories that reach a goal configuration from an initial one, while avoiding obstacles \cite{lavalle2006planning}. To address this challenge, several planning algorithms have been proposed, including potential fields and navigation functions \cite{koditschek1990robot,loizou2017navigation,loizou2022mobile,paternain2017navigation}, search-based methods \cite{koenig2006new,sun2008generalized}, and sampling-based approaches \cite{karaman2011sampling,kavraki1996probabilistic,lavalle2001randomized}. A comprehensive literature review can be found in \cite{garrett2021integrated,antonyshyn2023multiple,matni2024towards}. 

More recently, new planning approaches have been proposed that can handle a richer class of tasks, than the classical reach-avoid tasks, and can capture temporal and logical requirements. Such tasks include surveillance \cite{leahy2016persistent}, coverage \cite{fainekos2005temporal}, data-gathering \cite{guo2017distributed}, and intermittent connectivity \cite{kantaros2016distributedInterm} and can be captured using formal languages, such as Linear
Temporal Logic (LTL) \cite{baier2008principles}.
Task and motion planning algorithms for LTL-encoded requirements are presented in \cite{kloetzer2008fully, fainekos2005hybrid, smith2011optimal, chen2012formal, vasile2013sampling, luo2021abstraction, tumova2016multi, shoukry2017linear, kantaros2020stylus, gujarathi2022mt,chen2024fast,Cardona2024Planning,kurtz2023temporal,liu2024nngtl,luo2024decomposition} assuming robot teams with known dynamics operating known environments. These works have been extended recently to handle unknown static environments \cite{guo2013revising,guo2015multi,maly2013iterative,livingston2012backtracking,livingston2013patching,kantaros2020reactive,Kantaros2022perception}, unknown dynamic environments \cite{Kalluraya2023multi,li2022online,purohit2021dt,maity2015motion,li2021safe} and uncertain robot dynamics \cite{hasanbeig2019reinforcement,sun2022neurosymbolic,kantaros2022accelerated,guo2023hierarchical,guo2018probabilistic}.
However, these works lack reactivity to unexpected failures of robot capabilities that may occur unexpectedly during mission execution  due to e.g., inclement weather, human interventions, system component malfunctions, or adversarial attacks \cite{schlotfeldt2021resilient,notomista2021resilient,ramachandran2023resilient}.


This paper aims to address this challenge by proposing a reactive-to-failures planning algorithm for multi-robot systems with collaborative LTL tasks. Specifically, we consider robots that are heterogeneous with respect to their skills which may include e.g., mobility, sensing, or manipulation. The robots are responsible for accomplishing a high-level collaborative mission, expressed as an LTL formula, requiring them to apply their capabilities at certain areas/objects. We consider cases where failures that include permanent loss of capabilities (e.g., grasping) or complete removal of robots (e.g., due to battery draining) may occur unexpectedly at any time during deployment. 

Our objective is to design reactive multi-robot plans, defined as sequences of robot states and actions, that can adapt to these failures. 
To tackle this task planning problem, we propose a joint
task re-allocation and re-planning framework. 
First, when failures occur, the task re-allocation algorithm assigns robots to new sub-tasks based on their remaining functional capabilities. A key challenge is that mission completion may no longer be possible due to the limited number of functioning robots. 
Instead of reporting mission failure, the proposed method strategically prioritizes re-allocating the most crucial sub-tasks to robots with the required functioning skills, as per user-specified priorities.  
\textcolor{black}{Second, we introduce a planner that revises the current team paths to accommodate these new task assignments while minimally violating the LTL-encoded mission specification.
The proposed algorithm aims to minimally disrupt the team behavior by performing the fewest possible task re-assignments and locally  revising the team paths to accommodate the robot failures and the task re-allocations, all while ensuring minimal mission violations.} We demonstrate the efficiency of the proposed method through extensive comparative simulations and hardware experiments.




\textbf{Related works:} 
(i) \textit{Task assignment} methods for LTL-encoded missions have been proposed in \cite{schillinger2016decomposition,banks2020multi,Luo2022temporal, Li2023Fast,chen2024distributed,liu2022time,fang2024continuous}. These works perform task assignment offline and do not consider robot failures. In case of failures, these approaches could be employed online to globally re-allocate tasks to the robots and, consequently, globally re-plan; \textcolor{black}{however, this is impractical and, possibly, unnecessary especially for small number of failures relative to the team size.} Furthermore, they cannot
handle cases where there is not enough number of surviving
robots to take over the subtasks and, therefore, they cannot generate minimum violation solutions.
(ii) Related are also the works on \textit{minimum-violation temporal logic planning} 
\cite{tumova2016Least,lahijanian2016iterative,lahijanian2016specification,Vasile2017Minimum,cai2023learning}.
These works design single-robot paths - without considering failures of robot skills - that minimally violate temporal logic specifications in the presence of timing and environmental constraints, or exogenous disturbances that may render certain mission components hard or impossible to satisfy. In contrast, this paper focuses on designing minimum-violation multi-robot paths in the presence of failures of individual robot capabilities.
(iii) The closest works to this paper are presented in \cite{Feifei2022failure,Faruq2018Simultaneous,Zhou2022Reactive,kalluraya2023resilient} that propose \textit{multi-robot planners that adapt to unexpected robot failures}. Specifically, \cite{Feifei2022failure,Faruq2018Simultaneous} consider homogeneous robots and build a product automaton modeling the multi-robot state space, the specification space, as well as possible robot failures. Using this product system, reactive control strategies are constructed. Nevertheless, product-based methods lack scalability with respect to the number of robots, the size of the environment, task complexity, and number of failures. 
While \cite{Zhou2022Reactive} addresses heterogeneous robots that react locally to environmental and robot state changes, that approach necessitates global task re-allocation and re-planning across a team automaton. This limitation is addressed in our prior work \cite{kalluraya2023resilient} by proposing a local task re-allocation and re-planning framework. A common assumption in these works is that the mission remains feasible despite robot failures, which may not always hold in practice due to limited number of functioning robots. If the mission becomes infeasible, then these planners, unlike the proposed one, return a mission failure message. Building upon our prior work \cite{kalluraya2023resilient}, this paper aims to address this limitation by proposing a planner that computes minimum mission violation plans. 
\textcolor{black}{Specifically, we extend \cite{kalluraya2023resilient} in the following ways. First, we augment the task re-allocation method from \cite{kalluraya2023resilient} by incorporating a mission violation cost function to handle cases where the mission becomes infeasible due to failures. Second, we develop a novel re-planning algorithm capable of `locally' revising the paths, ensuring that the new plans minimally violate the mission specification.
The re-planner in \cite{kalluraya2023resilient} assumes the LTL task remains feasible, and therefore, cannot straightforwardly handle infeasible missions. 
Third, we provide minimum-violation guarantees regarding the resulting task allocation and team plan that do not exist in \cite{kalluraya2023resilient}.} 

\textbf{Contributions:}
\textit{First}, we formulate a new reactive temporal logic planning problem for heterogeneous robot teams in the presence of robot failures that may render an assigned LTL-encoded collaborative mission infeasible. 
\textit{Second}, we propose a reactive algorithm that can adapt to unexpected robot failures while generating least-violating plans when mission completion is not possible. 
\textit{Third}, our algorithm prioritizes minimal disruption of the original plan in the event of failures, eliminating the need for global re-assignment or re-planning. \textit{Fourth}, we provide theoretical conditions under which the proposed framework computes the minimum-violation task allocation and team plan.
\textit{Fifth}, we provide \textcolor{black}{numerical and hardware experiments} validating the efficiency of our algorithm. 



==> files/PF_ICRA.tex <==
\subsection{Modeling of Robots and Environment}\label{sec:PFmodelRobot}
\textcolor{blue}{Consider a team of $N$ mobile robots collected in a set $R = \{rob_j | j\in\{1,\dots,N\}\}$, governed by the following dynamics:\footnote{\textcolor{red}{I believe we discussed this before. You are using two representations for the same thing. You define robots as $R = [rob_1,\dots,rob_n]$ and $j\in\{1,\dots,N\}$. Which one will you use later? Also is $n$ the same as $N$? You also use $n$ to denote the dimension of the state $\bbp_j$. Make sure the notations are consistent.}\textcolor{blue}{fixed}} 
\begin{equation}\label{eq:rdynamics}
\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))
\end{equation}}
% Consider a team of $N$ mobile robots collected in a set $R = [rob_1,\dots,rob_n]$, governed by the following dynamics: $\bbp_{j}(t+1)=\bbf_j(\bbp_{j}(t),\bbu_{j}(t))$, for all $j\in\{1,\dots,N\}$,\footnote{\textcolor{red}{I believe we discussed this before. You are using two representations for the same thing. You define robots as $R = [rob_1,\dots,rob_n]$ and $j\in\{1,\dots,N\}$. Which one will you use later? Also is $n$ the same as $N$? You also use $n$ to denote the dimension of the state $\bbp_j$. Make sure the notations are consistent.}}
where $\bbp_{j}(t)\in\mathbb{R}^n$ stands for the state (e.g., position and orientation) of robot $j$ in the free space $\Omega$ at discrete time $t$, $\bbu_{j}(t) \in\mathit{U}_j$ stands for a control input selected from a space of admissible controls $\mathit{U}_j$. 
For simplicity, we also denote $\bbp_{j}(t)\in\Omega$. Hereafter, we compactly denote the dynamics of all robots as
\footnote{\textcolor{red}{Do you use the following notation anywhere? If not, no need to be defined.}\textcolor{blue}{removed definition of $\bbp(t+1)=\bbf(\bbp(t),\bbu(t))$,  but keeping at least one definition of  single robot model as it is given in the problem statement}} %$\bbp(t+1)=\bbf(\bbp(t),\bbu(t))$,
% \begin{equation}\label{eq:rdynamics}
% \bbp(t+1)=\bbf(\bbp(t),\bbu(t))
% \end{equation}
% where $\bbp(t)\in \Omega^N$, $\forall t\geq 0$, and $\bbu(t)\in\mathit{U}:=\mathit{U}_1\times\dots\times\mathit{U}_N$.
\footnote{\textcolor{red}{Do you use anywhere this set of control inputs? If not, delete it.}\textcolor{blue}{removed definition of $\bbu(t)\in\mathit{U}:=\mathit{U}_1\times\dots\times\mathit{U}_N$}} 

The robots operate in an environment that has a known geometric structure, such as walls, as well as a known metric structure. The robots know the obstacle-free space ($\Omega_{\text{free}}$) which is cluttered with more than zero ($M>0$) regions of interest that are static and are labeled as landmarks ($\ell_i$). The known geometric structure are defined as obstacles $o_i$, $o_i\notin\Omega_{\text{free}}$. The landmarks and obstacles together create a map ($\ccalM$). Each landmark ($\ell_i$) is defined by its position ($\bbx_i$). 
% The map distribution is represented by parameters ($\bbx_i$, $c_i$), where $\bbx_i$ is the coordinates of landmark $\ell_i$, and $c_i$ is a discrete distribution determined by $d_i$. 
These values are specified initially as the environment is either previously known or information has been previously gathered using SLAM algorithms. We assume that the robots have access to the true landmark positions. 

The robots are assumed to have the necessary sensors (e.g., cameras) for perceiving the environment and enabling them to do their tasks at the various landmarks in the environment. The robots are also equipped with sensors (e.g., cameras or LiDARs) to localize themselves in the environment.  

\subsection{Robot abilities and Teams}\label{sec:abilities_def}
We define an ability as a robot's skill to complete a certain task. For example, abilities of a drone can be to take photos enabled by a camera mounted onboard, or ground robot may have the ability to lift a package enabled by robotic arms mounted on it. Furthermore, depending on the application, these $N$ robots can be heterogeneous, that is, all $N$ robots need not be of the same type nor need to have common abilities.  

The robots have collectively $z$ number of abilities amongst themselves. Each ability is represented by $\varkappa_q$, where $q\in\{1,\dots,z\}$. 
We define robot ability list $\bbZ=[\zeta_{\varkappa_1},\dots,\zeta_{\varkappa_z}]$, where $\zeta_{\varkappa_q}$ is a binary variable that denotes if the ability is active or not. 
$\bbZ$ captures all possible actions/abilities a robot can or cannot do in the environment. Each robot $rob_j$ is assigned a robot ability list $\bbZ_j$, wherein the values of $\zeta_{\varkappa_q}$ are set to 1 if $rob_j$ has the ability $\varkappa_q$ or is set to 0 if it lacks the ability.\footnote{\textcolor{red}{this notation is not clear. $\zeta_{\varkappa_q}$ was previously defined as a skill (e.g., sensing). Now it is defined as a binary variable. This needs to become clear. Maybe the skill is denoted by $q$ and $\zeta_{\varkappa_q}$ is a binary variable denoting whether you have this skill or not?}\textcolor{blue}{fixed. $\varkappa_q$ represents the skill and $\zeta_{\varkappa_q}$ represents the binary variable}} In our problem setup, $\bbZ_j$ can change with time (refer Sec \ref{sec:failure_def}) and thus $\bbZ_j(t)$ keeps track of the robot's abilities as the mission progresses. 
Each robot is equipped with a health monitoring system that allows it to keep track of its own active and inactive abilities, that is, each robot $rob_j$ has access to and can update $\bbZ_j(t)$. Furthermore, each robot communicates $\bbZ_j(t)$ with the central planner, thus allowing the planner to know the condition of all robots at time $t$.
For future notation $\bbZ_j[q](t)$ refers to '$\zeta_{\varkappa_q}$' of robot $j$ at time $t$.

We define robot teams over each individual abilities.
A robot team $\bbT_q$ at time $t$ is defined as the set of all robots which have the ability $\varkappa_q$ at time $t$. In other words, all robots belonging to team $\bbT_q(t)$ can accomplish tasks that need ability $\varkappa_q$.
\begin{equation}\label{eq:rteams}
\bbT_q(t)=\{rob_j | rob_j\in\bbR, \bbZ_j[q](t) = 1 \}
\end{equation}
By definition, a robot will be part of all the teams corresponding to the abilities it has.  Since there are $z$ abilities in total amongst all the robots, there will be $z$ teams, one for each ability. For future reference, $\bbT(t)$ represents all the teams present at time $t$.



% Furthermore the robots are split into $k$ teams. Each team $K_k$, has $N_k$ robots, and $N_1+\dots+N_k=N$. We define a team as the set of robots that have the same abilities $Z_j$. For example drones form one team and ground robots form another team. If a robot fails/loses a particular ability it's $Z_j$ will be different from its team. So we can say team is set of robots that have same abilities at beginning of mission.
% \textcolor{red}{Current algorithm finds the first robot in the tree that can do the replacement and this robot may not necessarily belong to the team. So do we skip the definition of teams? or we can say that user can decide whether tree should search till team member is found or 1st robot is found.}




% \subsection{Robot monitoring and communication between robots}\label{sec:perception}
% Each robot has a health monitoring system that keeps track of its various abilities and subsystems. If for some reason a system fails on the robot causing the

% allows it to know the status of various subsystems of the robot. Knowledge of this status allows the robot to determine if any of its abilities have failed (refer Section \ref{sec:abilities_def} and Section \ref{sec:failure_def}). This status is communicated to the central planner.


% The robots have sensors (e.g., cameras) that allow them to collect measurements related to the positions of landmarks $\bbx$. This is done using a linear observation model, which is represented as $\bby_j(t) = \bbM_j(\bbp_j(t))\bbx$, where $\bby_j(t)$ is the measurement signal taken by robot $j$ at time $t$ from the set of robots $\ccalN$. 
% The observations made by all robots at a given time $t$ are compactly represented as $\bby(t) = \bbM(\bbp(t))\bbx$. $\bbM$ is a diagonal matrix with each block on the diagonal corresponding to the observations made by a specific robot. 
% The robot also uses its sensors to localize itself in the environment and thus knows its position $\bbp_j(t)$.




\subsection{LTL missions}\label{sec:PFLTLMission}
The goal of the robots is to accomplish a complex collaborative mission captured by a global co-safe Linear Temporal Logic (LTL) specification $\phi$. \textcolor{blue}{In order to meet LTL objectives, infinite paths can be used, but these are usually transformed into a finite representation called prefix-suffix solutions. The prefix is executed only once at the beginning and is then followed by the cyclic repetition of the suffix, which goes on indefinitely.} We define atomic predicates over specific robots that need to be completed.\footnote{\textcolor{red}{[I believe we said that we are considering arbitrary LTL formulas and that's why later we have NBA and DFA. Also, here you need to have a brief discussion on what LTL is. People are not necessarily familiar with it. Later you use $\Diamond$, etc but these operators are nowhere defined. Read/write your paper carefully and make sure it is accessible enough to all people working on planning problems.  \textcolor{blue}{fixed}]}} 
% \textcolor{magenta}{We assume each task needs only one robot. So even if task is defined over a team, only one robot from team needs to do it. Note for self: when defining multiple tasks over same team you will need to check if that many robots are available}
We define predicates, denoted by $\pi_{\bbT_q}^p(rob_j, \varkappa_q, \ell_i)$\footnote{\textcolor{red}{following up on an earlier comment, in the definition of the predicate, do you mean $q$ or $\zeta_{\varkappa_q}$. Again, $\zeta_{\varkappa_q}$ is just a binary variable and not a skill.} \textcolor{blue}{fixed}}, as follows: 
\begin{equation}\label{eq:pip}
\pi_{\bbT_q}^p(rob_j, \varkappa_q, \ell_i)=
 \begin{cases}
  \text{true}, & \text{if $rob_j\in\bbT_q \text{ applies } \varkappa_q\text{ at }\ell_i$}\\
  \text{false}, & \text{otherwise}
 \end{cases}       
\end{equation}

The predicate associated with \eqref{eq:pip} is true when a robot $rob_j$ belonging to the team $\bbT_q$, after applying control actions \textcolor{blue}{$\bbu_{0:t}$ (how do I write this?)}, visits location $\ell_i$ and uses the ability $\varkappa_q$. It is assumed that when $rob_j$ uses ability $\varkappa_q$, it successfully completes the task associated with the atomic predicate. When specifying an atomic predicate, $rob_j$ refers to the robot that the atomic predicate is currently assigned to. When defining the initial mission, we assume the initial task assignment to be completed and we specify the robots associated with each atomic proposition. This assignment can change during the mission to another robot as long as the newly assigned robot belongs to $\bbT_q$. The $p$ in $\pi^p$, is a unique identifier for each predicate, such that if there are $P$ predicates in the mission then $p\in\set{1,\dots,P}$. 
Hereafter, when it is clear from the context, we simply denote a \st{perception-based} predicate by $\pi^p$ or $\pi_{\bbT_q}^p$.\textcolor{red}{[Let's delete/edit this sentence. We do not really have `perception' in this paper]}\textcolor{blue}{fixed}
% Furthermore, when defining the initial mission, we specify the robots associated with each atomic proposition. That is the initial task assignment for the robots is assumed to be completed.  

% In \eqref{eq:pip}, $\Delta$ is a set of user-specified and case-specific parameters (e.g., task or robots indices) and $p(\bbp(t),\ccalM(t),\Deltra): \Omega^N\times\ccalM(t)\times\Delta\rightarrow\mathbb{R}$. Hereafter, when it is clear from the context, we simply denote a perception-based predicate by $\pi_p$.
% First, we define the following function reasoning about the metric uncertainty of the map:
% \begin{align}
% &p(\bbp(t),\ccalM(t), \{j,\ell_i,r,\zeta_{\varkappa_q},\psi_i\})=\nonumber\\&\mathbb{P}(||\bbp_j(t)-\bbx_i(t)||\leq r) X \nonumber\\&\mathbb{P}(\text{ability } \zeta_{\varkappa_q} \text{ used })\label{ap1} 
% \end{align}
% % \textcolor{magenta}{I don't know the correct notation, but $\mathbb{P}$ basically returns 1 if true and 0 if false}
% The predicate associated with \eqref{ap1} is true at time $t$ if robot $j$ is within distance less than $r$ from target $\ell_i$, after applying control actions $\bbu_{0:t}$, for some user-specified parameters $r>0$ $\And$ has successfully used ability $\zeta_{\varkappa_q}$ to complete its task at $\ell_i$. $\psi_i$ is the penalty associated for not completing the task. Assigning a penalty to each atomic proposition allows the algorithm (ref future section) to decide which proposition to prioritize in a scenario where only one proposition can be completed among two or more.


 \textcolor{blue}{The co-safe LTL syntax for a sequence of multi-robot states  ($\bbp_j(t)$) and a map $\ccalM$ is given by the expression $\phi::=\text{true}|\pi_p~|\neg\pi_p|\phi_1\wedge\phi_2|\phi_1\vee\phi_2|\phi_1\mathcal{U}~\phi_2$, where (i) $\pi_p$ is an atomic predicate as defined earlier \ref{eq:pip} and (ii) $\wedge$, $\vee$, $\neg$, and $\mathcal{U}$ represent the conjunction, disjunction, negation, and until operator, respectively. Additionally, the eventually operator $\Diamond$ can be defined using $\mathcal{U}$ \cite{baier2008principles}.}

\begin{ex}[LTL Mission Specification]\label{ex:LTL}
\textcolor{blue}{Consider a three-robot mission and the robots collectively having the following abilities $move$, $temperature$, $photo$ captured by the robot ability list $\bbZ=[\zeta_{move}, \zeta_{temp}, \zeta_{photo}]$}. Specifically, these are the abilities to move, record the temperature at a location, and the ability to take photos. Individual ability list of the three robots $rob_1$, $rob_2$, and $rob_3$ at the beginning of the mission are as follows $\bbZ_1=[1,1,0]$, $\bbZ_2=[1,1,1]$, and $\bbZ_3=[1,0,1]$.

The mission requires $rob_1$ to take a temperature reading ($\zeta_{temp}$) at location $\ell_1$ on a pipeline, and subsequently for $rob_2$ to take a photo ($\zeta_{photo}$) of the pipeline at a different location ($\ell_3$). 
% The mission requires $rob_1$, to deliver ($\zeta_{deliver}$) a \textcolor{blue}{package it's carrying} at landmark $\ell_1$, and subsequently for $rob_2$ to take a photo ($\zeta_{photo}$) of the delivered package at landmark $\ell_1$. 
Simultaneously $rob_3$ must take a temperature reading ($\zeta_{temp}$) of the pipeline at location $\ell_2$. 
% \textcolor{red}{[Maybe you need to define a `grasp' skill too? (to pick up the package that needs to be delivered)\textcolor{blue}{to keep the example/ltl formula simple, the setup assumes robots are already carrying the packages}]}
This task can be captured by the following co-safe LTL formula:%; see also Figure \red{(??)}:
%\begin{subequations}
\begin{align}\label{eq:ExampleTask1}
    \phi = &\Diamond[\pi_{\bbT_2}^1(rob_1, \zeta_2, \ell_1)\wedge\Diamond[\pi_{\bbT_3}^2(rob_2, \zeta_3, \ell_3)]]\nonumber\\&\wedge\Diamond[\pi_{\bbT_2}^3(rob_3, \zeta_2, \ell_2)]
\end{align}
where the atomic predicates are defined as in \eqref{eq:pip}.
\end{ex}

\subsection{Ability Failure}\label{sec:failure_def}
In practical situations, robots may not always function optimally either due to unfavorable environmental conditions or internal malfunction. This can result in a complete failure, such as a drone crashing into a tree, or a partial failure, such as a camera on the robot not working. We define this as "ability failure". 
Since the robot $rob_j$ is able to monitor its health, if it does lose any ability $\zeta_{\varkappa_q}$, it will set the corresponding value in the robot ability list $Z_j$ to $0$, i.e., $Z_j[q](t)=0$. Hence $Z_j(t)$, allows us to keep track of all the abilities that the robot can use at time $t$. Similarly if $rob_j$ loses ability $\zeta_{\varkappa_q}$, it will be removed from the team $\bbT_q$, since $\bbT_q(t)$ keeps track of all the robots that have ability $\zeta_{\varkappa_q}$.

Thus the state of each robot, $rob_j$ at time $t$, can be defined by its current position and its current abilities.
\begin{equation}\label{eq:rstate}
rob_j(t)=\{\bbp_j(t),Z_j(t)\}
\end{equation}
On the same lines if at any time the failure is fixed and the ability is restored, then the $\zeta_{\varkappa_q}$, in the robot ability list $Z_j$, corresponding to that particular ability is set to $1$, indicating the robot can start using that ability once more.

% For the purpose of experiments, we define $\zeta_1$ as the ability to move. Thus if this ability is set to 0, the robot is completely incapacitated and cannot use any other abilities. This is equivalent to disabling all the other abilities in the robot ability list $\bbZ_j$ of the robot to 0.



% \textcolor{magenta}{needs more elaboration. what if ability/task is to photograph. then it does not change state $\psi_i$. we could have state as not photographed and photographed. but then what to do if i want to photograph it more than once. how and when will i reset its state to not photographed.}



% \subsection{Types of failures}\label{sec:PFcases}
% example Cases for reference only. not part of problem formulation

% \textbf{Case} 1:
% Drone 1 fails completely (i.e., $\zeta_1 = 0$) Then all remaining tasks need to be reassigned to other members of drone team.

% \textbf{Case} 2:
% Task: take photo at height of 16m ;
% Drone 1 loses ability to fly at 16m altitude (can only fly at 8m) (i.e., $\zeta_1 = 0$) Then only this task needs to be reassigned to other members of drone team. Drone 1 continues with its other tasks.

% \textbf{Case} 3: replacing with another team  ;
% team 1 drones don't have flash, team 2 drones have flash.  ;
% Task: go to room and take photo.  ; 
% Drone 1 reaches target and realizes that room is dark. 
% Team 2 drone has ability flash. So drone1 replaced with team 2 drone for task.


% \textbf{Case} 4:
% Task: drone 1 should go to landmark inside room. (door is assumed open)\textcolor{red}{[YK: this is more of a new mission rather than a failure of one of the available robot abilities]}

% Drone 1 sees door is closed. generate new mission where ground robot is assigned task to open door.



\subsection{Resilience to Failures}
Suppose a multi-robot system is tasked with completing a certain mission and the system has generated trajectories for each robot to follow that will ensure that all the tasks in the mission are completed. At some point of time during the mission, if one or more robots in the system experience some kind of failure, then the pre-computed trajectories will no longer satisfy the mission requirements. This will result in a failed mission. This gives rise to our problem statement.
\begin{problem}\label{prob_statement}
Given a mission specification $\phi$, robot model \eqref{eq:rdynamics}, all robot states \eqref{eq:rstate}, the environment $\ccalM$, and the current time $t$, 
\footnote{\textcolor{red}{This does not make sense. If we focus on arbitrary LTL formulas, the horizon is infinite. LTL formulas are defined by infinite paths (written in a prefix-suffix form). Read your draft carefully and make sure there are no inconsistencies between the problem formulation and the proposed solution.}} 
a sequence $\bbu_{t:\inf}$ of control inputs $\bbu(\hat{t})$, for all $\hat{t}\in\set{t,\dots,\inf}$, that satisfy $\phi$. 
Since the robot states \eqref{eq:rstate} captured by $rob_j(t)$ keeps track of all its current set of active abilities, any failure is reflected in its state. As the control inputs $\bbu(\hat{t})$, needs to satisfy $\phi$ for all $\hat{t}\in\set{t,\dots,\inf}$, if $rob_j$ suffers a mission affecting failure at time $t$, we need to generate a new sequence of control inputs $\bbu(\hat{t})$ such that $\phi$ continues to remain satisfied. \textcolor{blue}{[shall we remove controls $\bbu(\hat{t})$ from problem statement completely and only say generate path $\tau$ that satisfies $\phi$? But the how do we say that this path is only from $\hat{t}$?]}
\end{problem}
% we can generate over a  horizon $H$, a sequence $\bbu_{0:H}$ of control inputs $\bbu(t)$, for all $t\in\set{0,\dots,H}$, that satisfy $\phi$


% Given a mission specification $\phi$, robot model \eqref{eq:rdynamics}, and the environment, we can generate over a  horizon $H$, a sequence $\bbu_{0:H}$ of control inputs $\bbu(t)$, for all $t\in\set{0,\dots,H}$, that satisfy $\phi$ \cite{Kantaros2020perception,Kalluraya2023multi}. However, if at a certain time $t$ during the mission, a robot $rob_j$ associated with a certain atomic predicate $\pi_{\bbT_q}$ loses its ability $\zeta_{\varkappa_q}$, the robot will no longer be able to complete the task associated with that predicate. Thus the sequence of control inputs $\bbu_{t:H}$ will not satisfy $\phi$. This will result in a failed mission. 



% The objective is to choose a stopping horizon $H$ and a sequence of control inputs $\bbu(t)$ for all $t\in{0,\dots,H}$ that fulfill the task specification $\phi$ while accommodating for any malfunctioning robots. This is achieved by incorporating the observation model, the robot dynamics, and environment characteristics. In the event of a robot failure, the task should be reassigned to a functioning robot to ensure its completion.


==> files/alg_ICRA.tex <==
In this section we present an algorithm to solve the planning problem defined in Problem \ref{prob_statement}. To solve this problem we split our solution into two parts. The first part of the solution is a sampling-based planner that we have developed in our previous work \cite{Kantaros2020perception}. In this algorithm, given a mission specification $\phi$, and the robot dynamics, the planner can generate path $\tau$ that satisfies $\phi$.
% the planner can generate a sequence of control inputs $\bbu(\hat{t})$, for all $\hat{t}\in\set{0,\dots,\inf}$, that satisfy $\phi$. 
This however does not have any provision for robot failures during the mission. While our previous work considers uncertainty in the environment, for sake of simplicity to explain our current approach we assume that there is no uncertainty in the environment.

In the second part of our solution we extend our planning algorithm to be resilient to robot failures.
In the event of a failure in robot $j$ at time $t$, our objective is to pick another robot $j'\in\ccalT_c$, and $j'\in\ccalR$, $j'\neq j$, that can replace robot $j$ in the affected atomic predicate $\pi_p$, where $\pi_p=\pi_{\ccalT_c}(j,c,\ell_i)$. In case of multiple abilities in multiple robots failing at the same time, the objective is to replace the robots in all the affected atomic propositions. 
We then run the sampling-based planner again to generate a new path $\tau$ such that $\phi$ is satisfied even after robot failures. 


\subsection{From LTL Missions to Automata}
Given an LTL mission $\phi$, first we translate it into a Nondeterministic B$\ddot{\text{u}}$chi Automaton(NBA), defined as follows \cite{baier2008principles}. 

%\begin{definition}[NBA]
%A Nondeterministic B$\ddot{\text{u}}$chi Automaton (NBA) $B$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\Sigma,\delta_B,q_F\right)$, where $\ccalQ_{B}$ is the set of states, $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is a set of initial states, $\Sigma$ is an alphabet, $\delta_B:\ccalQ_B\times\Sigma\rightarrow2^{\ccalQ_B}$ is a non-deterministic transition relation, and $q_F\in\ccalQ_{B}$ is the accepting/final state. 
%\end{definition}

\textcolor{red}{[I have edited the NBA definition. Please take a look and make sure you understand it. If you have any questions, let me know.]}
\begin{definition}[NBA]
A Nondeterministic B$\ddot{\text{u}}$chi Automaton (NBA) $B$ over $\Sigma=2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\Sigma,\delta_B,\ccalQ_{B}^F\right)$, where $\ccalQ_{B}$ is the set of states, $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is a set of initial states, $\Sigma$ is an alphabet, $\delta_B:\ccalQ_B\times\Sigma\rightarrow2^{\ccalQ_B}$ is a non-deterministic transition relation, and $\ccalQ_{B}^F\in\ccalQ_{B}$ is a set of accepting/final states. 
\end{definition}

%\textcolor{blue}{An infinite NBA run ($\rho_B$) is an unending sequence of states that begins with a starting state and follows the transition relation, where $\rho_B=q_B^0q_B^1q_B^2\dots$ such that  $q^0_B \in \ccalQ^0_B$ and $(q^k_B, \pi_k, q^{k+1}_B) \in \delta_B, \forall k \in \mathbb{N}$. The path $\tau$ and its corresponding run $\rho_B$ are called accepting if $\texttt{Inf}(\rho_B)\cap\ccalQ_B^F\neq\emptyset$, where $\texttt{Inf}(\rho_B)$ is the set of states that occur infinitely often in $\rho_B$. Thus if a generated path $\tau$ is accepting, it means that it satisfies the LTL mission specifications.}
%\textcolor{red}{[here you need to talk about the NBA accepting condition. Otherwise, it is unclear how/why you need this automaton]}

Next, we discuss the accepting condition of the NBA that is used to find plans $\tau$ that satisfy $\phi$. We define a labeling function $L:\mathbb{R}^{nN}\times\mathbb{R}^{N}\rightarrow 2^{\mathcal{AP}}$ determining which atomic propositions are true given the current multi-robot state $\bbp(t)$ and binary vector $\bbs(t)$ capturing the skills that each robot applies at time $t$.
An infinite run $\rho_B= q_B^1 \dots q_B^k \dots$ of $B$ over an infinite word $w = \sigma_0\sigma_1\sigma_2\dots\in\Sigma^{\omega}$, where $\sigma_k \in \Sigma$, $\forall k \in \mathbb{N}$, is an infinite sequence of NBA states $q_B^k$, $\forall k \in \mathbb{N}$, such that $q_B^{k+1}\in\delta_B(q_B^k, \sigma_k)$ and $q_B^0\in\ccalQ_B^0$. An infinite run $\rho_B$ is called 
\textit{accepting} if $\text{Inf} ( \rho_B) \bigcap \mathcal{Q}_B^F \neq \emptyset$, where $\text{Inf} (\rho_B)$ represents the set of states that appear in $\rho_B$ infinitely often. A plan $\tau=[\bbp(0),\bbs(0)],[\bbp(1),\bbs(1)],\dots,[\bbp(t),\bbs(t)],\dots$ is feasible if the word $w=\sigma_0\sigma_1\dots \sigma_t\dots$ where $\sigma_t=L([\bbp(t),\bbs(t)])$, results in at least one accepting run $\rho_B$.

% Any LTL formula $\phi$ can be translated into a Nondeterministic B$\ddot{\text{u}}$chi Automaton (NBA) over $2^{\mathcal{AP}}$ defined as follows \cite{vardi1986automata}:
% \begin{definition}[NBA]
% A \textit{Nondeterministic B$\ddot{\text{u}}$chi Automaton} (NBA) $B$ over $2^{\mathcal{AP}}$ is defined as a tuple $B=\left(\ccalQ_{B}, \ccalQ_{B}^0,\Sigma,\rightarrow_B,\mathcal{Q}_B^F\right)$, where $\ccalQ_{B}$ is the set of states, $\ccalQ_{B}^0\subseteq\ccalQ_{B}$ is a set of initial states, $\Sigma=2^{\mathcal{AP}}$ is an alphabet, $\rightarrow_{B}\subseteq\ccalQ_{B}\times \Sigma\times\ccalQ_{B}$ is the transition relation, and $\ccalQ_B^F\subseteq\ccalQ_{B}$ is a set of accepting/final states.
% \end{definition}

% {\textcolor{blue}{Is this para needed?} \textcolor{gray}{We define a labeling function $L:\Omega^N\times\ccalM(t)\rightarrow 2^{\mathcal{AP}}$ determining which atomic propositions are true given the current multi-robot state $\bbp(t)$ and the current map $\ccalM(t)$. Given a robot trajectory $\bbp_{0:H}$ and a corresponding sequence of maps $\ccalM_{0:H}$, we get the labeled sequence $L(\bbp_{0:H}, \ccalM_{0:H}) =L([\bbp(0), \ccalM(0)])\dots L([\bbp(H), \ccalM(H)])$. This labeled sequence satisfies the specification $\phi$, if starting from the initial state $q_B^0$, each symbol/element in $L(\bbp_{0:H}, \ccalM_{0:H})$ yields an NBA transition so that eventually -after $H$ NBA transitions- the final state $q_F$ is reached \cite{baier2008principles}.} %With slight abuse of notation we denote this compactly by $q_F=\delta_B(q_B^0,w)$.  

\textcolor{red}{[You may want to move the following paragraph and example later in the text when it is needed. Probably at the beginning of Section III.C]}
\textcolor{blue}{[But we briefly use the concept of picking among $\sigma_b$ in Section III.B?]}
The transition between any two consecutive states $q_B$ and $q_{B}^{\prime} \in \ccalQ_{B}$ in the NBA is governed by a Boolean $b_{q_B,q_{B}^{\prime}}$. The Boolean is defined over the atomic predicates which when satisfied enables the transition from $q_B$ to $q_{B}^{\prime}$. 
Let $\sigma_b$ represent a combination of truth values for the atomic predicates which can satisfy the Boolean ($\sigma_b\models b_{q_B,q_{B}^{\prime}}$).
$\Sigma_{q_B,q_{B}^{\prime}}$ is the set of all such combinations $\sigma_b$ that satisfy the Boolean $b_{q_B,q_{B}^{\prime}}$. 
\textcolor{blue}{Our sampling-based planner (Sec \ref{sec:samplingAlg}) picks $\hat{\sigma}\in\Sigma_{q_B,q_{B}^{\prime}}$ to bias the sampling strategy to satisfy these predicates to enable the transition. }
% We arbitrarily pick $\hat{\sigma}\in\Sigma_{q_B,q_{B}^{\prime}}$ that is referenced by our sampling-based planner (Sec \ref{sec:samplingAlg}) as the set of predicates that need to be satisfied to enable the transition. 
To understand this we will refer to the following example:

\begin{figure}[t]
  \centering
\includegraphics[width=0.95\linewidth]{figures/LTLtransition.png}
% \vspace{-1em}
    \caption{\textcolor{black}{Example of a transition between two states in the NBA.} }
    \vspace{-0.3cm}
  \label{fig:LTL}
\end{figure}

\begin{ex}[NBA transition]\label{ex:LTL_trans}
% Consider a mission involving 5 robots, $rob_1,\dots,rob_5$. Assume $rob_1,rob_2,rob_4,rob_5$ have the same single ability $\zeta_1$ and $rob_3$ has a different ability $\zeta_3$. Consider the following atomic predicates in the mission:   $\pi_{\ccalT_1}^1(rob_1, \zeta_1, \ell_1)$, $\pi_{\ccalT_1}^2(rob_2, \zeta_1, \ell_2)$, $\pi_{\ccalT_3}^3(rob_3, \zeta_3, \ell_3)$, $\pi_{\ccalT_1}^4(rob_4, \zeta_1, \ell_2)$,
% Consider a mission involving five robots, robot $1$ to robot $5$. Assume robots $1,2,4,5$ have the same single ability $c_2$ and robot $3$ has a different ability $c_3$. All robots have the ability to move $c_1$. Robot $4$ has addition ability $c_4$ Consider the following atomic predicates in the mission:   $\pi_1=\pi_{\ccalT_1}(1, c_2, \ell_1)$, $\pi_2=\pi_{\ccalT_1}(2, c_2, \ell_2)$, $\pi_3=\pi_{\ccalT_3}(3, c_3, \ell_3)$, $\pi_4=\pi_{\ccalT_4}(\emptyset, c_1, \ell_2)$,

% \begin{align}\label{eq:taskEx2}
%     \phi = &\Diamond[\pi_{\ccalT_2}(rob_1, \zeta_2, l_1)\wedge\Diamond[\pi_{\ccalT_3}(rob_2, \zeta_3, l_1)]]\nonumber\\&\wedge\Diamond[\pi_{\ccalT_2}(rob_3, \zeta_2, l_2)]\nonumber
% \end{align}

\textcolor{blue}{We build the NBA for the mission given in Example \ref{ex:LTL}.
A particular transition in the NBA $q_B\rightarrow q_{B}^{\prime}$ (Fig. \ref{fig:LTL}) is governed by the boolean $b_{q_B,q_{B}^{\prime}}$ = $(\pi_1\land\pi_2\land\neg\pi_4)\lor(\pi_1\land\pi_3\land\neg\pi_4)$. There are self loops at both ends, $b_{q_B,q_B}$ = $b_{q_{B}^{\prime},q_{B}^{\prime}}$ = $\neg\pi_4$. 
For this example if any of $\sigma_1$ = $(\pi_1,\pi_2)$, $\sigma_2$ = $(\pi_1,\pi_3)$, or $\sigma_3$ = $(\pi_1,\pi_2,\pi_3)$ are true, and $(\pi_4)$ is not true, then the transition $q_B\rightarrow q_{B}^{\prime}$ is satisfied. Therefore, $\Sigma_{q_B,q_{B}^{\prime}}=[\sigma_1,\dots,\sigma_5]$.}

%\begin{subequations}
% \begin{align}\label{eq:taskEx}
%     \phi = &\Diamond[\pi_{\ccalT_2}(rob_1, \zeta_2, l_1)\wedge\Diamond[\pi_{\ccalT_3}(rob_2, \zeta_3, l_1)]]\nonumber\\&\wedge\Diamond[\pi_{\ccalT_2}(rob_3, \zeta_2, l_2)]\nonumber
% \end{align}

\end{ex}

% \textcolor{red}{Not sure if I should mention all the parameters stored in DFA edge: transition skill, etc}

% \textcolor{red}{How much to write about sampling method?}
\subsection{Sampling-based planner}\label{sec:samplingAlg}
The sampling-based planner is designed to search simultaneously both the mission space as well as the physical space. It does this by sampling states of the form \textcolor{blue}{$\bbq(t)=[\bbp(t), \bbs(t), q_B(t)]$}, where $\bbp(t)\in\Omega_{free}$, $s_j(t)\in\ccalC$, and $q_B(t)\in\ccalQ_B$. 
% \textcolor{red}{[This needs to be fixed. Define our nodes appropriately. I believe our nodes should have the form $[\bbp(t), \bbs(t), q_B(t)]$} \textcolor{blue}{Yes, I agree $\ccalM(t)$ will not be included in the node as $\ccalM$ is constant. But even $\bbs(t)$ need not be included, because during offline planning $\bbs$ is also constant.} \textcolor{red}{[$\bbs$ cannot be constant. It tells you what skills (if any) the robots should apply at each time $t$. Determining only robot positions is not enough to satisfy the considered tasks (satisfaction of our atomic predicates requires both positions and application of skills) ]} 
These states, if feasible, are added to a tree. 
\textcolor{blue}{Since some transitions from one state to next could be satisfied in more than one way, the planner picks one symbol $\hat{\sigma}\in\Sigma_{q_B,q_{B}^{\prime}}$ for every transition and uses it to bias the exploration towards locations that are expected to contribute to the satisfaction of the assigned mission specification.} When we sample a state such that $q_B(t)$ can be visited infinitely often and it belongs to the final accepting state of the mission ($q_B(t)\in \ccalQ_B^F$), we have found a path that navigates the environment and satisfies the mission.   
% By picking a $\hat{\sigma}$ for each state transition,} we bias the exploration towards locations that are expected to contribute to the satisfaction of the assigned mission specification. When we sample a state such that $q_B(t)$ belongs to the final accepting state of the mission ($q_B(t)\in q_F$), and it to the tree, we have found a path that navigates the environment and satisfies the mission.   
% Essentially, it samples states in the NBA ($q_B)$ while simultaneously sampling points in the obstacle-free space $\Omega_{free}$ in the environment $\ccalM$. The resulting trajectory satisfies the mission requirements, while navigating through the physical environment. 
For details regarding the implementation, refer \cite{luo2021abstraction}. 
% \textcolor{red}{[I suggest you cite this \cite{luo2021abstraction} instead of \cite{Kantaros2020perception}, since \cite{Kantaros2020perception} extends \cite{luo2021abstraction} to unknown environments. Also,  \cite{Kantaros2020perception} considers co-safe LTL formulas and not arbitrary ones that we consider here.]}

% We store in each transition the robots and their respective atomic propositions that enable the transition.

% where $q_D(0)=q_D^0$, $\sigma(t)=L([\bbp(t),\ccalM(t)])$, %and $\ccalM(t)$ is determined by $\hat{\bbx}(t)$, $\Sigma(t)$, 
% and $d(t)$. Note that the constraint in \eqref{constr1c} captures the automaton dynamics, i.e., the next DFA state that will be reached from the current DFA state under the observation/symbol $\sigma(t)$.
% %
% In words, \eqref{eq:ProbR}, is a reachability problem defined over a joint space consisting of the automaton state-space (see \eqref{constr1c}), the robot motion space (see \eqref{constr3c}-\eqref{obsFree2}), and the future target states along with their corresponding metric and semantic uncertainty (see \eqref{constr7x}-\eqref{constr8c}) while the terminal constraint requires to reach the final automaton state (see \eqref{constr9c}).


\subsection{Resilient planning algorithm}
When a robot's ability ($c$) fails, it will not be able to complete any atomic predicates $\pi_p$ that requires it to use $c$. 
\textcolor{blue}{If these predicates are included in $\hat{\sigma}\in\Sigma_{q_B,q_{B}^{\prime}}$, then that transition will not be satified ($\hat{\sigma}\not\models b_{q_B,q_{B}^{\prime}}$),\footnote{\textcolor{red}{Where is that $\hat{\sigma_b}$ coming from?? Something is missing here. }\textcolor{blue}{[In Sec III-A we mention "We arbitrarily pick $\hat{\sigma}\in\Sigma_{q_B,q_{B}^{\prime}}$ that is referenced by our sampling-based planner (Sec \ref{sec:samplingAlg}) as the set of predicates that need to be satisfied to enable the transition. "]} \textcolor{red}{This needs to be fixed based on our slack conversation}} and our previously planned path will no longer satisfy the mission.
We solve this by looking at all affected transitions and the symbols ($\sigma_b$) in the transition and finding a new set of task assignments for the robots which will ensure that the task of the failed robot is assigned to another robot.}
% In this situation we have two options, one is to find a new set of task assignments for the robots which will ensure that the task of the failed robot is assigned to another robot. The other option is to replace $\hat{\sigma}$ with $\sigma_b$, where, $\sigma_b\in\Sigma_{q_B,q_{B}^{\prime}}$, such that $\sigma_b\models b_{q_B,q_{B}^{\prime}}$. 
Note that multiple robots and multiple abilities can fail at the same time. The proposed algorithm is summarized in Algorithm \ref{alg:RP} and Algorithm \ref{alg:bfs}. 

% The NBA is represented as a graph with each edge in the set $E$ represts the transition from one state to another. This transition is enabled when all the atomic predicates associated with that edge are satisfied. In case of robot ability failures, one or more of these predicates in the relevant transitions may not be satisfied and hence we try to fix it. There would be some transitions in the NBA that might not involve the failed abilities and in such cases we would not need to change anything in that particular NBA transition. 
In what follows, we provide some intuition for the steps of the Algorithm \ref{alg:RP}. Let $q_{curr}\in\ccalQ_{B}$ be our current state in the mission that we have successfully reached and at some time $t$, when transitioning to the next state, the abilities of one or more robots fail. 
We look at all the paths we can take in the NBA from $q_{curr}$ to $\ccalQ_{B}^F$ and collect all the transitions that are affected by the failed robot
% between two consecutive states and transitions from each state to itself in these paths 
in the set $\mathcal{E}$ (line \ref{rp:collect}, Alg. \ref{alg:RP}). Essentially the states in the paths are the states we can reach in the remaining part of the mission.
For every $\sigma_b$ in every transition $\Sigma_{q_B,q_{B}^{\prime}}$ in the set $\mathcal{E}$, we initialize an empty set $\mathcal{F}$ (line \ref{rp:assign}, Alg. \ref{alg:RP}). $\mathcal{F}$ will store all the atomic predicates that have failed in $\sigma_b$. 

We also initialize empty sets $\mathcal{A}[\pi_p]$, $\mathbb{C}[\pi_p]$, and $\mathcal{U}[\pi_p]$ for every $\sigma_b$. $\mathcal{A}$ is defined as the set that stores atomic predicates $\pi_p$ ($\pi_p=\pi_{\ccalT_c}(j,c,\ell_i)$), and the respective set of robots for each atomic predicate, where the robots have the ability to satisfy the predicate ($\pi_p$) but are currently ``\textbf{assigned}" to complete another atomic predicate in $\sigma_b$. Mathematically,
\begin{equation}\label{eq:assigned}
\mathcal{A}[\pi_p]=\{j|j\in\ccalT_c \text{ and } j\models\pi_{p'}, \text{ where }\pi_{p'}\in\sigma_b\}
\end{equation}

% $\mathbb{C}[\pi_p]$ is defined as the ``\textbf{constrained}" set that contains all the robots which have mission constraints that restrict them from completing the task $\pi_p$. 
\textcolor{blue}{Constraints are captured by predicates with negation and their presence in a boolean  $b_{q_B,q_B}$ or $b_{q_B,q_B^{\prime}}$ means that the transition will be possible only if these predicates are \textbf{not} satisfied. If constraints are present, then robots that need to satisfy these constraints may not be able to accomplish $\pi_p$, even if they have the ability to do so, if the task that needs to be fulfilled for $\pi_p$ might lead to violations of those constraints. We add such robots to $\mathbb{C}[\pi_p]$ which we call as the ``\textbf{constrained}" set.}
\textcolor{red}{[The statement `in the LTL formula' is not accurate. The formula may have constraints that only temporarily should hold (e.g., do X, Y, Z and avoid X until you do Y. This does not mean that the robots are always subject to the constraint X.)]}\textcolor{red}{[this definition is unclear. Where does this `negation' appear? be more specific.]}
\begin{equation}\label{eq:constraints}
    \mathbb{C}[\pi_p]=\{j | j\in\ccalT_c \text{ and } rob_j\not\models\pi_p\}
\end{equation}
% In Example \ref{ex:LTL_trans}, if we consider the transition enabled by $\sigma_1$, $\mathbb{C}[\pi_{\ccalT_1}^2] = [rob_4]$, due to existence of $b_{q_B,q_B}$ = $\neg\pi^4$ that restricts $rob_4$ from doing $\zeta_1$ at $\ell_2$ which is needed to satisfy $\pi_{\ccalT_1}^2$.

Similarly, $\mathcal{U}$ is defined as the set that stores atomic predicates ($\pi_p$) and the respective set of robots for each atomic predicate, where the robots are chosen such that they have the ability to satisfy the predicate ($\pi_p$), are currently ``\textbf{unassigned}", i.e., they are free and not involved in any task and have no constraints to complete the task. 
% Some robots may be free but the mission might have additional constraints that might restrict them from visiting a certain location or doing a task. Such robots are included in the set $\mathbb{C}[\pi_p]$. These robots are not considered in $\mathcal{U}$ 
Mathematically,
\begin{equation}\label{eq:unassigned}
\mathcal{U}[\pi_p]=\ccalT_c - \mathcal{A}[\pi_p] - \mathbb{C}[\pi_p]
\end{equation}
\textcolor{red}{[i do not see where exactly you use these sets in the following steps]}\textcolor{blue}{[set $\mathbb{C}$ is only used to calculate $\mathcal{U}$. $\mathcal{A}$ and $\mathcal{U}$ are inputs to the BFS alg. I have added a line mentioning that]}

In Example \ref{ex:LTL_trans}, if we consider the transition enabled by $\sigma_1$, then for predicate $\pi_2=\pi_{\ccalT_3}(2, c_3, \ell_2)$, $\ccalT_3=[1,2,4,5]$, and $\mathcal{A}[\pi_2] = [1,2]$ as robot $1$ and robot $2$ are assigned to do predicates $\pi_1$ and $\pi_2$ respectively in $\sigma_1$. 
Next, due to the presence of $\neg\pi^4$ in $b_{q_B,q_B^{\prime}}$, robots belonging to $\ccalT_2$ (robots $1$ and $4$) are restricted from approaching at $\ell_2$ and thus they cannot be assigned to do $\pi_2$ as it involves approaching $\ell_2$. Therefore $\mathbb{C}[\pi_2] = [1,4]$.
Thus, $\mathcal{U} = \ccalT_c - \mathcal{A}[\pi_p] - \mathbb{C}[\pi_p] = [5]$ which means robot $5$ is the free robot that can replace robot $2$ at its task in $\pi_2$ if needed. 

Accordingly, in the algorithm, for every atomic predicate $\pi_p$ in $\sigma_b$, we initialize $\mathcal{A}[\pi_p]$, $\mathbb{C}[\pi_p]$ and $\mathcal{U}[\pi_p]$ as defined in \eqref{eq:assigned}, \eqref{eq:constraints} and \eqref{eq:unassigned} (lines \ref{rp:GETassign}-\ref{rp:GETunassign}, Alg. \ref{alg:RP}).
We then check if the robot $j$ that is currently assigned to do $\pi_p$ is present in $\ccalT_c(t)$. Since $\ccalT_c(t)$ is the set of all robots that currently have the ability $\zeta_c$, if $j$ is not present in $\ccalT_c(t)$, it means that the robot has lost ability $\zeta_c$ and will no longer be able to satisfy $\pi_p$. In this case, we add $\pi_p$ to the set of failed tasks, $\mathcal{F}$ (line \ref{rp:fail_t}, Alg. \ref{alg:RP}).

Finally, for each predicate $\pi_p$ that has failed, we run the BFS Algorithm (Alg. \ref{alg:bfs}). \textcolor{blue}{This algorithm takes the failed predicate, sets $\mathcal{U}$ and $\mathcal{A}$, and symbol $\sigma_b$, to determine the right set of ``robot-task" reassignments.}
This algorithm builds a tree starting from the failed robot and its task to find a task assignment for the robots that will fix the ensure the failed task can be completed by another robot. 
The tree consists of nodes that are of the form $\bbq$=[$j$, $\pi_p$, $\bbq_{parent}$], where robot $j\in\ccalR$, $\pi_p$ is the task currently assigned to robot $j$, and $\bbq_{parent}$ is the parent node of $\bbq$ in the tree. In case robot $j$ is currently unassigned to a task, then the node is of the form $\bbq$=[$j$, $\emptyset$, $\bbq_{parent}$]. For future reference $\bbq.robot$ refers to robot $j$ in the node $\bbq$, $\bbq.task$ refers to the task ($\pi_p$) assigned to the robot $j$, and $\bbq.parent$ refers to the parent node of $\bbq$. The approach is summarized in Algorithm \ref{alg:bfs} and in Sec \ref{bfs_explanation}.
Algorithm \ref{alg:bfs} returns a leaf node in the tree ($\bbq_{child}$) and a flag that is True if a feasible re-assignment is found and False otherwise (line \ref{rp:bfs}, Alg. \ref{alg:RP}).
The idea is that the robot in $\bbq_{child}$ will take up the task of the robot in its parent node. The parent robot will take up the task of its parent node and so on till we replace failed robot in the root node of the tree. Since the root node with the failed robot will not have a parent node, this loop will stop at this point.
At each step, we call the function ROB2task() to update the newly assigned robots in the atomic predicates in $\sigma_b$(lines \ref{rp:rob2task}-\ref{rp:parent_parent}, Alg. \ref{alg:RP}).

Following this, we will end up with the correct robot-task reassignment for that particular failure. We update $\sigma_b$ in the NBA with the new robot-task assignments and make a note that we found a solution ($flag$) (line \ref{rp:update1}, Alg. \ref{alg:RP}). This reassignment might lead to some free/unassigned robots getting assigned and some robots already assigned getting unassigned. To reflect this, we also update $\mathcal{A}$, and $\mathcal{U}$ (line \ref{rp:update2}, Alg. \ref{alg:RP}). 
If we did not find a solution, then we don't make any changes to $\sigma_b$ but note that $flag$ is False (line \ref{rp:update3}, Alg. \ref{alg:RP}). 

% Once these steps are followed for every $\sigma_b \in \Sigma_{q_B,q_{B}^{\prime}}$ we use the function BESTin() to pick a $\hat{\sigma}\in \Sigma_{q_B,q_{B}^{\prime}}$ for which we found a solution (i.e., $flag$=True). Ideally, if we find a reassignments for all failures, then $\hat{\sigma}$ will be the same as it was before the failure. The atomic predicates in $\hat{\sigma}$ will then guide the sampling-based planner for that transition. 

% For example, in Example \ref{ex:LTL_trans} if originally $\hat{\sigma}=\sigma_2$ and say robot $2$ and robot $3$ failed, then BFS will be able to find a solution only for $\sigma_1$, by replacing robot $2$ with robot $5$. In that case, we set $\hat{\sigma}=\sigma_1$.

\begin{algorithm}[t]
\caption{Resilient Planning}
\LinesNumbered
\label{alg:RP}
\KwIn{ (i) NBA, (ii) $\ccalT(t)$, (iii) $q_{curr}$}
\KwOut{Updated NBA}
% reassign\_flag = False\;
$\mathcal{E}=$ COLLECT(NBA, $q_{curr}$)\;\label{rp:collect}
\For{every $\Sigma_{q_B,q_{B}^{\prime}}\in\mathcal{E}$}{
    \For{every $\sigma_b \in \Sigma_{q_B,q_{B}^{\prime}}$}{
        % $tasks$$\leftarrow$ all $\pi_{\ccalT}^p$ in $\sigma$\;\label{rp:tasks}
        % $task\_rob$$\leftarrow$ all task and robot pairs in $tasks$\;\label{rp:t_r}
        % $rob\_task$$\leftarrow$ all robot and task pairs in $tasks$\;\label{rp:r_t}
        $\mathcal{F},\mathcal{U},\mathcal{A}=\emptyset$\; \label{rp:assign}
        % $\mathcal{A}$ = \{\}\;
        % $\mathcal{U}$ =\{\}\;
        \For{$\pi_p \in \sigma_b$, where $\pi_p=\pi_{\ccalT_c}(j,c,\ell_i)$}{
            Generate $\mathcal{A}[\pi_p]$ as per (\ref{eq:assigned})\;\label{rp:GETassign}
            Generate $\mathbb{C}[\pi_p]$ as per (\ref{eq:constraints})\;
            Initialize $\mathcal{U}[\pi_^p]$ as per (\ref{eq:unassigned})\;\label{rp:GETunassign}
            % $\mathcal{A}[\pi_{\ccalT_c}^p]\leftarrow$\small{GET\_assigned}($\pi_{\ccalT_c}^p,T_q(t)$,$\sigma$)\;\label{rp:GETassign}
            % $\mathcal{U}[\pi_{\ccalT_c}^p]\leftarrow$\small{GET\_unassigned{U}}($\pi_{\ccalT_c}^p,T_q(t)$,$\sigma$)\;\label{rp:GETunassign}
            \If{$j\notin\ccalT_c(t)$}{ \label{rp:for1}
                $\mathcal{F}=\mathcal{F}\cup\pi_p$ \label{rp:fail_t}
            }
        }
        \For{$\pi_p \in$ $\mathcal{F}$, where $\pi_p=\pi_{\ccalT_c}(j,c,\ell_i)$}{
            $\bbq_{child},flag$=BFS($\pi_p, \mathcal{U}, \mathcal{A}, \sigma_b$)\;\label{rp:bfs}
            \If{flag = True}{
                $\bbq_{p} = \bbq_{child}.parent$\;
                \While{$\sim$empty($\bbq_{parent}$)}{
                    \small ROB2task($\bbq_{p}.task$, $\bbq_{child}.robot, \sigma_b$)\;\label{rp:rob2task}
                    \normalsize$\bbq_{child}=\bbq_{p}$\;
                    $\bbq_{p}=\bbq_{child}.parent$\;\label{rp:parent_parent}
                }
                Update $\sigma_b, flag$ in NBA\; \label{rp:update1}
                Update $\mathcal{A}[\pi_p]$, $\mathcal{U}[\pi_p]$\;\label{rp:update2}
            }\Else{
                Update $\sigma_b, flag$ in NBA\;\label{rp:update3}
            }
        }
    }
    % $\hat{\sigma}=$BESTin($\Sigma_{q_B,q_{B}^{\prime}}$)\;
    % Update $\hat{\sigma}$ in NBA
}
% Among all nodes in $\ccalX_g$, find $\bbq_{\text{end}}(t_{\text{end}})$ \; \label{rrt:node}
% $H=t_{\text{end}}$ and recover $\bbu_{0:H}$ by computing the path $\bbq_{0:t_{\text{end}}}= \bbq(0), \dots, \bbq(t_{\text{end}}) $\;\label{rrt:solution}
\end{algorithm}





\subsection{BFS algorithm}\label{bfs_explanation}
Given the failed task $\pi_p$, the failed robot $j$, sets $\mathcal{U}$ and $\mathcal{A}$, and the atomic predicates that need to be satisfied ($\sigma_b$) for the NBA transition, this algorithm builds a tree that searches a solution for the failure with the minimum number of robot-task reassignments. The approach is summarized in Algorithm \ref{alg:bfs}.

% The tree consists of nodes that are of the form $\bbq$=[$rob_g$, $\pi^p$, $\bbq_{parent}$], where $rob_g\in R$, $\pi^p$ is the task currently assigned to $rob_g$, and $\bbq_{parent}$ is the parent node of $\bbq$ in the tree. In case $rob_g\in\mathcal{U}$, i.e., if $rob_g$ is currently unassigned to a task, then the node is initialized as $\bbq$=[$rob_g$, $\emptyset$, $\bbq_{parent}$]. For future reference $\bbq.robot$ refers to $rob_g$ in the node $\bbq$ and $\bbq.task$ refers to the task ($\pi^p$) assigned to the $rob_g$.

The first step is to create the root node of the tree as $\bbq_{root}$ = [$j,\pi_p,\emptyset$] and add $\bbq_{root}$ to a queue $\mathcal{Q}$ (lines \ref{bfs:root}-\ref{bfs:queue}, Alg. \ref{alg:bfs}).
We initialize an empty set $\mathcal{V}$ (line \ref{bfs:visited}, Alg. \ref{alg:bfs}) which will keep track of all the robots that we visit while building the tree. $\mathcal{V}$ helps us avoid creating more than one node for a robot. Intuitively a robot cannot be in the tree more than once as that could lead to a solution where that robot might need to do two tasks at the same time which is infeasible. The only robot allowed to appear in the tree a second time is the robot with the failed ability (robot $j$). This can happen if that robot has another active ability and thus can take over another task giving up on the current failed task.


We then keep building the tree until $\mathcal{Q}$ is not empty. To do so we pop the first element in $\mathcal{Q}$ and assign it to $\bbq$ (line \ref{bfs:pop}, Alg. \ref{alg:bfs}). If we haven't previously visited the robot in this node ($\bbq.robot\not\in\mathcal{V}$) and if this is not the root node ($\bbq\neq\bbq_{root}$), we add the robot $\bbq.robot$ to the visited set $\mathcal{V}$ (line \ref{bfs:add2visited}, Alg. \ref{alg:bfs}). 
If there are unassigned robots in $\mathcal{U}$ that can accomplish the task of the robot in $\bbq$, we choose one of the unassigned robots $j'$ using the function PICK (line \ref{bfs:pick}, Alg. \ref{alg:bfs}). This function can choose an unassigned robot based on some optimization criteria. In our implementation, we pick the first robot in the set for simplicity. We then create a new node $\bbq_{child}$ = [$j',\emptyset,\bbq$] 
and return $\bbq_{child}$ and a flag set to True as the solution of the algorithm (lines \ref{bfs:answer1}-\ref{bfs:return1}, Alg. \ref{alg:bfs}).
Intuitively since robot $j'$ is unassigned, it is free to take over the task of the parent, allowing the parent robot to take over the task of its parent, and so on. 
If there are no unassigned robots, then for every robot $j'$ in $\mathcal{A}$ we first check if $j'$ is the robot with the failed ability, robot $j$. If that is the case we create a new node $\bbq_{child}$ = [$j,\emptyset,\bbq$] and return $\bbq_{child}$ and a flag set to True (lines \ref{bfs:answer1}-\ref{bfs:return1}, Alg. \ref{alg:bfs}). We call this type of replacement ``looped-reassignment" as the robot with the failed ability, used its other active ability to take over the task of another robot thus completing a loop in the reassignments. We will see an example of this in Section \ref{sec:looped}. 

If $j'\neq j$ and if we have not visited $j'$ before, we create a node $\bbq_{child}$ = [$j'$, TASK($j'$, $\sigma_b$),$\bbq$], where TASK($j'$,$\sigma_b$) is a function that returns the task  $j'$ is currently assigned to so as to satisfy $\sigma_b$. This node is added to the queue $\mathcal{Q}$ (lines \ref{bfs:child}-\ref{bfs:add2q}, Alg. \ref{alg:bfs}). 
If $\mathcal{Q}$ is emptied without finding a solution, it means there is no feasible solution for this failure in this transition of the NBA and we return an empty node and flag that is set to false indicating that the algorithm could not find a feasible solution. (line \ref{bfs:failreturn}, Alg. \ref{alg:bfs}) 

\textcolor{blue}{Observe that we build the tree in a breadth-first manner and stop building the moment we find a robot that is unassigned to a task. This however does not mean that this is the only solution present. If we continue building the tree, we might find other combinations of robot-task reassignments, but the number of robots that will be reassigned to fix the failure will always be equal to or more than the first solution that we find because we build the tree in a breadth-first manner.}   
\textcolor{red}{[Also, here you need to discuss if your tree considers all possible re-assignments. If I remember correctly, the tree does not really search exhaustively all possible reassignments. This is important to mention. Please provide these details. ]}


\textbf{Proposition}: For a single failure we are guaranteed to find a solution if one exists.

The design of the tree is such that the robots in the child nodes are the robots that can replace the parent node in its current task. We add child nodes to the tree irrespective of whether the robots in the child nodes are free or are currently doing a task. Thus when we build the complete tree we will search the entire space of robots that can replace another robot starting from the failed robot. Thus if there exists a free robot in any of the child nodes, we have found a solution for the failure.

In case of multiple simultaneous failures, the order in which we fix these failures does not matter, because when we fix one failure, the changes due to this re-assignment will get reflected in the new tree we build for the second failure.  
% In this tree, all the children of a node are the robots that have the ability to replace the parent robot at its task. Since we keep expanding this tree for all the children, we search for all possible robots that can replace each task. Thus if there exists a solution, that is if there exists a particular order of robot-task re-assignments, we are guaranteed to find it. Furthermore, since the tree is built in a breadth-first manner, the first solution that we find is guaranteed to have the least number of robot-task re-assignments.

\begin{algorithm}[t]
%\footnotesize
\caption{Breadth First Search}
\LinesNumbered
\label{alg:bfs}
\KwIn{ (i) Failed robot and task: $\pi_p=\pi_{\ccalT_c}(j, \zeta_c, \ell_i)$, (ii)$\mathcal{U}$, (iii)$\mathcal{A}$, (iv) $\sigma_b$}
\KwOut{answer node}
$\bbq_{root}$ = [$j$, $\pi_p$,$\emptyset$]\;\label{bfs:root}
$\mathcal{Q}$ = [$\bbq_{root}$]\;\label{bfs:queue}
$\mathcal{V}=\emptyset$\;\label{bfs:visited}
% $flag$ = False\;\label{bfs:first_time}
\While{$\sim$empty($\mathcal{Q}$)}{
    $\bbq\leftarrow$ POP($\mathcal{Q}$)\;\label{bfs:pop}
    \If{$\bbq.robot\notin \mathcal{V}$}{
        \If{$\bbq\neq\bbq_{root}$ }{
            $\mathcal{V}=\mathcal{V}\cup\bbq.robot$\;\label{bfs:add2visited}
        }
        % $flag$ = True\;
        \If{$\sim$empty($\mathcal{U}[\bbq.task]$}{
            $j'$ = PICK($\mathcal{U}[\bbq.task]$)\;\label{bfs:pick}
            $\bbq_{child}$ = [$j'$, $\emptyset$, $\bbq$]\;\label{bfs:answer1}
            return ($\bbq_{child}$, True)\;\label{bfs:return1}
        }
        \For{$j' \in \mathcal{A}[\bbq.task]$}{
            \If{$j'$ = $j$}{
                $\bbq_{child}$ = [$j$, $\emptyset$, $\bbq$]\;\label{bfs:answer2}
                return ($\bbq_{child}$, True)\;\label{bfs:return2}
            }
            \ElseIf{$j'\notin \mathcal{V}$}{
                $\bbq_{child}$ = [$j'$, TASK($j',\sigma_b$), $\bbq_{child}$]\;\label{bfs:child}
                $\mathcal{Q}=\mathcal{Q}\cup child$\;\label{bfs:add2q}
            }
        }
    }
}
return ($\emptyset$, False) \label{bfs:failreturn}
\end{algorithm}



% \subsection{BFS algorithm}\label{bfs_explanation}
% This algorithm builds a tree such that each node in the tree represents a robot and the children of that node are those robots that can do the task of the parent robot. We start the tree with the root node representing the failed robot. We build the tree in a breadth-first manner, and if there exists a solution, the tree will stop building when it finds a robot that is currently unassigned. While this robot may not necessarily directly replace the failed robot, the path in the tree from this robot to the root is the sequence of reassignments that need to be done to fix the failed task.

% The input for the algorithm is the failed task $\pi_{\ccalT_c}^p$, failed robot $rob_j$, sets $\mathcal{U}$ and $\mathcal{A}$, and the atomic predicates that need to be satisfied ($\sigma_b$) for the NBA transition to happen. The first step is to add the failed robot and failed task to the root node called $root$ and add the $root$ to a queue $\mathcal{Q}$ (lines \ref{bfs:root}-\ref{bfs:queue}, Alg. \ref{alg:bfs}). We initialize an empty set $\mathcal{V}$ which will keep track of all the nodes that we visit (line \ref{bfs:visited}, Alg. \ref{alg:bfs}). $\mathcal{V}$ helps us avoid expanding the tree for a particular robot more than once. Intuitively a robot cannot be in the tree more than once as that could lead to a solution where that robot might need to do two tasks at the same time which is infeasible. The only robot allowed to appear in the tree a second time is the robot with the failed ability ($root$). This can happen if that robot has another active ability and thus can take over another task giving up on the current failed task.

% We then keep building the tree until $\mathcal{Q}$ is not empty. To do so the node $parent$ is set to the first node in $\mathcal{Q}$ and that node is removed from $\mathcal{Q}$ (line \ref{bfs:pop}, Alg. \ref{alg:bfs}). If we haven't previously visited this node and if this is not the root node, we add $parent$ to $\mathcal{V}$ (line \ref{bfs:add2visited}, Alg. \ref{alg:bfs}). If there are unassigned robots that can accomplish the task of the robot in $parent$, we choose one of the unassigned robots $rob_g$ using the function PICK (line \ref{bfs:pick}, Alg. \ref{alg:bfs}). This function can choose an unassigned robot based on some optimization criteria. In our implementation, for simplicity, we pick the first robot in the set. We then add the $rob_g$ and the $parent$ to a new node called $answer$ and return $answer$ and a flag set to True as the solution of the algorithm (lines \ref{bfs:answer1}-\ref{bfs:return1}, Alg. \ref{alg:bfs}). If there are no unassigned robots, then for every robot $rob_g$ in $\mathcal{A}$ we first check if this $rob_g$ is the same as the $root$ robot or in other words the robot with the failed task. If that is the case we add $rob_g$ and the $parent$ to a new node called $answer$ and return  $answer$  and a flag set to True (lines \ref{bfs:answer1}-\ref{bfs:return1}, Alg. \ref{alg:bfs}) (we call this type of replacement ``looped-reassignment" and we will see an example of this in Section \ref{sec:looped}). Otherwise, if we have not visited $rob_g$ before, we create a child node with $rob_g$, the task $rob_g$ is currently assigned to (using function TASK($rob_g$,$\sigma_b$) that returns the task  $rob_g$ needs to do to satisfy $\sigma_b$), and $parent$, and add this node to $\mathcal{Q}$. (lines \ref{bfs:child}-\ref{bfs:add2q}, Alg. \ref{alg:bfs}). If we empty $\mathcal{Q}$ without finding a solution, then we return an empty node and  flag that is set to false indicating that the algorithm could not find any feasible solution.  

% When we build this tree, we search all possible robots that can replace each task. Thus if there exists a solution, that is if there exists a particular order of robot-task re-assignments, we are guaranteed to find it. Furthermore, since the tree is built in a breadth-first manner, the first solution that we find is guaranteed to have the least number of robot-task re-assignments.

% \begin{algorithm}[t]
% %\footnotesize
% \caption{Breadth First Search}
% \LinesNumbered
% \label{alg:bfs}
% \KwIn{ (i) Failed robot and task: $\pi_{\ccalT_c}^p(rob_j, \zeta_c, l_i)$, (ii)$\mathcal{U}$, (iii)$\mathcal{A}$, (iv) $\sigma_b$}
% \KwOut{answer node}
% $root$ = [$rob_j$, $\pi_{\ccalT_c}^p$,parent=None]\;\label{bfs:root}
% $\mathcal{Q}$ = [$root$]\;\label{bfs:queue}
% $\mathcal{V}=\emptyset$\;\label{bfs:visited}
% $first\_time$ = True\;\label{bfs:first_time}
% \While{$\sim$empty($\mathcal{Q}$)}{
%     $parent\leftarrow$ POP($\mathcal{Q}$)\;\label{bfs:pop}
%     \If{$parent\notin \mathcal{V}$}{
%         \If{$\sim first\_time$}{
%             $\mathcal{V}\leftarrow parent$\;\label{bfs:add2visited}
%         }
%         $first\_time$ = False\;
%         \If{$\sim$empty($\mathcal{U}[parent.task]$}{
%             $rob_g$ = PICK($\mathcal{U}[parent.task]$)\;\label{bfs:pick}
%             $answer$ = [$rob_g$, parent=$parent$]\;\label{bfs:answer1}
%             return ($answer$, True)\;\label{bfs:return1}
%         }
%         \For{$rob_g \in \mathcal{A}[parent.task]$}{
%             \If{$rob_g$ = $root.robot$}{
%                 $answer$ = [$root.robot$, parent=$parent$]\;\label{bfs:answer2}
%                 return ($answer$, True)\;\label{bfs:return2}
%             }
%             \ElseIf{$rob_g\notin \mathcal{V}$}{
%                 \small$child$ = [$rob_g$,TASK($rob_g,\sigma_b$),parent=$parent$]\;\label{bfs:child}
%                 $\mathcal{Q}\leftarrow child$\;\label{bfs:add2q}
%             }
%         }
%     }
% }
% return ($\emptyset$, False)
% \end{algorithm}



\subsection{Online replanning}
\textcolor{green}{[IMPORTANT:} \textcolor{red}{I suggest here we explain how we can possibly leverage the previous tree (or the previous paths). This text implies that we do local task allocation but we do global re-planning which somehow makes us similar to [32] (in some sense the global replanning defeats the purpose of local task reallocation). For example, here: use the previous tree to initialize the planner as follows. For every node $\bbq(t)=[\bbp(t),\bbs(t),q_B(t)]$ in the previous tree, switch the abilities in $\bbs(t)$ from $c$ to $\varnothing$ if they have failed. Then, after you do this, recompute the NBA states associated with these tree nodes. Then use that tree to initialize your planner. OR: you could possibly use the planner to locally revise the paths. e.g., to fix the path connecting $q_B$ to $q_B'$ if this an affected transition. I thought that you were doing the latter. Possibly we could describe both or the one that is easier to explain]}

The sampling-based planner builds a tree by sampling nodes in the form $\bbq(t)=[\bbp(t), \bbs(t), q_B(t)]$ and every node $\tau(t)$ in the resulting path $\tau$ corresponds to a node $\bbq(t)$ in the tree and a state  $q_B(t)$ in the NBA. The run $\rho_B=q_B^1\dotsq_B^k\dots$ corresponding to path $\tau$ is the sequence of NBA states that are visited when the robots follow $\tau$. Every time we visit a new state in the NBA while following $\tau$,  we add the node in the tree $\bbq(t)=[\bbp(t), \bbs(t), q_B(t)]$ at that time instant to a set $\mathbb{T}$. In other words $\mathbb{T}$ consists of nodes in the tree at which point we have transitioned to a new state $q_B$ in the NBA. 

At any time $t$, if one or more abilities of robots fail during the mission, Algorithm \ref{alg:RP} is executed. If the failure affects the mission in any way, the necessary robot reassignments will be reflected in the NBA. Thus at the end of the reassignment, if a transition is affected then it will result in different robots enabling the transition to the next state. We then compare for states in $\rho_B$ the  

We then run the sampling-based planner again from the current robot positions (\bbp(t)) and the current state in the NBA ($q_{curr}$)to generate a new path $\tau=\tau(t)\dots\textcolor{blue}{\tau(\infty)}$, that satisfy $\phi$
% sequence $\bbu_{t:H}$ of control inputs $\bbu(\hat{t})$, for all $\hat{t}\in\set{t,\dots,H}$, that satisfy $\phi$. 
\textcolor{blue}{[self note: maybe mention here that planner picks $\hat\sigma$ such that $\hat\sigma$ has a valid assignment. For example, in Example \ref{ex:LTL_trans} if originally $\hat{\sigma}=\sigma_2$ and say robot $2$ and robot $3$ failed, then BFS will be able to find a solution only for $\sigma_1$, by replacing robot $2$ with robot $5$. In that case, when we recall the sampling-based planner, the planner picks $\hat{\sigma}=\sigma_1$.]}

\textcolor{red}{[You are still missing a theoretical result here. As we discussed last time, you need to have a proposition here discussing that if a single failure happens then you can find a re-assignment that satisfies all the imposed constraints. Provide a short proof on this. then, discuss what happens if you have multiple failures. Not as a theorem (if you don't have a proof for this) but at least a discussion is needed. Then, provide at least a discussion on under what conditions there exist feasible paths for the new assignment.]}

==> files/notes.tex <==

%%%%%%
\textcolor{magenta}{To prove this result, we will express the violation cost $\mathbb{C}_{\tau_\text{new}}$ of a plan $\tau_\text{new}$ (see \eqref{eq:violation}) generated by Alg. \ref{alg:local}, in terms of the assignment costs defined in \eqref{eq:assignmentCost}. Then, the result will follow by contradiction. 
Specifically, if there exists a different combination of task re-assignments that would allow a globally optimal temporal logic to compute a plan $\tau_{\text{new}}'$ with $\mathbb{C}_{\tau_{\text{new}}}\geq \mathbb{C}_{\tau_{\text{new}}'}$, it would imply that there exists at least one failed predicate that could have been repaired differently to achieve a lower assignment cost. This, however, contradicts Proposition \ref{prop:opt1}.}

%Specifically, if there exists a different combination of task re-assignments that would allow a global optimal temporal logic to compute  a plan  $\tau_{\text{new}}'$ with $\mathbb{C}_{\tau_{\text{new}}}\geq \mathbb{C}_{\tau_{\text{new}}'}$ that would imply that there exists at least one failed predicate that could have been repaired differently so that it can achieve a lower assignment cost. This however is not possible due to Proposition \ref{prop:opt1}.

%$B$ be the revised NBA after implementing Alg. \ref{alg:RP} and 
\textcolor{magenta}{Let $\tau_{\text{new}}$ be the plan generated by Alg. \ref{alg:local} associated with a violation cost $\mathbb{C}_{\tau_{\text{new}}}$ (see \eqref{eq:violation}) and a sequence of NBA states $\ccalP^{\tau_{\text{new}}}$ (see Section \ref{sec:onlineReplan}). For simplicity, hereafter, we simply denote 
$\ccalP^{\tau_{\text{new}}}$ by $\ccalP^{\text{new}}$. Due to Assumption \ref{cond:NBA_self_loop}, following the same logic used in the proof of Proposition \ref{prop:optiLVP} (see Case I), we conclude that 
%
\begin{equation}
\mathbb{C}_{\tau_{\text{new}}}=\ccalC_{\ccalP^{\text{new}}}=
%
\sum_{m=1}^{|\ccalC_{\ccalP^{\text{new}}}|-1} \ccalC_{\sigma_{\ccalP^{\text{new}}(m),\ccalP^{\text{new}}(m+1)}},
\end{equation}
where the last inequality is due to \eqref{eq:NBAviolation}.}
%
%
%Also, let $B'$ be an NBA revised using any combination of task re-assignments. Let $\tau_{\text{new}}'$ be the plan with the minimum violation cost, as per \eqref{eq:violation}, generated by any optimal temporal logic planner using the NBA $B'$. Let 
%$\mathbb{C}_{\tau_{\text{new}}'}$ be the cost of $\tau_{\text{new}}'$.  Our goal is to show that $\mathbb{C}_{\tau_{\text{new}}}\leq \mathbb{C}_{\tau_{\text{new}}'}$. We will show this by contradiction.

%Assume that there exists a combination of task re-assignment, different from the one generated by Alg. \ref{alg:RP}-\ref{alg:local}, that can yield an optimal plan $\tau_{\text{new}}'$ satisfying 
%\begin{equation}\label{eq1}
%\mathbb{C}_{\tau_{\text{new}}}\geq \mathbb{C}_{\tau_{\text{new}}'}.
%\end{equation}
%$\mathbb{C}_{\tau_{\text{new}}}\geq \mathbb{C}_{\tau_{\text{new}}'}$. 

%Let $\ccalP_{\text{min}}$ and $\ccalP_{\text{min}}'$ be sequences of NBA states, constructed as described in Section \ref{sec:onlineReplan}, using the NBA $B$ and $B'$, respectively. As shown in the proof of Proposition \ref{prop:optiLVP}, if the Alg. \ref{alg:local} does not trigger global replanning, then  $\mathbb{C}_{\tau_{\text{new}}}=\mathbb{C}_{P_{\text{min}}}$. Thus, \eqref{eq1} yields
%\begin{equation}\label{eq2}
%\mathbb{C}_{P_{\text{min}}}\geq \mathbb{C}_{\tau_{\text{new}}'}.
%\end{equation}

%Due to \eqref{eq:NBAviolation}, we have that
%\begin{equation}\label{eq3}
%\sum_{m=1}^{|\ccalP_{\text{min}}|} \mathbb{C}_{\sigma_{\ccalP_{\text{min}}(m),\ccalP_{\text{min}}(m+1)}}\geq \mathbb{C}_{\tau_{\text{new}}'}.
%\end{equation}

\textcolor{magenta}{
Consider a transition $e=(\ccalP^{\text{new}}(m),\ccalP^{\text{new}}(m+1))$, for some $m$. By definition of the cost function $\mathbb{C}_{\sigma_{\ccalP^{\text{new}}(m),\ccalP^{\text{new}}(m+1)}}$ in \eqref{eq:edgeviolation},  we have that $\mathbb{C}_{\sigma_{\ccalP^{\text{new}}(m),\ccalP^{\text{new}}(m+1)}}$ is equal to the total assignment cost incurred to fix that NBA transition from the initial time step till the current time step $t$, i.e., the sum of assignment costs, as per \eqref{eq:assignmentCost}, incurred every time that edge had to be repaired.\footnote{If that edge never required repairing, then that cost $0$.} \textcolor{green}{[is this true? how to formally show this? This could be a different proposition..]} Notice that unassigned predicates in an edge $e$ may arise due to the failures occurred at the current time step $t$ as well as due to past failures $\bar{t}<t$. Thus, we get that: 
%
\begin{equation}\label{eq5}
    \mathbb{C}_{\sigma_{\ccalP^{\text{new}}(m),\ccalP^{\text{new}}(m+1)}}=\mathbb{C}_{q_B',q_B'',d}^{\pi}+\mathbb{C}_{e,\text{past}},
\end{equation}
where with slight abuse of notation $\mathbb{C}_{e,\text{past}}$ denotes the assignment costs incurred due to repairs in edge $e$ at time steps $\bar{t}<t$. Notice that $\mathbb{C}_{e,\text{past}}$ cannot be affected by the repairs occurred at current time step $t$, as unassigned predicates that come from past time steps $\bar{t}<t$ will remain un-assigned in the future.\textcolor{green}{[is this true? If so, why don't we attempt to assign them in the future once more failures occur? Maybe these past unassigned predicates are more important than the current failed predicates.]}
%
Also, in \eqref{eq5}, $\mathbb{C}_{q_B',q_B'',d}^{\pi}$ denotes the current assignment cost to fix the currently failed predicate $\pi$ in the edge $e=(\ccalP^{\text{new}}(m),\ccalP^{\text{new}}(m+1))$. The superscript $d$ refers to the $d$-th conjunction, when the Boolean formula $b_{\ccalP^{\text{new}}(m),\ccalP^{\text{new}}(m+1)}$ is written in DNF, that the plan $\tau_{\text{new}}$ satisfies.
%\footnote{Observe that the superscript in $\mathbb{C}_{\pi,e}^1(p)$ is $1$, and not $d$ as in \eqref{eq:assignmentCost}, because by definition of $\ccalP^{\text{new}}$, we have that  $b_{\ccalP^{\text{new}}(m),\ccalP^{\text{new}}(m+1)}$, i.e.,  the Boolean formula associated with the NBA transition from $\ccalP^{\text{new}}(m)$ to $\ccalP^{\text{new}}(m+1)$, when written in DNF, consists of a single conjunction of one or more literals.}
%
Thus, we get that:}

\textcolor{magenta}{\begin{equation}\label{eq6}
\mathbb{C}_{\tau_{\text{new}}}=\sum_{e\in\ccalE_{\ccalP^{\text{new}}}}(\mathbb{C}_{q_B',q_B'',d}^{\pi}+\mathbb{C}_{e,\text{past}})
\end{equation}
where $\ccalE_{\ccalP^{\text{new}}}$ is a set that collects all edges incurred in $\ccalP^{\text{new}}$, i.e.,
$\ccalE_{\ccalP^{\text{new}}}=\{\ccalP^{\text{new}}(m),\ccalP^{\text{new}}(m+1)\}_{m=1}^{|\ccalP^{\text{new}}|-1}$.}

\textcolor{magenta}{The result in \eqref{eq6} allows us to express the cost of a plan in terms of assignment costs defined in \eqref{eq:assignmentCost}. Thus, if there exists a different combination of assignments that would allow Alg. \ref{alg:local} to compute a better plan $\tau_{\text{new}}'$, it means that there exists at least one edge in the automaton that would could have been repaired differently so that it can achieve a lower cost than the one achieved by Alg. \ref{alg:bfs}. However, this contradicts Proposition \ref{prop:opt1}. Also, since there does not exist a different combination of assignments that would allow Alg. \ref{alg:local} to compute a better plan, then, due to Proposition \ref{prop:optiLVP}, we conclude that there does not exist a different combination of assignments that would allow any other optimal global optimal temporal logic planner to compute a better plan. This completes the proof.}

==> files/solution_v2.tex <==
\vspace{-0.1cm}
In this section, we outline the proposed \textcolor{black}{minimum-violation} algorithm for addressing Problem \ref{prob_statement}. Our solution comprises of three components. First, we create an offline path $\tau$ that satisfies $\phi$ using existing LTL planners \cite{luo2021abstraction}. \textcolor{black}{In the second part, we use the concepts of \cite{kalluraya2023resilient_arxiv} to set up all the constraints needed for the task reallocation process; see Sec. \ref{sec:taskRealloc0}-\ref{sec:taskRealloc2}.
We then reason about robot failures and reassign sub-tasks to operational robots, while minimizing the total number of sub-task re-allocations; see Sec. \ref{sec:taskRealloc3}. Unlike \cite{kalluraya2023resilient_arxiv}, the proposed algorithm can address cases where feasible task re-allocations cannot be made due to a limited number of available robots. This is achieved by strategically prioritizing assignment of tasks/predicates with high penalty scores (see Definition \ref{def:penalty}).} Once the LTL formula is revised, according to the reassignments, we implement an online re-planning method that designs minimum violation plans as per \eqref{eq:violation}; see Sec \ref{sec:onlineReplan}.


%We note that the major difference with \cite{kalluraya2023resilient_arxiv} is in the problem setup, where in this paper, we assume the possibility that a limited number of operational robots are available after robot failures. Specifically, unlike \cite{kalluraya2023resilient_arxiv}, the proposed algorithm can address cases where feasible task re-allocations cannot be made due to a limited number of available robots; see Sec. \ref{sec:taskRealloc3}.} Once the LTL formula is revised according to the reassignments, we implement an online re-planning method that designs plans that have the lowest violation score along the plan; Sec \ref{sec:onlineReplan}.

% In this section we present an algorithm to solve Problem \ref{prob_statement}. Our solution consists of three parts. In the first part, we generate offline a path $\tau$ satisfying $\phi$ using our recently proposed sampling-based planner \cite{luo2021abstraction}; see Sections \ref{sec:nba}-\ref{sec:samplingAlg}. In the second part, %we provide a framework to reason about whether a failure of a robot capability  disrupts feasibility of the current plan $\tau$. If so, in the third part,
% we design an online local task re-allocation algorithm re-assigning sub-tasks to robots. The proposed algorithm is \text{local} in the sense that it aims to minimize the total number of sub-task re-allocations that have to happen due to the failed skill; see Sections \ref{sec:taskRealloc0}-\ref{sec:taskRealloc3}. Given the revised LTL formula, we propose an online re-planning method 
% that locally revises the current robot paths to design new feasible ones. %minimally disrupt the previously designed paths. %The proposed algorithm is also summarized in Alg. \ref{alg:plan}.
% % \textcolor{red}{[Samarth, please add references to lines of the algorithm 1,2, and 3 throughout the paper ]} 
% % In Section \ref{sec:analysis}, we analyze correctness, completeness, and optimality of the proposed algorithm as well as its limitations. %Examples illustrating the proposed algorithm can be found in \textcolor{red}{[X]}.

%\begin{algorithm}[t]
%\caption{Resilient Mission Planning}
%\LinesNumbered
%\label{alg:plan}
%\KwIn{ LTL mission $\phi$ }
%\KwOut{Mission plan $\tau\models\phi$}
%% reassign\_flag = False\;
%%\textit{Offline Part}\\
%Convert $\phi$ into an NBA and design a plan $\tau\models\phi$ \;\label{plan:nba}%(\textit{offline})
%%\textit{Online Part}\;
%\For{$t=0,1\dots,$}{
%Apply $\tau(t)$\;\label{plan:applyTau}
%\If{\text{Failures occur at time} $t\geq0$}{
%\If{\text{Failures are critical}}{
%Revise the mission plan $\tau$ (Alg. \ref{alg:RP})\;\label{plan:revise}
%}
%}
%}
%\end{algorithm}

%The first part of the solution is a sampling-based planner that we have developed in our previous work \cite{luo2021abstraction}. In this algorithm, given a mission specification $\phi$, and the robot dynamics, the planner can generate a sequence of control inputs $\bbu(\hat{t})$, for all $\hat{t}\in\set{0,\dots,H}$, that satisfy $\phi$. This however does not have any provision for robot failures during the mission. While our previous work considers uncertainty in the environment, for sake of simplicity to explain our current approach we assume that there is no uncertainty in the environment.

%In the second part of our solution we extend our planning algorithm to be resilient to robot failures. In the event of a failure in $rob_j$ at time $t$, our objective is to pick another robot $rob_g\in\bbT_q$, $g\in\{1,\dots,N\}$, $g\neq j$, that can replace $rob_j$ in the affected atomic predicate $\pi_{\bbT_q}^p$. In case of multiple abilities in multiple robots failing at the same time, the objective is to replace the robots in all the affected atomic propositions. We then generate a new sequence of control inputs $\bbu_{t:H}$ for only those robots that are assigned new atomic predicates such that $\phi$ is satisfied.   


\vspace{-0.2cm}
\subsection{Offline Temporal Logic Planning}\label{sec:samplingAlg}
\vspace{-0.1cm}
Given an LTL task $\phi$, we generate offline a feasible plan $\tau_H$ a using a sampling-based planner \cite{luo2021abstraction}. We select this planner due to its scalability and abstraction-free benefits. Its key idea is to build trees incrementally that explore both the multi-robot motion space and the automaton state-space. This planner is asymptotically optimal, i.e., if $\phi$ is feasible, then as the tree grows, the probability of finding the optimal path with a respect to a cost function (e.g., \eqref{eq:violation}) goes to one. % 
Alternative temporal logic planners with finite-time guarantees can also be used \cite{gujarathi2022mt}.


\vspace{-0.2cm}
\subsection{Setting Up the Online Task Reallocation Process}\label{sec:taskRealloc0}
%\textcolor{red}{[Not sure if this title is appropriate but we needed to break that long sections into smaller ones]}
\vspace{-0.1cm}
As the robots execute $\tau_H$, assume that at time $t$ a sub-set of robot capabilities fail, resulting in the new vector $\bbZ_j(t)$ for some robots $j\in\ccalR$. %\textcolor{red}{[what is $\ccalR$? Is it defined anywhere? Maye we should delete it]}\textcolor{cyan}{$\ccalR$ is defined in Sec. II A, as $j\in\ccalR=\{1,...,N\}$}
% Assume that a feasible plan $\tau$ has been generated as in Section \ref{sec:samplingAlg}. Consider the case where, as the robots execute the plan $\tau$, a sub-set of robot capabilities fail at an a priori unknown time $t$ resulting in new vectors $\bbZ_j(t)$ for some robots $j\in\ccalR$. 
%Assume that the occurred failures are critical and, therefore, the current mission plan is not feasible.
Consider a set $\mathcal{AP}_F\subseteq\mathcal{AP}$ collecting atomic predicates $\pi_{\ccalT_c}(j,c,\ell_e)$ in $\phi$ that cannot be satisfied due to skill failures and the current predicate-robot assignments. We refer to these predicates as 'failed' atomic predicates. 
\textcolor{black}{Our first goal is to re-assign failed predicates to robots with the required function skills; see Alg. \ref{alg:RP}.} %presents our approach to find a reassignment that solves all these failures.
The following process is individually applied to all failed atomic predicates (either in parallel or sequentially) (line \ref{rp:for1}, Alg. \ref{alg:RP}). %\textcolor{red}{[You need a sentence somewhere earlier saying something along the lines `this process is summarized in Alg. 1']}
% Let $\mathcal{AP}_F\subseteq\mathcal{AP}$ be a set collecting all atomic predicates $\pi_{\ccalT_c}(j,c,\ell_e)$ in $\phi$ that can never be true due to the failed skills, given the current assignment of predicates to robots.\footnote{Negated predicates of the form $\neg\pi_{\ccalT_c}(\varnothing,c,\ell_e)$ are not included in $\mathcal{AP}_F$ as such predicates refer to the whole team $\ccalT_c$ and not a specific robot. As a result, it is not meaningful to re-assign them.} With slight abuse of terminology, we refer to $\pi_{\ccalT_c}(j,c,\ell_e)\in\mathcal{AP}_F$ as a `failed' atomic predicate. The following process is repeated for all failed atomic predicates \textcolor{black}{sequentially and in any order (line \ref{rp:for1}, Alg. \ref{alg:RP})}. %\textcolor{red}{[Could this also be done in p]}


%Our goal is to re-allocate tasks to the robots based on their currently active skills; see also Alg. \ref{alg:RP}. %, i.e., it aims to perform the minimum re-assignments of sub-tasks (i.e., atomic predicates of the form \eqref{eq:pip}) to robots. 
%\textcolor{red}{[If we agree on this description we need a new algorithm to summarize it.]}
%
%The transition between any two consecutive states $q_B$ and $q_{B}^{\prime} \in \ccalQ_{B}$ in the NBA is governed by a Boolean $b_{q_B,q_{B}^{\prime}}$. The Boolean is defined over the atomic predicates which when satisfied enables the transition from $q_B$ to $q_{B}^{\prime}$. 
%Let $\sigma_b$ represent a combination of truth values for the atomic predicates which can satisfy the Boolean ($\sigma_b\models b_{q_B,q_{B}^{\prime}}$).
%$\Sigma_{q_B,q_{B}^{\prime}}$ is the set of all such combinations $\sigma_b$ that satisfy the Boolean $b_{q_B,q_{B}^{\prime}}$. We arbitrarily pick $\hat{\sigma}\in\Sigma_{q_B,q_{B}^{\prime}}$ that is referenced by our sampling-based planner (Sec \ref{sec:samplingAlg}) as the set of predicates that need to be satisfied to enable the transition. 
%To understand this we will refer to the following example:


%To re-assign tasks to the robots, we repeat the following process for each pair of failed capability and associated robot, i.e., for each $\zeta_c^j$ that switched from $1$ to $0$, at time $t$. 
%
Our aim is to reassign $\pi_{\ccalT_c}(j,c,\ell_e)\in\mathcal{AP}_F$ to a different robot $i\in\ccalT_c$, a process we informally call 'fixing/repairing'. If all robots $i\in\ccalT_c$ are potentially occupied with other sub-tasks (refer to Ex. \ref{ex:LTL}), repairing the failed predicate may trigger a sequence of task reassignments, where fixing the failed predicate requires robot $i\in\ccalT_c$ to take over, which may, in turn, necessitate another robot to assume the sub-task originally assigned to robot $i$ and so on until all sub-tasks are reassigned. 
%
% Our goal is to re-assign $\pi_{\ccalT_c}(j,c,\ell_e)\in\mathcal{AP}_F$ to a new robot $i\in\ccalT_c$; again, with slight abuse of terminology, we also refer to this process as `fixing/repairing' the failed predicate. Informally, the key challenge here is that possibly all robots $i\in\ccalT_c$ may be busy with other sub-tasks; see Ex. \ref{ex:LTL}. In this case, repairing the failed predicate may trigger a sequence of task re-assignments. The reason is that fixing the failed predicate requires another robot $i\in\ccalT_c$ to take over it while, at the same time, another robot may have to take over the sub-task that was originally assigned to robot $i$ and so on until there are no unassigned sub-tasks. Our goal is to fix the failed predicate by making the minimum possible number of task re-assignments to minimally disrupt mission planning.  
%
\textcolor{blue}{A new challenge arising here, compared to \cite{kalluraya2023resilient_arxiv}, is the potential situation where there may not be any available robot capable of taking over failed predicates. This implies the necessity of sacrificing the completion of one sub-task/predicate, incurring a penalty. In this case, we want to re-allocate tasks so that the unassigned predicates, i.e., the ones that will not be satisfied, are the ones with the smallest penalty given by $F$} (see Section \ref{sec:PFLTLMission}). %In such a case our goal is to start the re-assignment sequence from the task with the lowest penalty, as no robot will be assigned to this task. In case the original failed task has the lowest penalty, then we will not re-assign it to another robot.} 

Let $q_B^\text{cur}=q_B(t)$ represent the current NBA state of the robots at time $t$, when executing plan $\tau_H$. If failures occur at that time, given a failed predicate $\pi_{\ccalT_c}(j,c,\ell_e)$, we calculate all the NBA states can be reached from $q_B^\text{cur}$ using a multi-hop path. We collect these states, including $q_B^\text{cur}$, in a set called $\hat{\ccalQ}_B^{\text{cur}}\subseteq\ccalQ_B$. Let $e=(q_B',q_B'')$ denote an NBA transition from $q_B'$ to $q_B''$, if $\pi_{\ccalT_c}(j,c,\ell_e)$ appears in the corresponding Boolean formula $b_{q_B',q_B''}$ , where $q_B',q_B''\in\hat{\ccalQ}_B^{\text{cur}}$; (line \ref{rp:collect}, Alg. \ref{alg:RP}).  Let $\ccalE$ be a set collecting all such edges $e$.


% Let $q_B^\text{cur}=q_B(t)$ be the NBA state that the robots are currently in (as per the current plan $\tau_H$) at time $t$ when failures occur.
% Given a failed predicate $\pi_{\ccalT_c}(j,c,\ell_e)$, we compute all NBA states that can be reached from $q_B^\text{cur}$ through a multi-hop path. This step can be implemented by treating the NBA as a directed graph and checking which states $q_B'\in\ccalQ_B$ can be reached from $q_B^\text{cur}$. We collect these states (including $q_B^\text{cur}$) in a set $\hat{\ccalQ}_B^{\text{cur}}\subseteq\ccalQ_B$.
% Then, among all NBA transitions between states  $q_B',q_B''\in\hat{\ccalQ}_B^{\text{cur}}$, we collect in a set $\ccalE$ the ones for which $\pi_{\ccalT_c}(j,c,\ell_e,\chi)$ appears in the corresponding Boolean formula $b_{q_B',q_B''}$ (line \ref{rp:collect}, Alg. \ref{alg:RP}). 
% With slight abuse of notation, let $e=(q_B',q_B'')$ denote an edge in $\ccalE$ (i.e., an NBA transition from $q_B'$ to $q_B''$). 
% Given the edge $e\in\ccalE$, we define the Boolean formula $b_{q_B',q_B''}$ defined over $\mathcal{AP}$ for which it holds that if $q_B''\in\delta_B(q_B',\sigma)$, for some $\sigma\in\Sigma$, then $\sigma\models b_{q_B',q_B''}$ and vice versa. 



%
\vspace{-0.2cm}
\subsection{\textcolor{black}{Constraints for Task Reallocation}}\label{sec:taskRealloc2}
\vspace{-0.1cm}
%With slight abuse of notation, let $e=(q_B',q_B'')$ denote an edge in $\ccalE$ (i.e., an NBA transition from $q_B'$ to $q_B''$). We repeat the following steps for each edge in $\ccalE$. We first focus on self-loop edges (if any) since, as it will be explained later, fixing the predicates on the remaining transitions where $q_B'\neq q_B''$, depends on the fixed predicates on the self loops of $q_B'$. We assume that $\ccalE$ is an ordered set where the self-loop edges appear first (in any order), followed by the remaining edges (in any order).

%the set $\Sigma_{q_B',q_B''}\subseteq\Sigma$ that collects symbols required to enable a transition from $q_B'$ to $q_B''$, i.e., $\Sigma_{q_B',q_B''}=\{\sigma\in\Sigma~|~q_B''\in\delta_B(q_B',\sigma)\}.$ In fact, an NBA transition from $q_B'$ to $q_B''$ can be activated only if a Boolean formula, denoted by $b_{q_B',q_B''}$ defined over $\mathcal{AP}$ is satisfied. Thus, $\Sigma_{q_B',q_B''}$ can be constructed by collecting all symbols $\sigma\in\Sigma$ that satisfy $b_{q_B',q_B''}$; see also Example \ref{ex:LTL_trans}.
%
%Also, from $\Sigma_{q_B',q_B''}$, we exclude symbols associated with robots that do not play any role in satisfying $b_{q_B',q_B''}$. For instance, if $b_{q_B',q_B''}=(\pi_{\ccalT_c}(j,c,\ell_e)\vee\pi_{\ccalT_m}(r,m,\ell_e))\wedge\neg\pi_{\ccalT_f}(\varnothing,f,\ell_p)$, then $\Sigma_{q_B',q_B''}$ includes only the symbols that can be generated exclusively by robots in teams $\ccalT_c$, $\ccalT_m$, and $\ccalT_f$. %\textcolor{red}{[probably we don't need the definition of $\Sigma_{q_B',q_B''}$ ]}

 %; the following discussion also explains why self-loops are excluded from the set $\ccalE$. 


\begin{algorithm}[t]
\footnotesize
\caption{Minimum-Violation Task Re-allocation}
\LinesNumbered
\label{alg:RP}
\KwIn{ (i) NBA $\ccalB$, (ii) Current NBA state $q_B^{\text{cur}}$; (iii) Set of failed predicates $\mathcal{AP}_F$}
\KwOut{Revised NBA}
% reassign\_flag = False\;

\For{every $\pi\in\mathcal{AP}_F$}{\label{rp:for1}
Define the ordered set of edges $\ccalE$\;\label{rp:collect}
\For{every $e=(q_B',q_B'')\in\mathcal{E}$}{\label{rp:for2}
    Rewrite: $b_{q_B',q_B''}=\bigvee_{d=1}^D b_{q_B',q_B''}^d$\;\label{rp:DNF} 
    \For{$d=1,\dots,D$}{\label{rp:for3}
    % \textcolor{black}{Will need to update $\ccalG$ as after failures teams will be different}\;
    Define $\ccalG$ and functions $V^{d}_{q_B',q_B''}, g^{d}_{q_B',q_B''}$\;\label{rp:graph}
    % Compute constraints $\ccalG$\;\label{rp:constraints}
    Apply Alg. \ref{alg:bfs} to compute a sequence of re-assignments $p=p(0),\dots,p(P)$\;\label{rp:applyBFS}
    % \If{$\exists p$}{
    Re-assign atomic predicates as per $p$\;\label{rp:reassign}
    % }
    % \Else{
    % Assign $\pi=\text{False}$\;\label{rp:no_sol}
    % }
    Revise $b_{q_B',q_B''}^d$\;
    }
    }
    }
% Among all nodes in $\ccalX_g$, find $\bbq_{\text{end}}(t_{\text{end}})$ \; \label{rrt:node}
% $H=t_{\text{end}}$ and recover $\bbu_{0:H}$ by computing the path $\bbq_{0:t_{\text{end}}}= \bbq(0), \dots, \bbq(t_{\text{end}}) $\;\label{rrt:solution}
\vspace{-0.05cm}
\end{algorithm}
\setlength{\textfloatsep}{2pt plus 0pt minus 2.0pt}

To maintain the feasibility of the LTL formula, it is necessary that $b_{q_B',q_B''}$ can be satisfied after re-allocation, $\forall e=(q_B',q_B'')\in\ccalE$. %; see Rem. \ref{rem:limitations}. %That is,  there must be a symbol $\sigma=L([\bbp,\bbs])$ produced by the robots that fulfills the modified formulas $b_{q_B',q_B''}$ resulting from task re-assignment.
Similar to \cite{kalluraya2023resilient_arxiv}, our approach inspects all edges $e\in\ccalE$, and reassigns predicates appearing in the respective formulas $b_{q_B',q_B''}$. However, unlike \cite{kalluraya2023resilient_arxiv}, our approach can handle cases where $b_{q_B',q_B''}$ cannot be satisfied. Specifically, instead of reporting `assignment failure', it aims to compute a task reassignment that minimizes an assignment penalty function defined later using $F$.
We refer to this process as minimum-violation task re-allocation.
%allows for unsatisfiable predicates in the Boolean to be considered true by taking a penalty given by the mapping $\ccalF$ thus being able to generate a solution that partially satisfies the mission by taking on some penalty. 
  
% The key idea in our approach is to inspect all edges $e\in\ccalE$ and re-assign the predicates appearing in the respective formulas $b_{q_B',q_B''}$ so that there is no unassigned predicate and that the resulting LTL formula remains feasible (i.e., the robots can still generate paths that yield accepting NBA runs). In case there is no feasible solution and we are forced to leave a certain predicate unassigned, then those predicates should have the lowest penalty.%Toward achievinf the latter,
% A necessary condition to preserve the feasibility of the LTL formula after task re-allocation is that $b_{q_B',q_B''}$ should be feasible (i.e., it can become `true') after task reallocation, $\forall e=(q_B',q_B'')\in\ccalE$; see also Rem. \ref{rem:limitations}. 
% With slight abuse of notation, if we have a predicate to which no robot is assigned, and thus we activate it's associated penalty, we say that the predicate is true but with a penalty equal to the $\chi$ of that predicate. Thus the LTL formula is feasible albeit with the penalty equal to the sum of all the activated penalties in that transition.
% In other words, there should exist a symbol $\sigma=L([\bbp,\bbs])\in\Sigma$ generated by the robots, that satisfies the revised formulas $b_{q_B',q_B''}$ arising after task re-assignment. 
% \textcolor{blue}{(alternately we can have a new definition for predicate with penalty $\pi_{\ccalT_c}(\chi,c,\ell_e,\chi)$ where robot $j$ is replaced by penalty value. And thus say that this predicate is always true)}

Next, we translate this requirement into constraints that should be respected when a failed predicate is repaired in an edge $e=(q_B',q_B'')$. %These constraints are similar to the constraints discussed in our previous work and more details and examples can be found in \cite{kalluraya2023resilient_arxiv}.
Essentially we re-write the Boolean $b_{q_B',q_B''}$ in a disjunctive normal form (DNF), i.e., $b_{q_B',q_B''}=\bigvee_{d=1}^Db_{q_B',q_B''}^d$, for some $D>0$ and for each Boolean formula $b_{q_B',q_B''}^d$, we define the set $\ccalR_{q_B',q_B''}^d\subseteq\ccalR$ that collects robots that appear in $b_{q_B',q_B''}^d$.
We further define the set $\mathcal{AP}_i$ that collects all predicates that appear in $b_{q_B',q_B''}^d$ assuming that the ones that are associated with skills $c$ for which $\zeta_c^i(t)=1$ are all assigned to robot $i$. Using $\mathcal{AP}_i$, we construct the alphabet $\Sigma_i=2^{\mathcal{AP}_i}$. Then we define following functions that help model the task re-allocation constraints

% Accordingly, we set up constraints that should be respected when a failed predicate is repaired in an edge $e=(q_B',q_B'')$.% (where  $q_B'$ may coincide with $ q_B''$).   
% To this end, we re-write the Boolean $b_{q_B',q_B''}$ in a disjunctive normal form (DNF), i.e., $b_{q_B',q_B''}=\bigvee_{d=1}^Db_{q_B',q_B''}^d$, for some $D>0$.\footnote{The failed predicate may appear in more than one sub-formula $b_{q_B',q_B''}^d$ but it will be repaired separately/independently for each sub-formula; see Remark \ref{rem:independ}.}
% %
% For each Boolean formula $b_{q_B',q_B''}^d$, we define the set $\ccalR_{q_B',q_B''}^d\subseteq\ccalR$ that collects robots that appear in $b_{q_B',q_B''}^d$; see also Ex. \ref{ex:Rg}. %Then we define the following function 
% %and the function $V_{q_B',q_B''}^d$ exactly as above; see also Example \ref{ex:Vi}.
% Given $b_{q_B',q_B''}^d$, we also define the set $\mathcal{AP}_i$ that collects all predicates of the form \eqref{eq:pip} that appear in $b_{q_B',q_B''}^d$ assuming that the ones that are associated with skills $c$ for which $\zeta_c^i(t)=1$ are all assigned to robot $i$. \textcolor{black}{Given $\mathcal{AP}_i$, we can construct the alphabet $\Sigma_i=2^{\mathcal{AP}_i}$.} For instance, if $b_{q_B',q_B''}^d=\pi_{\ccalT_c}(j,c,\ell_e)\wedge\pi_{\ccalT_m}(i,m,\ell_f)$, then $\mathcal{AP}_i=\{\pi_{\ccalT_c}(i,c,\ell_e), \pi_{\ccalT_m}(i,m,\ell_f) \}$ if $i\in\ccalT_m\cap\ccalT_c$ %\footnote{ }
% %
% \textcolor{black}{ and $\Sigma_i=\{\pi_{\ccalT_c}(i,c,\ell_e),\pi_{\ccalT_m}(i,m,\ell_f), \pi_{\ccalT_c}(i,c,\ell_e)\pi_{\ccalT_m}(i,m,\ell_f),\epsilon\}$, where $\epsilon$ stands for the empty symbol.}
% Then, we define following function modeling task re-allocation constraints.


\begin{definition} [Function $V_{q_B',q_B''}^d$]\label{def:constrainedSet}
\textcolor{black}{The set-valued function $V_{q_B',q_B''}^d:\ccalR\rightarrow \Sigma_i$, given as input a robot index $i\in\ccalR$, returns a set collecting all symbols $\sigma_i\in\Sigma_i$ that if robot $i\in\ccalR$ generates, then $b_{q_B',q_B''}^d$ will be `false' regardless of the values of the other predicates}. %$\mathcal{AP}_i$ is a subset of $\mathcal{AP}$ collecting all predicates associated with robot $i$ that appear in.
%
We define $V_{q_B',q_B''}^d(i)=\emptyset$ for all robots $i\in\ccalR\setminus\ccalR_{q_B',q_B''}^d$. 
\end{definition}

The sets $V^d_{q_B',q_B''}(i)$ capture \textit{constraints} on what tasks/predicates a robot $i$ can take over. Specifically, if robot $i\in\ccalR_{q_B',q_B''}^d$ took over predicates that appear in $V^d_{q_B',q_B'';}(i)$, it would falsify $b_{q_B',q_B''}^d$. \textcolor{blue}{See Example \ref{ex:LTL} and Fig. \ref{fig:bfs}.} 
We also define the function $g_{q_B',q_B''}^d$ to determine which predicates robots are currently assigned to.

\begin{definition} [Function $g_{q_B',q_B''}^d$]
The function $g_{q_B',q_B''}^d:\ccalR\rightarrow \mathcal{AP}$, given as an input a robot index $i\in\ccalR$, returns a set collecting the atomic predicates that are assigned to robot $i$ in $b_{q_B',q_B''}^d$ excluding the negated ones and the failed predicate.\footnote{There is at most one predicate assigned to a robot $i\in\ccalR_{q_B',q_B''}^d$ as all NBA transitions requiring a robot to satisfy more than one predicate at a time are pruned; see Section \ref{sec:nba}.} We define $g(i)=\varnothing$, for all robots $i\not\in\ccalR_{q_B',q_B''}^d$ and for all robots $i\in\ccalR_{q_B',q_B''}^d$ appearing in negated predicates or in the failed predicate. %\textcolor{black}{and $g(i)=\varnothing$, for all $i\not\in\ccalR_{q_B',q_B''}^d$}.
\end{definition}

% \begin{ex}[Function $g_{q_B',q_B''}^d$, $V_{q_B',q_B''}^d$ and sets $\ccalR_{q_B',q_B''}^d$]\label{ex:Rg}
% Consider the LTL formula given in Example \ref{ex:LTL}. We focus on an NBA transition with: $b_{q_B',q_B''}^{d}=\pi_2\wedge\pi_5\wedge\neg\pi_4$, where recall  
% $\pi_2=\pi_{\ccalT_3}(2, c_3, \ell_2)$, $\pi_5=\pi_{\ccalT_5}(5, c_5, \ell_5)$, and $\pi_4=\pi_{\ccalT_2}(\varnothing, c_1, \ell_2)$.
%  \textcolor{black}{Then, $\ccalR_{q_B',q_B''}^d=\{2,5\}\cup\ccalT_2$.} Also, $g_{q_B',q_B''}^d(i)=\varnothing$, for all robots $i\in\ccalR_{q_B',q_B''}^d\setminus\{2,5\}$ and $g(2)=\pi_2$, $g(5)=\pi_5$. We also have $V_{q_B',q_B''}^d(i)=\emptyset$ for all $i\notin\ccalT_2$ and $V_{q_B',q_B''}^d(i)=\{\pi_{\ccalT_2}(i,c_1,\ell_2), \pi_{\ccalT_3}(i,c_3,\ell_2), \pi_{\ccalT_2}(i,c_1,\ell_2)\pi_{\ccalT_3}(i,c_3,\ell_2)\}$ for all $i\in\ccalT_2\cap\ccalT_3$. Notice that $\pi_{\ccalT_2}(i,c_1,\ell_2)$ and $\pi_{\ccalT_2}(i,c_1,\ell_2)\pi_{\ccalT_3}(i,c_3,\ell_2)$ are included because of $\neg\pi_{\ccalT_2}(\varnothing, c_1, \ell_2)$ in $b_{q_B',q_B''}^{d}$. Also, $\pi_{\ccalT_3}(i,c_3,\ell_2)$ is included because if robot \textcolor{black}{$1$ or} $4$ satisfies it, then \textcolor{black}{they} will be close to location $\ell_2$; therefore, $\pi_{\ccalT_2}(i,c_1,\ell_2)$ will also be satisfied resulting in violation of  $b_{q_B',q_B''}^{d}$.

% \end{ex}

% \begin{rem}[Excluding current self-loop]\label{rem:selfloop}
% Including the self-loop at $q_B^{\text{cur}}$ in $\ccalE$ (if it is eligible for inclusion) is unnecessary. The reason is that if the failed predicate results in falsifying $b_{q_B^{\text{cur}},q_B^{\text{cur}}}$, then, this subsequently, may result in either violating the LTL formula or enabling a transition to another NBA state. In other words, fixing the failed predicate in that self-loop will not let the robots stay in $q_B^{\text{cur}}$.
% \end{rem}
%their current NBA state $q_B^{\text{cur}}$. 
%\textcolor{red}{[possibly this discussion can be moved in the next subsection where we discuss correctness of the algorithm. here it might feel out of place to discuss why we ignore self loops; what we do (algorithm description) should be separate from why we do it this way (algorithm analysis)]}
%%
%Including self-loop edges in $\ccalE$ is unnecessary. To explain this, consider an edge $e=(q_B',q_B')$ in the NBA.
%%assume that $q_B'= q_B''$, i.e., the considered edge $e$ is a self-loop in the NBA. 
%The Boolean condition $b_{q_B',q_B'}$ for self-loops typically captures either requirements that should always hold (e.g., always avoid obstacles) and, therefore, they appear in every self-loop or they should temporarily (e.g., keep the camera on or stay in a certain area) hold until another event happens. In the latter case, these requirements appear in the self-loop Boolean conditions for a subset of NBA states. In either case, if a failed predicate exists in $b_{q_B',q_B'}$, then it is pointless to fix it, as $b_{q_B',q_B'}$ may get immediately violated %(unless $b_{q_B',q_B'}$ has the OR operator) 
%that may result in violation of the condition (i) that may either lead to violation of the LTL formula or trigger another NBA transition to a state $q_B''\neq q_B$.
%. We note that violation of condition (i) does not imply violation of the LTL formula as there may exist another NBA state $q_B''$ that can be reached from $q_B'$.
%In either case, fixing the failed predicate cannot let the robots stay in $q_B'$ as $b_{q_B',q_B'}$. Therefore, we focus on repairing failed predicates that exist only on edges  $e=(q_B',q_B'')$ where $q_B'\neq q_B''$. \textcolor{red}{[possibly this discussion can be moved in the next subsection where we discuss correctness of the algorithm. here it might feel out of place to discuss why we ignore self loops; what we do (algorithm description) should be separate from why we do it this way (algorithm analysis)]}


%\begin{ex}[Function $V^{d}_{q_B',q_B''}$]\label{ex:Vi}
%In what follows, we focus on sub-formulas $b_{q_B,}$
%(i) Consider the Boolean formula $b_{q_B',q_B''}^{d}=\pi_{\ccalT_c}(i,c,\ell_e)\wedge\neg\pi_{\ccalT_m}(\varnothing,m,\ell_e)$. (i.1) %Consider the Boolean formula $b_{q_B',q_B'}^d=\neg\pi_{\ccalT_c}(\varnothing,c,\ell_e)$. Then, $\ccalV_{q_B',q_B'}^{d,i}=\{\pi_{\ccalT_c}(i,c,\ell_e)\}$, for all $i\in\ccalT_c$.
%Assume $i\in\ccalT_m$. Then, $V_{q_B',q_B''}^{d}(i)=\{\pi_{\ccalT_m}(i,m,\ell_e)\}$. (i.2) 
% Assume $i\notin\ccalT_m$. Then, $V_{q_B',q_B''}^{d}(i)=\emptyset$ as there is no predicate that if robot $i$ satisfies, then $b_{q_B',q_B''}^{d,i}$ will be false. %(ii) Consider the Boolean formula $b_{q_B',q_B''}^{d}=\pi_{\ccalT_c}(i,c,\ell_e)\wedge(\neg\pi_{\ccalT_m}(\varnothing,m,\ell_e)\vee \neg\pi_{\ccalT_f}(\varnothing,f,\ell_e))$. Assume $i\in\ccalT_m\cap\ccalT_f$. In this case, $V_{q_B',q_B''}^{d}(i)=\emptyset$. 
% (ii)A particular transition in the NBA $q_B^{\prime}\rightarrow q_{B}^{\prime\prime}$ %(Fig. \ref{fig:LTL}) 
%is governed by the following Boolean formula (expressed in DNF) $b_{q_B^{\prime},q_{B}^{\prime\prime}}$ = $(\pi_1\land\pi_2\land\neg\pi_4)\lor(\pi_1\land\pi_3\land\neg\pi_4)$. We focus on 
%$b_{q_B^{\prime},q_{B}^{\prime\prime}}^1 = (\pi_1\land\pi_2\land\neg\pi_4)$. Then, for robot $4$ we have, $V_{q_B',q_B''}^{1}(4) = \{\pi_2,\pi_4,\textcolor{red}{\pi_2\pi_4}\}$; %\footnote{\textcolor{red}{[Since we are V collects symbols and not just predicates now (i this is more accurate) then we should include ${\pi_2\pi_4}$ too]}} 
% $\pi_4$ because of the presence of $\neg\pi_4$ in the Boolean, and $\pi_2$ because if robot 4 satisfies $\pi_2$ then $\pi_4$ will also be satisfied, thus violating the boolean.
%\mathcal{AP}_i\setminus\pi_{\ccalT_c}(i,c,\ell_e)$
%
%collects all atomic propositions in $\mathcal{AP}$ associated with robot $i$, denoted by $\mathcal{AP}_i\subseteq\mathcal{AP}$, except for $\pi_{\ccalT_c}(i,c,\ell_e)$.
%\textcolor{black}{[Is it  $\ccalV_{q_B',q_B'}^{d,i}$ or  $\ccalV_{q_B',q_B''}^{d,i}$]}\textcolor{red}{yes, i fixed it}
%
% \textcolor{black}{[If I understand (ii) correctly, if a robot $i$ is assigned to a predicate $\pi^1$ in the transition then, $\ccalV_{q_B',q_B'}^{d,i}$ is collecting all other predicates in the mission that have robot $i$ assigned to it? 
%
% \textcolor{red}{[No, this set collects all predicates that if robot $i$ satisfies then the Boolean formula is `false']}
%
% I didn't understand the purpose of adding these predicates to the set. \textcolor{red}{[The purpose is to create sets for each robot i that collect all subtasks/predicates that robot i cannot take because otherwise it will violate the formula (e.g., hitting an obstacle). Probably that definition is missing something (?); i think it may wrongly prevent robots from taking over some tasks ]}  I feel it might not allow us to do some valid reassignments. Let us say there are 3 predicates in the LTL mission $\pi^1 =\pi_{\ccalT_1}(1,1,\ell_1)$ $\pi^2 =\pi_{\ccalT_2}(2,2,\ell_2)$, and
% $\pi^3 =\pi_{\ccalT_2}(1,2,\ell_2)$. Assume a third robot robot 3 is free throughout the mission. Note that $\pi^2$ and $\pi^3$ are essentially the same tasks defined over different robots. Say we have a transition $\pi^1 \wedge \pi^2$. Suppose robot 2 fails, and technically a possible reassignment is 3->1->2, that is 3 does $\pi^1$ and 1 does $\pi^2$.  But then according to (ii) in the example $\ccalV_{q_B',q_B''}^{d,1} = \mathcal{AP}_i\setminus\pi^1=\pi^3$. \textcolor{red}{[I revised the definition of this set; see the magenta color earlier in that section. I believe now $\ccalV_{q_B',q_B''}^{d,1}$ is the empty set. ]} So this will prevent us from replacing $\pi^2$ with robot 1.]
%}
% \textcolor{black}{[I agree with these changes. Shall we add another numerical example over here based on Example 3.4? For example $\ccalV_{q_B',q_B''}^{d,1} = \ccalV_{q_B',q_B''}^{d,4} = [\pi_4]$ (according to example 3.5 due to presence of $\neg\pi_4$). ...} \textcolor{red}{[done, I added a similar example]}
%
% \textcolor{olive}{Actually thinking about this we might need to add something more to the definition of $\ccalV_{q_B',q_B''}^{d,4}$ , because according to what we say, since $\pi_4$ is in $\ccalV^{d,4}$, we wont assign robot 4 to task $\pi_4$. But that means we are not restricting robot 4 from being assigned to $\pi_2$ (which is the actual constraint as $\pi_4$ says we cant move in $\ell_2$ and $\pi_2$ demands doing a task in $\ell_2$) ]}
%
% \textcolor{olive}{ohh! wait a second I see it. since we say all the predicates robot can't do that means we are automatically saying  $\ccalV_{q_B',q_B''}^{d,1} = \ccalV_{q_B',q_B''}^{d,4} = [\pi_2, \pi_4]$ ... So the definition still holds.]}
%
%[It should be $\{\pi_2,\pi_3\}$. I believe the definition of AP and $AP_i$ is not clear. By AP i mean all possible predicates of the form \eqref{eq:pip} that we can construct (not all of them will show up in $\phi$) using the set of robots $\ccalR$, the set of skills $\ccalC$, and the locations $\ell_e$. By APi, i mean all possible predicates that we can construct as before but using only robot i. This should be written more clearly. But I am still unsure where the definition of the sets $\ccalV$ is correct or if something is missing]
%\end{ex}

%that takes as input a robot $i$ that belongs to $\ccalR_{q_B',q_B''}^d$ and returns the atomic predicates that are assigned to $i$ in $b_{q_B',q_B''}^d$ (excluding the negated ones \textcolor{red}{and the failed predicate}). We define $g(i)=\varnothing$, for all robots $i\in\ccalR_{q_B',q_B''}^d$ with no assigned predicates; see also Example \ref{ex:Rg}. 



\vspace{-0.2cm}
\subsection{Minimum-Violation Local Task Reallocation}\label{sec:taskRealloc3}
\vspace{-0.1cm}

In this section, we present the proposed minimally-violating, task re-allocation algorithm that fixes failed predicates.
For each $e\in\ccalE$, we express its respective Boolean formula in a DNF form $b_{q_B',q_B''}=\bigvee_{d=1}^Db_{q_B',q_B''}^d$ (lines \ref{rp:collect}-\ref{rp:DNF}, Alg. \ref{alg:RP}).
Then for each sub-formula $b_{q_B',q_B''}^d$ (lines \ref{rp:for3}-\ref{rp:applyBFS}, Alg. \ref{alg:RP}) we search for task re-assignments over a directed graph $\ccalG$ capturing all possible reassignments in $b_{q_B',q_B''}^d$; see Alg. \ref{alg:bfs}.

This graph is defined as $\ccalG=\{\ccalV_{\ccalG},\ccalE_{\ccalG},w_{\ccalG}\}$, where $\ccalV_{\ccalG},\ccalE_{\ccalG}$, and $w_{\ccalG}$ denote the set of nodes, edges, and a cost function, respectively. The set of nodes is defined as $\ccalV_{\ccalG}=\ccalR$ and a directed edge from node $a$ to $a'\neq a$ exists if $a'\in\ccalT_{c}$, where $c$ is the skill required to satisfy the predicate $g_{q_B',q_B''}^d(a)$. The directed edge indicates that robot $a'$ can take over predicate of $a$ in $b_{q_B',q_B''}^d$.
% $w_{\ccalG}:\ccalE_{\ccalG}\rightarrow\mathbb{R}$
The cost function $w_{\ccalG}$ assigns cost of $1$ to each edge. 
% \textcolor{red}{[Is this correct? Shouldnt this cost be associated with the penalty?]}
Note that, our algorithm only needs knowledge of the nodes $a'$ \textcolor{black}{$\in\ccalT_c$} that can be reached in one hop from any node $a$; thus, there is no need to explicitly construct $\ccalG$. %(line \ref{rp:graph}, Alg. \ref{alg:RP}).




% In this section, we present the proposed task re-allocation algorithm. Once the set $\ccalE$ is constructed, we repeat the following steps for each edge $e\in\ccalE$ \textcolor{black}{in parallel (line \ref{rp:for2}, Alg. \ref{alg:RP})}. 
% % 
% Given $e$, we express its corresponding Boolean formula in a DNF form $b_{q_B',q_B''}=\bigvee_{d=1}^Db_{q_B',q_B''}^d$ (whether $q_B'=q_B''$ or not) (line \ref{rp:DNF}, Alg. \ref{alg:RP}). Then we repeat the following steps \textcolor{black}{in parallel} for each sub-formula $b_{q_B',q_B''}^d$ (line \ref{rp:for3}, Alg. \ref{alg:RP}).


% First, we define the following directed graph capturing all possible reassignments \textcolor{black}{in $b_{q_B',q_B''}^d$} \textcolor{black}{(even ones that violate constraints discussed in Section \ref{sec:taskRealloc2})}. Then, we will search over it to find  re-assignments of the sub-tasks/predicates appearing in $b_{q_B',q_B''}^d$ \textcolor{black}{so that there are no unassigned predicates and all assignments respect the constraints captured by $V_{q_B',q_B'}^d$.}
% We denote this graph by $\ccalG=\{\ccalV_{\ccalG},\ccalE_{\ccalG},w_{\ccalG}\}$, where $\ccalV_{\ccalG},\ccalE_{\ccalG},w_{\ccalG}$ denote the set of nodes, edges, and a cost function $w_{\ccalG}:\ccalE_{\ccalG}\rightarrow\mathbb{R}$. \textcolor{black}{The set of nodes is defined as $\ccalV_{\ccalG}=\ccalR$}.
% % 
% \textcolor{black}{An edge from a node $a$ to $a'\neq a$ exists if $a'\in\ccalT_{c}$, where $c$ is the skill required to satisfy the predicate $g_{q_B',q_B''}^d(a)$}. %; notice that this graph does not have self-loops. 
% If $g_{q_B',q_B''}^d(a)=\varnothing$, then there no outgoing edges from $a$. The physical meaning of an edge is that robot $a'$ can take over the predicate (if any) assigned to $a$ in $b_{q_B',q_B''}^d$. %\textcolor{black}{[Since we define $b_{q_B',q_B''}^d$ in the next para, should we move this para to after that?]}. 
% The cost function $w_{\ccalG}$ is defined so that each edge has a cost equal to $1$. %Construction of this graph depends only on the robot skills and it is agnostic to the LTL formula. Also, 
% We emphasize that we do not explicitly construct this graph; instead, the task re-allocation algorithm only requires knowledge of the nodes $a'$ \textcolor{black}{$\in\ccalT_c$} that can be reached in one hop from any node $a$ (line \ref{rp:graph}, Alg. \ref{alg:RP}).



%\textcolor{red}{Then, the goal of running Algorithm \ref{alg:bfs} (in line \ref{rp:applyBFS} of Alg. \ref{alg:RP}), is to find a path in $\ccalG$ from the robot associated with the failed predicate, denoted by $a_{\text{root}}$, to a goal node $a'$, while ensuring $a'$ does not violate any constraints discussed in \ref{sec:taskRealloc2}.  Next, we define the set of goal nodes in $\ccalG$ that we want to reach as follows $\ccalA=\{a\in\ccalR~|~g_{q_B',q_B''}^d(a))=\varnothing\}$.}



We define the set $\ccalA=\{a\in\ccalR~|~g_{q_B',q_B''}^d(a)=\varnothing\}$.
Then, the goal of running Algorithm \ref{alg:bfs} (line \ref{rp:applyBFS} of Alg. \ref{alg:RP}), is to find a path in $\ccalG$ from the robot associated with the failed predicate, denoted by $a_{\text{root}}$, to any node $a'\in\ccalA$, while ensuring $a'$ does not violate any constraints discussed in \ref{sec:taskRealloc2}. In this case, robot $a'$ is not currently assigned to a task in $b_{q_B',q_B''}^d$. %
%
Let $p=p(0),p(1),\dots,p(P)$ denote such a path over $\ccalG$, where $p(0)=a_{\text{root}}$, $p(P)=a'$ and $p(k)\notin\ccalA$, for all $k\in\{2,\dots,P-1\}$. 
Such a path will dictate the re-assignment of tasks required to fix the failed predicate while minimizing the penalty in case of a violating solution. 
% 
Specifically, robot $p(k+1)$ assumes the sub-task currently assigned to robot $p(k)$ in $b_{q_B',q_B''}^d$, represented by the atomic predicate $g_{q_B',q_B''}^d(p(k))$. Note that this means robot $p(k+1)$ relinquishes its current sub-tasks, which will be taken over by robot $p(k+2)$. Additionally, considering the constraints discussed in Section \ref{sec:taskRealloc2}, the path must adhere to the condition that $g_{q_B',q_B''}^d(p(k))\notin V_{q_B',q_B''}^d(p(k+1))$ holds for all $k\in{2,\dots,P-1}$. 

In what follows, we adopt a  Breadth First Search (BFS) inspired approach to find the shortest path $p$ summarized in Alg. \ref{alg:bfs}; see Fig. \ref{fig:bfs}.
%\footnote{\textcolor{blue}{We use BFS instead of Depth First Search because this allows us to generate solutions with minimum number of reassignments without searching the whole graph $\ccalG$.}}
%
If such a path does not exist, then the proposed algorithm can compute the path with the minimum violation penalty cost (to be defined later).
%
We use a queue data structure $\mathcal{Q}$ similar to traditional BFS algorithms. When a node $a$ is removed from $\mathcal{Q}$, then each adjacent node $a'$ is added  to $\mathcal{Q}$ if (1) it has not been explored yet (as in standard BFS) and (2) $g_{q_B',q_B''}^d(a)\notin V^{d}_{q_B',q_B''}(a')$ (line \ref{bfs:conditions}, Alg. \ref{alg:bfs}).
The initial constraint serves to avoid situations where a single robot might have to complete two tasks at the same time, %a single robot is tasked with replacing two robots. This is crucial as it might lead to scenarios where the Boolean formulas $b_{q_B',q_B''}^d$ are satisfied only if a robot can apply multiple skills simultaneously, which is not feasible as outlined in Section \ref{sec:PF}. 
while the second constraint guarantees that the constraints discussed in Section \ref{sec:taskRealloc2} are met.
Also, the root node is not initially marked as `explored'. This deliberate choice permits the robot with the failed skill (the root) to undertake other sub-tasks utilizing its remaining (if any) operational skills. 
% The second difference from the standard BFS is the termination criterion. 
Simultaneously, every time we add a node to the queue, we update $a^*$ to point to the node with the \textit{lowest penalty} defined as $F(g_{q_B',q_B''}^d(a^*))$ (line \ref{bfs:penaltyConditions}-\ref{bfs:reassign2ndBest}, Alg. \ref{alg:bfs}). 
%The assignment cost incurred by the path connecting the root to $a^*$ is defined to be $F(g_{q_B',q_B''}^d(a^*))$ as $g_{q_B',q_B''}^d(a^*)$ will not be completed. %\textcolor{cyan}{I couldn't think of any appropriate variable name in place of $2ndBest$.}\textcolor{red}{ why is it the `2nd' best if it has the lowest penalty? Maybe call it $a^*$? }
%then we evaluate the nodes we did explore during the search. Among these nodes, we identify the node $a'$ \textcolor{blue}{[$a'$ or $a^*$ since we use $a^*$ in the algorithm to refer to the node with the lowest penalty?]}whose predicate has the least penalty. In other words, within all the explored nodes, we choose the node $a'$ where $\ccalF(g_{q_B',q_B''}^d(a'))$ has the smallest value. \textcolor{blue}{We define this as the penalty associated with finding a reassignment for a failed predicate.} %\textcolor{cyan}{[this will be referred to in prop 3.3]}


%If, even after an exhaustive search of the graph, we cannot find such a node $a'\in\ccalA$, then 



% \textcolor{cyan}{[Conflict: $\ccalF$ is now $P$, but $P$ is already used. fix it]}    
% 

% Specifically, the robot $p(k+1)$ takes over the sub-task of robot $p(k)$ in $b_{q_B',q_B''}^d$ (i.e., the atomic predicate $g_{q_B',q_B''}^d(p(k))$). Note that this means that the robot $p(k+1)$ gives up on its current sub-tasks (which will be taken over by the robot $p(k+2)$). Also, since this path should respect the constraints discussed in Section \ref{sec:taskRealloc2}, it must also hold that $g_{q_B',q_B''}^d(p(k))\notin V_{q_B',q_B''}^d(p(k+1))$ for all $k\in\{2,\dots,P-1\}$.

% If we do not find any node $a'$ satisfying $g_{q_B',q_B''}^d(a')=\varnothing$, i.e., if $\ccalA$ is an empty set, then our goal is to find the node $a'$ such that the predicate $a'$ is assigned to in $b_{q_B',q_B''}^d$ has the lowest penalty among all nodes. In this case, we set $p(P)=a'$ and we complete the re-assignment as described above. Note that after the reassignment the predicate $a'$ is assigned to will not have any robot assigned to it and thus will not be satisfied. However, as mentioned previously we say that this predicate is satisfied with a penalty.



% Then, we apply a constrained Breadth First Search (BFS) algorithm over $\ccalG$ to re-assign sub-tasks (i.e., predicates appearing in $b_{q_B',q_B''}^d$) to robots (line \ref{rp:applyBFS}, Alg. \ref{alg:RP}). 
% Our goal is to find a path in $\ccalG$ from the robot associated with failed predicate, denoted by $a_{\text{root}}$, to any node $a'$ satisfying $g_{q_B',q_B''}^d(a')=\varnothing$ (i.e., $a'$ is not assigned any task in $b_{q_B',q_B''}^d$) while respecting the constraints discussed in Section \ref{sec:taskRealloc2}. \textcolor{black}{We define the set $\ccalA=\{a\in\ccalR~|~g_{q_B',q_B''}^d(a)=\varnothing\}$.} %\cup\{a_{\text{root}}\}
% %
% %
% \textcolor{black}{Let $p=p(0),p(1),\dots,p(P)$ denote such path over $\ccalG$, where $p(0)=a_{\text{root}}$, $p(P)\in\ccalA$ and $p(k)\notin\ccalA$, for all $k\in\{2,\dots,P-1\}$. %Also, the path $p$ should respect the constraints discussed in Section \ref{sec:taskRealloc2}, In other words, since the robot $p(k+1)$ takes over the task of $p(k)$
% %
% Such a path will dictate the re-assignment of tasks required to fix the failed predicate. %For instance, let $p=p(0),p(1),\dots,p(K)$ denote such a path where $p(k)\in\ccalV$, $p(0)=a_{\text{root}}$, and $p(K)\in\ccalB$. 
% %Given such path, a sequence of task re-assignments arise. 
% Specifically, the robot $p(k+1)$ takes over the sub-task of robot $p(k)$ in $b_{q_B',q_B''}^d$ (i.e., the atomic predicate $g_{q_B',q_B''}^d(p(k))$). Note that this means that the robot $p(k+1)$ gives up on its current sub-tasks (which will be taken over by the robot $p(k+2)$).} \textcolor{black}{Also, since this path should respect the constraints discussed in Section \ref{sec:taskRealloc2}, it must also hold that $g_{q_B',q_B''}^d(p(k))\notin V_{q_B',q_B''}^d(p(k+1))$ for all $k\in\{2,\dots,P-1\}$.}

% If we do not find any node $a'$ satisfying $g_{q_B',q_B''}^d(a')=\varnothing$, i.e., if $\ccalA$ is an empty set, then our goal is to find the node $a'$ such that the predicate $a'$ is assigned to in $b_{q_B',q_B''}^d$ has the lowest penalty among all nodes. In this case, we set $p(P)=a'$ and we complete the re-assignment as described above. Note that after the reassignment the predicate $a'$ is assigned to will not have any robot assigned to it and thus will not be satisfied. However, as mentioned previously we say that this predicate is satisfied with a penalty.  

\begin{algorithm}[t]
\footnotesize
\caption{Breadth First Search}
\LinesNumbered
\label{alg:bfs}
\KwIn{ (i) Failed predicate $\pi_{\ccalT_c}(j, c,\ell_e$), 
% (ii)\textcolor{black}{$\ccalG$,}\textcolor{red}{[remove it?]} %$b_{q_B',q_B''}^d$, 
% (iii)\textcolor{black}{$\ccalR_{q_B',q_B''}^d$,} 
(ii) $V^{d}_{q_B',q_B''}$, (iii) $g^{d}_{q_B',q_B''}$, (iv) \textcolor{black}{Teams $\ccalT_c(t), ~\forall c\in\ccalC$}}
\KwOut{Path $p$}
$a_{\text{root}}$ = $j$\;\label{bfs:root}
% label $a_{\text{root}}$ as explored\;
$\mathcal{Q}$ = [$a_{\text{root}}$]\;\label{bfs:queue}
$\texttt{Flag}_{\text{root}}$ = True\;\label{bfs:falgSetTrue}
$a^*$ = $a_{\text{root}}$\;\label{bfs:assign2ndBest}
\While{$\sim$empty($\mathcal{Q}$)}{
    $a\leftarrow$ POP($\mathcal{Q}$)\;\label{bfs:pop}
    \If{$a\in\ccalA$ \& $\sim \texttt{Flag}_{\text{root}}$}{\label{bfs:terminate}
        Using $\texttt{Parent}$ function return path $p$ from $a$\;\label{bfs:return}
    }
    $\texttt{Flag}_{\text{root}}$=False\;\label{bfs:falgSetFalse}
    \For{$a'$ adjacent to $a$ in $\ccalG$}{
    % \For{$a'\in\ccalT_c\setminus {a}$}{
        \If{$g_{q_B',q_B''}^d(a)\notin V^{d}_{q_B',q_B''}(a')$ \& $a'$ not explored}
        % \& $a'\neq a$ $a'\notin \textcolor{black}{\texttt{Parents}(a')\setminus{a^{root}}}$ \& \textcolor{black}{$g_{q_B',q_B''}^d(a')<=1$}}
        {\label{bfs:conditions}
            % $new\_path$ = $path$\;\label{bfs:newpath}
            Label $a'$ as explored\;
            $\texttt{Parent}(a') = a$\;\label{bfs:addparent}
            Append $a'$ to $\mathcal{Q}$;\label{bfs:appendToQ}
            
            \If{$F(g_{q_B',q_B''}^d(a'))<F(g_{q_B',q_B''}^d(a^*))$}
            {\label{bfs:penaltyConditions}
                $a^*$ = $a'$ ;\label{bfs:reassign2ndBest}
            }
        }
        
    }
    \If{empty(Q)}{
        Using $\texttt{Parent}$ function return path $p$ from $a^*$\;\label{bfs:penalty_return}
    }
}
% return ($\emptyset$) \label{bfs:failreturn}
\vspace{-0.1cm}
\end{algorithm}
% \vspace{-0.1cm}



Finally, we note that the graph-search process is terminated in two ways. The first way is when the first feasible path from $a_{\text{root}}$ to any node in $\ccalA$ is found (line \ref{bfs:terminate}-\ref{bfs:return}, Alg. \ref{alg:bfs}). In this case, the assignment cost is $0$. If such paths cannot be computed (i.e., there is no available robot), \textcolor{blue}{then  Alg. \ref{alg:bfs} terminates when it has emptied the $\mathcal{Q}$, meaning it has searched all possible reassignments in $\ccalG$.} 
Then Alg. \ref{alg:bfs} returns as a solution the path with the smallest assignment cost, i.e., the path to the node $a^*$ with the smallest penalty $F(g_{q_B',q_B''}^d(a^*))$ where the penalty function $F$ is defined in Definition \ref{def:penalty} (line \ref{bfs:penalty_return}, Alg. \ref{alg:bfs}). The assignment cost incurred by the path connecting the root to $a^*$ is defined to be $F(g_{q_B',q_B''}^d(a^*))$, as task $g_{q_B',q_B''}^d(a^*)$ will not be completed.\footnote{\textcolor{black}{While fixing the predicate in $a_{\text{root}}$, we may sacrifice at most one predicate, by construction of the BFS algorithm.
%. Because of how we have defined the reassignment process, if we have to sacrifice, it would be the predicate corresponding to $p(P)$.
}}
%
%This path corresponds to the minimum possible re-assignments that can occur to fix the failed predicate in $b_{q_B',q_B''}^d$. The second way is when we have searched the entire graph and could not find a feasible solution. In this case, we return the path to the node with the lowest penalty (line \ref{bfs:penalty_return}, Alg. \ref{alg:bfs}).
%
Once all failed predicates are fixed with the least amount of violation, the associated formulas $b_{q_B',q_B''}$ are accordingly revised, yielding a new NBA (line \ref{rp:reassign}, Alg. \ref{alg:RP}). 
This revised NBA is an input to an online planner that designs new paths.


%\textcolor{red}{[We need a short proposition for this.]} \textcolor{red}{[I believe we need a toy example/figure to describe the BFS algorithm; similar to the graph you have in the simulations. also if we agree on this description, we should update the notations in algorithm 2. I suggest we make it more concise by more or less copying and pasting the standard BFS algorithm (with minor modification if needed); see e.g., https://www.cs.umd.edu/class/spring2021/cmsc351-0201/files/bfs.pdf]} 
% \textcolor{black}{[I think we will need to mention that the set $\ccalB$ is updated everytime we reassign tasks. i.e., when we reassign robots that were free are now assigned something, and the failed robot could have become free. And mostly since $g(i)$ is a function, we will not need to update the reassignment for it.]}.\textcolor{red}{[Hmm I think the set of free robots remains always the same. Or I am wrong?]}\textcolor{black}{[The way I see it is that if there are two or more robot failures, then after fixing the first failure, one robot that was initially free is now assigned to a task, and the failed robot is now free. So when we start to fix the next failure, we will need to refer to the new $\ccalB$. But if we are initialize $\ccalB$ every time we start our BFS algorithm, then you are right,the set of free robots is constant]}
%\textcolor{red}{Agreed. $\ccalB$ is initialized for each new assignment. This needs to be clear in the algorthm}


%(b) is allowed to take over the task modeled by $a$, i.e., (b.1) $a\notin\ccalV^{d,a_{\text{rbt}}'}$; and (b.2) $a_{\text{rbt}}'\neq a_{\text{rbt}}$.
%
%Constraint (b.1) applies only in case $q_B'\neq q_B''$ as these constraints do not apply to self-loops.\textcolor{black}{[Will we need to mention that when adding $a'$ into the graph, $a'_{\text{rbt}}$ should not already exist in the graph. i.e., each robot can only be added once. The only exception is the root robot which can be added one more time as it belongs to $\ccalB$ once it is removed from its current failed task.]}.





%\textcolor{red}{[to be updated--$>$]}
%\begin{ex}[NBA transition]\label{ex:LTL_trans}
%We build the NBA for the mission given in Example \ref{ex:LTL}.
%A particular transition in the NBA $q_B^{\prime}\rightarrow q_{B}^{\prime\prime}$ %(Fig. \ref{fig:LTL}) 
%is governed by the Boolean $b_{q_B^{\prime},q_{B}^{\prime\prime}}$ = $(\pi_1\land\pi_2\land\neg\pi_4)\lor(\pi_1\land\pi_3\land\neg\pi_4)$. There are self loops at both ends, $b_{q_B^{\prime},q_B^{\prime}}$ = $b_{q_{B}^{\prime\prime},q_{B}^{\prime\prime}}$ = $\neg\pi_4$. 
%For this example if any of $\sigma_1$ = $(\pi_1,\pi_2)$, $\sigma_2$ = $(\pi_1,\pi_3)$, or $\sigma_3$ = $(\pi_1,\pi_2,\pi_3)$ are true, and $(\pi_4)$ is not true, then the transition $q_B^{\prime}\rightarrow q_{B}^{\prime\prime}$ is satisfied.
%Therefore, $\Sigma_{q_B^{\prime},q_{B}^{\prime\prime}}=[\sigma_1,\sigma_2,\sigma_3]$. 
% Consider a mission involving 5 robots, $rob_1,\dots,rob_5$. Assume $rob_1,rob_2,rob_4,rob_5$ have the same single ability $\zeta_1$ and $rob_3$ has a different ability $\zeta_3$. Consider the following atomic predicates in the mission:   $\pi_{\ccalT_1}^1(rob_1, \zeta_1, \ell_1)$, $\pi_{\ccalT_1}^2(rob_2, \zeta_1, \ell_2)$, $\pi_{\ccalT_3}^3(rob_3, \zeta_3, \ell_3)$, $\pi_{\ccalT_1}^4(rob_4, \zeta_1, \ell_2)$,
%Consider a mission involving five robots, robot $1$ to robot $5$. Assume robots $1,2,4,5$ have the same single ability $\zeta_1$ and robot $3$ has a different ability $\zeta_3$. Consider the following atomic predicates in the mission:   $\pi_1=\pi_{\ccalT_1}(1, 1, \ell_1)$, $\pi_2=\pi_{\ccalT_1}(2, 1, \ell_2)$, $\pi_3=\pi_{\ccalT_3}(3, 3, \ell_3)$, $\pi_4=\pi_{\ccalT_1}(4, 1, \ell_2)$,
%
% \begin{align}\label{eq:taskEx2}
%     \phi = &\Diamond[\pi_{\ccalT_2}(rob_1, \zeta_2, l_1)\wedge\Diamond[\pi_{\ccalT_3}(rob_2, \zeta_3, l_1)]]\nonumber\\&\wedge\Diamond[\pi_{\ccalT_2}(rob_3, \zeta_2, l_2)]\nonumber
% \end{align}
%A particular transition in the NBA $q_B\rightarrow q_{B}^{\prime}$ (Fig. \ref{fig:LTL}) is governed by the boolean $b_{q_B,q_{B}^{\prime}}$ = $(\pi_1\land\pi_2)\lor\pi_3$. There are self loops at both ends, $b_{q_B,q_B}$ = $b_{q_{B}^{\prime},q_{B}^{\prime}}$ = $\neg\pi_4$. 
%For this example if any of $\sigma_1$ = $(\pi_1,\pi_2)$, $\sigma_2$ = $(\pi_3)$, $\sigma_3$ = $(\pi_3,\pi_2)$, $\sigma_4$ = $(\pi_3,\pi_2)$, or $\sigma_5$ = $(\pi_3,\pi_1,\pi_2)$ are true, and $(\pi_4)$ is not true, then the transition $q_B\rightarrow q_{B}^{\prime}$ is satisfied. Therefore, $\Sigma_{q_B,q_{B}^{\prime}}=[\sigma_1,\dots,\sigma_5]$.
%\end{ex}



%\textcolor{black}{[shall we add this here (but modified according to current notation]: Thus if we consider the transition enabled by $\sigma_1$, then for predicate $\pi_2=\pi_{\ccalT_3}(2, c_3, \ell_2)$, $\ccalT_3=[1,2,4,5]$, and $\mathcal{A}[\pi_2] = [1,2]$ as robot $1$ and robot $2$ are assigned to do predicates $\pi_1$ and $\pi_2$ respectively in $\sigma_1$. 
%Next, due to the presence of $\neg\pi^4$ in $b_{q_B,q_B^{\prime}}$, robots belonging to $\ccalT_2$ (robots $1$ and $4$) are restricted from approaching at $\ell_2$ and thus they cannot be assigned to do $\pi_2$ as it involves approaching $\ell_2$. Therefore $\mathbb{C}[\pi_2] = [1,4]$.
%Thus, $\mathcal{U} = \ccalT_c - \mathcal{A}[\pi_p] - \mathbb{C}[\pi_p] = [5]$ which means robot $5$ is the free robot that can replace robot $2$ at its task in $\pi_2$ if needed. }


%\textcolor{red}{END}



\vspace{-0.1cm}
\subsection{Minimum Violation Online Re-planning}\label{sec:onlineReplan}
\vspace{-0.1cm}

Assume that the multi-robot system is at state $\tau_H(t)=[\bbp(t), \bbs(t), q_B(t)]$ when capability failures occurred and that Alg. \ref{alg:RP} has re-assigned tasks to robots. A possible approach to revise the plan $\tau_H$ and, consequently, $\tau$ is to re-plan globally. Specifically, given the revised NBA, we can use any existing  temporal logic planner to compute the  paths satisfying the LTL task starting from the state $\tau_H(t)$ that minimize the cost function \eqref{eq:violation} \cite{luo2021abstraction,gujarathi2022mt}. 
%We then use a sampling-based planner \cite{luo2021abstraction} to generate new plans $\tau$, \textcolor{black}{that minimize the cost function \eqref{eq:violation}}. %We then pick the plan $\tau$ with the lowest violation score as described in Section \ref{sec:Vscore}. 
If the total cost is zero, it means we have found the path that completely satisfies the mission.\footnote{\textcolor{black}{Note that 
it is possible that the violation cost of the revised plan is $0$ even though Alg. \ref{alg:bfs} fails to fix all predicates.
%not being able to fix all predicates with zero penalty does not imply that we cannot find a plan with zero violation score.
}} %finding a plan with zero violation score does not imply that we fixed all failed predicates. }
%
% \textcolor{red}{[Is this possible even if you werent able to fix all predicates? If so, I think this is important to mention i.e., that not being able to fix all predicates does not imply that we cannot find a plan with zero cost. ]}
%
If the score is non-zero, it means we have found the least violating path such that the tasks which will not be completed, have cumulatively the smallest penalty. Nevertheless, global re-planning can be impractical especially for large robot teams or complex missions. 


In what follows, we present a more efficient re-planning approach that locally revises the paths of those robots affected by failures. Our approach, essentially, determines the local parts of the global plan $\tau_H$ that need to revised. %, thus avoiding the need for global re-planning.% as in our previous work \cite{kalluraya2023resilient_arxiv}. 
% \textcolor{cyan}{I don't discuss local revised plans here.}\textcolor{red}{[That's fine but I think a reference to the arxiv paper is needed here; otherwise reviewers may think that local revision is not possible. ]}
%
First, we define the path $\hat{\tau}_H=\tau_H^{\text{pre}}\tau_H^{\text{suf}}=[\bbq(1),\dots,\bbq(T)],[\bbq(T+1),\dots, \bbq(T+K)]$ that concatenates the prefix and the suffix part of the current plan $\tau_H$ (without repeating  $\tau_H^{\text{suf}}$); see also Section \ref{sec:Vscore}.
%
Second, we compute the state $\hat{\tau}_H(k)$ for which it holds $\hat{\tau}_H(k)=\tau_H(t)$.\footnote{It is possible that $t>T+K$ since the state $\tau_H(t)$ may belong to the suffix part and $\tau_H$ contains an infinite repetition of the suffix part. In $\hat{\tau}_H(k)$, $k$ points to the $k$-th entry in $\hat{\tau}_H$ where   $\hat{\tau}_H(k)=\tau_H(t)$.} 
Third, we define the ordered set $\Upsilon_{\text{pre}}$ collecting all states $\hat{\tau}_H(k')=[\bbp(k'), \bbs(k'), q_B(k')]$ in $\hat{\tau}_H$ that satisfy the following requirements: i) $k' \geq k$; ii) ($q_B(k')\neq q_B(k'-1)$; and iii) $k'\leq T$.
The states in $\Upsilon_{\text{pre}}$ are projected onto the NBA to get $\ccalP_{\text{pre}}^{\tau}$ which is of the form $\ccalP_{\text{pre}}^{\tau}=\{q_B^0,q_B^1,\dots\}$, where $q_B^0=q_B(t)$.
We denote by $\Upsilon_{\text{pre}}(e)$ and $\ccalP_{\text{pre}}^{\tau}(e)$ the $e$-th entry in $\Upsilon_{\text{pre}}$ and $\ccalP_{\text{pre}}^{\tau}$, respectively. %We also include the current state $\hat{\tau}_H(k)$. 
We similarly define $\Upsilon_{\text{suf}}$ and $\ccalP_{\text{suf}}^{\tau}$ where the third requirement is replaced by $T+1\leq k'\leq T+K$. 
Together $\ccalP^{\tau}=\ccalP_{\text{pre}}^{\tau}\ccalP_{\text{suf}}^{\tau}$.


% \textcolor{pink}{lets do it the other way around. define hypothetical paths corrsponding to runs in the nba. and find violation cost for each path. and pick path with lowest violation cost}




Next, we will try to determine the sequence of states in the NBA that would correspond to the new optimal plan.  
Any hypothetical plan that satisfies the mission can be projected onto the NBA, as done above, to get a sequence of states $\ccalP=\ccalP_{\text{pre}}\ccalP_{\text{suf}}$. Thus, if we implement a simple graph search on the NBA from the current state  $q_B(t)$ to obtain an accepting run $\ccalP=\ccalP_{\text{pre}}\ccalP_{\text{suf}}$, there will exist at least one plan (assuming it is feasible in the environment), that if projected on the NBA will generate the same sequence of NBA states. 

Given the revised NBA with the new robot-task assignments, there could be some transitions $q_B'$ to $q_B''$ where a task was sacrificed (predicate corresponding to the $a^*$ node) to fix a failure in a minimally violating way. Thus the predicate associated with such a sacrificed task will not have a robot assigned to it and thus won't be completed. Now for the hypothetical plan to transition from $q_B'$ to $q_B''$ it will need to generate a hypothetical symbol $\sigma(t')=L([\bbp(t'),\bbs(t')])$, at some arbitrary time $t'$, such that $\sigma(t')\models b_{q_B',q_B''}$. However, after the reassignment, some of the predicates may not be satisfied due to a robot not being assigned to it, $\sigma(t')\not\models b_{q_B',q_B''}$. There exists at least one $\sigma^* \in \Sigma$, such that the concatenation of the symbols $\sigma(t')$ and $\sigma^*$ satisfies $b_{q_B',q_B''}$, i.e., $\sigma(t')\sigma^*\models b_{q_B',q_B''}$. Thus the predicates in $\sigma^*$, if assumed true at time $t'$, allow the transition from $q_B'$ to $q_B''$. Intuitively, $\sigma^*$ will include the unassigned predicates. Therefore, the predicted cost of violation in this transition can be calculated using \ref{eq:edgeviolation}.  
Recollect here that, reassignment done by Alg. \ref{alg:bfs} ensures that this violation cost will be the lowest possible for this transition.

With slight abuse of terminology, the total violation score, $\mathbb{C}_\ccalP$, along the projection $\ccalP$ of a hypothetical plan can be calculated using \ref{eq:violation}, where instead of summing over each time step, we sum over each subsequent transition $q_B', q_B''$ in $\ccalP$. 
Thus, 
\begin{equation}\label{eq:NBAviolation}
\mathbb{C}_\ccalP =  \sum_{q_B', q_B'' \in \ccalP} \min_{\forall \sigma^* \in \Sigma^*} (\sum_{\pi\in\sigma^*} F(\pi))
\end{equation}

We first search in the NBA to find an accepting run $\ccalP^{\text{min}}=\ccalP_{\text{pre}}^{\text{min}}\ccalP_{\text{suf}}^{\text{min}}$ from the current state $q_B(t)$ such that $\mathbb{C}_\ccalP$ is the lowest.\footnote{For sake of brevity we assume that the boolean cannot be split into DNF form. In case the boolean can be represented in it's DNF form, a unique path $\ccalP$ must be considered for each boolean in the DNF form} If there exists more than one such path $\ccalP^{\text{min}}$ in the NBA that has the same minimum cost, we choose $\ccalP^{\text{min}}$ as the path which has the most ``true" overlap (defined in next para) with $\ccalP^{\tau}$. 
Intuitively, an overlap is the set of edges that both paths $\ccalP^{\text{min}}$ and $\ccalP^{\tau}$ share in the NBA. We collect all such overlap edges in the ordered set $\ccalO = \{ (q_B^i,q_B^{i+1}) \mid \forall q_B^i,q_B^{i+1} \in \ccalP^{\text{min}}, \exists q_B^j,q_B^{j+1}\in\ccalP^{\tau} : (q_B^i,q_B^{i+1})=(q_B^j,q_B^{j+1}) \}$. 
% Furthermore, we call a state $q_B^i$ as the start of an overlap if $(q_B^{i-1},q_B^i)\notin\ccalO\text{ and }(q_B^i,q_B^{i+1}) \in \ccalO$. Similarly a state $q_B^i$ is the end of an overlap if $(q_B^{i-1},q_B^i)\in\ccalO\text{ and }(q_B^i,q_B^{i+1}) \notin \ccalO$.


\begin{figure}[t]
  \centering
      \subfigure[Current NBA state sequence $\ccalP_{\text{pre}}^{\tau}$]{
    \label{fig:curNBA}
  \includegraphics[width=1\linewidth]{figures/orp1.png}}
  \subfigure[Minimum violating NBA state sequence $\ccalP_{\text{pre}}^{\text{min}}$]{
    \label{fig:revNBA}
  \includegraphics[width=1\linewidth]{figures/orp2.png}}
  \subfigure[Current Path]{
    \label{fig:curPath}
  \includegraphics[width=1\linewidth]{figures/orp3.png}}
  \subfigure[Revised Path]{
    \label{fig:revPath}
  \includegraphics[width=1\linewidth]{figures/orp4.png}}
  \caption{Hypothetical example of online revision of a part of the prefix path. NBA states $\text{A,B,\dots,J}\in\ccalQ_{B}$, where $q_B(t)=q_B(k)=\text{A}$. Fig. \ref{fig:curNBA} shows the states in $\ccalP_{\text{pre}}^{\text{min}}$, along with the predicate-robot assignment that enables the transition to each state (the predicates and robot numbers are for illustrative purposes only). Assume some robot failures have occurred rendering some of the transitions in the NBA infeasible (red cross). Fig. \ref{fig:revNBA} shows the path in the NBA that generates the lowest violation cost after fixing the failures. Here the overlap exists from C to F. However, only transition from D to E will be considered a true overlap as the predicates and the robots assigned to them to reach D and E are the same in both $\ccalP_{\text{pre}}^{\text{min}}$ ND $\ccalP_{\text{pre}}^{\tau}$.
  The disks in Figs. \ref{fig:curPath} and \ref{fig:revPath} capture states in $\hat{\tau}_H$.
  Yellow states $\hat{\tau}_H(k')$ model states for which it holds $q_B(k')\neq q_B(k'-1)$. The part of $\hat{\tau}_H$ connecting  NBA states $q_B$ and $q_B'$, where $e=(q_B,q_B')\in\ccalE$ (see Alg. \ref{alg:RP}) is marked with a red color and a red `X' denoting that it requires revision. In this example, the planner re-plans a path from current state $\hat{\tau}_H(k)$ to  $\Upsilon_{\text{pre}}(3)$ which is the start of a true overlap, and re-plans another path from the end of the overlap $\Upsilon_{\text{pre}}(3)$ to the final accepting state. The planner does not plan for the true overlap section (D-E) and instead uses the original plan.
  }
%\vspace{0.2cm}
  \label{fig:revise}
\end{figure}


Note that an overlap does not necessarily mean the path is reusable because an overlapped edge could have different robot-task reassignments after running Alg. \ref{alg:RP}. We classify a ``true" overlap of an edge $q_B^i,q_B^{i+1}\in \ccalP^{\text{min}}$, if the starting conditions of the edge and ending conditions of the edge are the same in the original path. 
If $(q_B^i,q_B^{i+1})\in\ccalO$, then without loss of generality let $\ccalP_{\text{pre}}^{\tau}(j)=q_B^j$ and $\ccalP_{\text{pre}}^{\tau}(j+1)=q_B^{j+1}$, such that $(q_B^j,q_B^{j+1})=(q_B^i,q_B^{i+1})$, and let the corresponding states be $\Upsilon_{\text{pre}}(j)=[\bbp(k'), \bbs(k'), q_B(k')]$ and $\Upsilon_{\text{pre}}(j+1)=[\bbp(k''), \bbs(k''), q_B(k'')]$. If $L([\bbp(k'-1),\bbs(k'-1)])=b_{q_B^{i-1},q_B^i}$ and $L([\bbp(k''-1),\bbs(k''-1)])=b_{q_B^i,q_B^{i+1}}$, or in words, if the same set of robots are assigned to the predicates that satisfy the transition to $q_B^i$ and $q_B^{i+1}$ in $\ccalP^{\text{min}}$ and $\ccalP^{\tau}$, then $q_B^i,q_B^{i+1}\in \ccalP^{\text{min}}$ is considered a ``true" overlap. We collect all such edges in the ordered set $\ccalO^*$.


% Thus only if the starting conditions of the edge and ending conditions of the edge are the same in the original path, only then can we say that there is a ``true" overlap in the edge.
Furthermore, we call a state $q_B^i$ as the start of a true overlap if $(q_B^{i-1},q_B^i)\notin\ccalO^*\text{ and }(q_B^i,q_B^{i+1}) \in \ccalO^*$. Similarly a state $q_B^i$ is the end of a true overlap if $(q_B^{i-1},q_B^i)\in\ccalO^*\text{ and }(q_B^i,q_B^{i+1}) \notin \ccalO^*$. 
If $|\ccalO^*|=0$, it means that there is no overlap with the original plan and to minimally violate the mission, we need to globally re-plan. If $|\ccalO^*|> 0$, we plan locally from the current state $\hat{\tau}_H(k)$ to the state $\hat{\tau}_H(k')$ in the original plan corresponding to the start of the first overlap in $\ccalO^*$.\footnote{\textcolor{blue}{Here we make an assumption that the path from  $\hat{\tau}_H(k)$ to  $\hat{\tau}_H(k')$ is feasible in the environment. If the planner cannot find a feasible path, then it must switch to global replanning. }\textcolor{red}{[What happens if a path connecting $\hat{\tau}_H(k)$ to  $\hat{\tau}_H(k')$ does not exist?]}} Similarly, we re-plan only from the end of each overlap, to either the beginning of the next overlap or until our planner reaches an accepting state in the automaton. See Fig. \ref{fig:revise}.   
$q_B''$. 
.\\
.\\
.\\.\\.\\

% Next, we define the idea of a violation cost in the revised automaton. Given the revised NBA with the new robot-task assignments, there could be some transitions $q_B'$ to $q_B''$ where a task was sacrificed (predicate corresponding to the $a^*$ node) to fix a failure in a minimally violating way. Thus the predicate associated with such a sacrificed task will not have a robot assigned to it. \textcolor{blue}{We can then split $b_{q_B',q_B''}^d$ into two sets of predicates where one set consists of predicates that have a robot assigned to them and the other consists of predicates without a robot assigned.
% Let $\sigma_d\in\Sigma$ and $\sigma_d^*\in\Sigma$, be such that,
% % \footnote{\textcolor{red}{This notation is not correct. A symbol $\sigma$ satisfies ($\models$) a boolean formula. Are you splitting the Boolean formula into two subformulas or the symbol into two symbols? If the latter, the notations needs to change.}}
% $\sigma_d$ satisfies the predicates that have a robot assigned to them and $\sigma_d^*$ satisfies the predicates that do not have a robot assigned to them.}
% We can then calculate the violation cost of a transition $q_B'$ to $q_B''$ in the NBA as  $\mathbb{C}_{q_B',q_B''} =  \underset{1 \leq d \leq D}{\text{min}} (\sum_{\pi\in\sigma_d^*} F(\pi))$. Given a run in the NBA $\ccalP=\ccalP_{\text{pre}}\ccalP_{\text{suf}}$, we can calculate the total violation cost $\mathbb{C}_\ccalP$ as the sum of the violation cost between each consecutive states $q_B',q_B''$ in $\ccalP$.
% \textcolor{blue}{Note that the violation score $\mathbb{C}_\tau(t)$ is the violation of the plan, calculated based on the actual plan executed after time $t$. It depends on the booleans the plan satisfies to complete the mission. On the other hand, if $\ccalP$ is the projection of the plan in the NBA, then $\mathbb{C}_\ccalP$ is the lowest possible violation score achievable by a plan, by satisfying the booleans that result in the smallest penalties. }
% \textcolor{red}{[You need somehow to draw a connection to original cost function we defined in (1). If this is not possible to do here, you should do it in the proof. Currently we introduce several cost functions with no clear connections between them.]}


% \textcolor{red}{[Here you need 1-2 sentences describing your goal is in the following text. If I understand correctly, your goal is to identify, which parts of the plan $\tau_H$ need to be revised. ]}

% \textcolor{blue}{The goal is now to determine the sequence of states in the NBA from our current state that would allow the planner to generate the lowest violation score, while simultaneously trying to reuse parts of the original plan $\hat{\tau}_H$ in the revised plan.}  
% We first search in the NBA to find an accepting run $\ccalP^{\text{min}}=\ccalP_{\text{pre}}^{\text{min}}\ccalP_{\text{suf}}^{\text{min}}$ from the current state $q_B(t)$ such that $\mathbb{C}_\ccalP$ is the lowest. If there exists more than one such path $\ccalP^{\text{min}}$ in the NBA that has the same minimum cost, we choose $\ccalP^{\text{min}}$ as the path which has the most ``true" overlap (defined in next para) with $\ccalP^{\tau}$. 
% Intuitively, an overlap is the set of edges that both paths $\ccalP^{\text{min}}$ and $\ccalP^{\tau}$ share in the NBA. We collect all such overlap edges in the ordered set $\ccalO = \{ (q_B^i,q_B^{i+1}) \mid \forall q_B^i,q_B^{i+1} \in \ccalP^{\text{min}}, \exists q_B^j,q_B^{j+1}\in\ccalP^{\tau} : (q_B^i,q_B^{i+1})=(q_B^j,q_B^{j+1}) \}$. 
% % Furthermore, we call a state $q_B^i$ as the start of an overlap if $(q_B^{i-1},q_B^i)\notin\ccalO\text{ and }(q_B^i,q_B^{i+1}) \in \ccalO$. Similarly a state $q_B^i$ is the end of an overlap if $(q_B^{i-1},q_B^i)\in\ccalO\text{ and }(q_B^i,q_B^{i+1}) \notin \ccalO$.


% \begin{figure}[t]
%   \centering
%       \subfigure[Current NBA state sequence $\ccalP_{\text{pre}}^{\tau}$]{
%     \label{fig:curNBA}
%   \includegraphics[width=1\linewidth]{figures/orp1.png}}
%   \subfigure[Minimum violating NBA state sequence $\ccalP_{\text{pre}}^{\text{min}}$]{
%     \label{fig:revNBA}
%   \includegraphics[width=1\linewidth]{figures/orp2.png}}
%   \subfigure[Current Path]{
%     \label{fig:curPath}
%   \includegraphics[width=1\linewidth]{figures/orp3.png}}
%   \subfigure[Revised Path]{
%     \label{fig:revPath}
%   \includegraphics[width=1\linewidth]{figures/orp4.png}}
%   \caption{Hypothetical example of online revision of a part of the prefix path. NBA states $\text{A,B,\dots,J}\in\ccalQ_{B}$, where $q_B(t)=q_B(k)=\text{A}$. Fig. \ref{fig:curNBA} shows the states in $\ccalP_{\text{pre}}^{\text{min}}$, along with the predicate-robot assignment that enables the transition to each state (the predicates and robot numbers are for illustrative purposes only). Assume some robot failures have occurred rendering some of the transitions in the NBA infeasible (red cross). Fig. \ref{fig:revNBA} shows the path in the NBA that generates the lowest violation cost after fixing the failures. Here the overlap exists from C to F. However, only transition from D to E will be considered a true overlap as the predicates and the robots assigned to them to reach D and E are the same in both $\ccalP_{\text{pre}}^{\text{min}}$ ND $\ccalP_{\text{pre}}^{\tau}$.
%   The disks in Figs. \ref{fig:curPath} and \ref{fig:revPath} capture states in $\hat{\tau}_H$.
%   Yellow states $\hat{\tau}_H(k')$ model states for which it holds $q_B(k')\neq q_B(k'-1)$. The part of $\hat{\tau}_H$ connecting  NBA states $q_B$ and $q_B'$, where $e=(q_B,q_B')\in\ccalE$ (see Alg. \ref{alg:RP}) is marked with a red color and a red `X' denoting that it requires revision. In this example, the planner re-plans a path from current state $\hat{\tau}_H(k)$ to  $\Upsilon_{\text{pre}}(3)$ which is the start of a true overlap, and re-plans another path from the end of the overlap $\Upsilon_{\text{pre}}(3)$ to the final accepting state. The planner does not plan for the true overlap section (D-E) and instead uses the original plan.
%   }
% %\vspace{0.2cm}
%   \label{fig:revise}
% \end{figure}


% Note that an overlap does not necessarily mean the path is reusable because an overlapped edge could have different robot-task reassignments after running Alg. \ref{alg:RP}. We classify a ``true" overlap of an edge $q_B^i,q_B^{i+1}\in \ccalP^{\text{min}}$, if the starting conditions of the edge and ending conditions of the edge are the same in the original path. Let $d'$ and $d''$ be such that $b_{q_B^{i-1},q_B^i}^{d'}$ and $b_{q_B^i,q_B^{i+1}}^{d''}$ correspond to the booleans with the lowest violation cost on their respective edges. 
% If $(q_B^i,q_B^{i+1})\in\ccalO$, then without loss of generality let $\ccalP_{\text{pre}}^{\tau}(j)=q_B^j$ and $\ccalP_{\text{pre}}^{\tau}(j+1)=q_B^{j+1}$, such that $(q_B^j,q_B^{j+1})=(q_B^i,q_B^{i+1})$, and let the corresponding states be $\Upsilon_{\text{pre}}(j)=[\bbp(k'), \bbs(k'), q_B(k')]$ and $\Upsilon_{\text{pre}}(j+1)=[\bbp(k''), \bbs(k''), q_B(k'')]$. If $L([\bbp(k'-1),\bbs(k'-1)])=b_{q_B^{i-1},q_B^i}^{d'}$ and $L([\bbp(k''-1),\bbs(k''-1)])=b_{q_B^i,q_B^{i+1}}^{d''}$, or in words, if the same set of robots are assigned to the predicates that satisfy the transition to $q_B^i$ and $q_B^{i+1}$ in $\ccalP^{\text{min}}$ and $\ccalP^{\tau}$, then $q_B^i,q_B^{i+1}\in \ccalP^{\text{min}}$ is considered a ``true" overlap. We collect all such edges in the ordered set $\ccalO^*$.


% % Thus only if the starting conditions of the edge and ending conditions of the edge are the same in the original path, only then can we say that there is a ``true" overlap in the edge.
% Furthermore, we call a state $q_B^i$ as the start of a true overlap if $(q_B^{i-1},q_B^i)\notin\ccalO^*\text{ and }(q_B^i,q_B^{i+1}) \in \ccalO^*$. Similarly a state $q_B^i$ is the end of a true overlap if $(q_B^{i-1},q_B^i)\in\ccalO^*\text{ and }(q_B^i,q_B^{i+1}) \notin \ccalO^*$. 
% If $|\ccalO^*|=0$, it means that there is no overlap with the original plan and to minimally violate the mission, we need to globally re-plan. If $|\ccalO^*|> 0$, we plan locally from the current state $\hat{\tau}_H(k)$ to the state $\hat{\tau}_H(k')$ in the original plan corresponding to the start of the first overlap in $\ccalO^*$.\footnote{\textcolor{blue}{Here we make an assumption that the path from  $\hat{\tau}_H(k)$ to  $\hat{\tau}_H(k')$ is feasible in the environment. If the planner cannot find a feasible path, then it must switch to global replanning. }\textcolor{red}{[What happens if a path connecting $\hat{\tau}_H(k)$ to  $\hat{\tau}_H(k')$ does not exist?]}} Similarly, we re-plan only from the end of each overlap, to either the beginning of the next overlap or until our planner reaches an accepting state in the automaton. See Fig. \ref{fig:revise}.   


% \textcolor{red}{[Here we need to say again that we can use any finite time planner and then the plans can be locally revised in the same way. I believe the local revision (ie which local part of the plan we revise) does not depend on the type of planner we pick. It might be a good idea to highlight this in the proof. I.e., we compute the minimum violation plan as long as we select any optimal planner.]}


% \textcolor{red}{[Following up on the above comment. I think here it would be quite helpful to just explain/define the parts of the plan we need to rewire/revise (as in the cdc paper). Once we define them, we can say that we can use any planner to compute these `local' paths. ]}

% \textcolor{red}{[IMPORTANT: Also, I believe the optimality result in proposition 3.4 holds only if we replan globally. Does local replanning preserves optimality?  ]}


% \textcolor{cyan}{Maybe we can mention here that optimality/completeness proofs for 0 penalty solutions are given in old paper and then skip those parts here}
\vspace{-0.1cm}
\subsection{Algorithm Analysis}
\vspace{-0.1cm}
Next, we discuss optimality properties of the proposed algorithm. The proofs are omitted due to space limitations.
\begin{prop}[Optimality of Alg. \ref{alg:bfs}]\label{prop:optiAlg1}
Consider a failed predicate $\pi\in\mathcal{AP}_F$ and Boolean formula $b_{q_B',q_B''}^d$ that contains $\pi$. %where $e=(q_B',q_B'')\in\ccalE$. 
Alg. \ref{alg:bfs} %is optimal,
%i.e., if there exist multiple feasible re-allocations it 
will find the re-allocation with the lowest penalty \textcolor{black}{as mentioned in Sec. \ref{sec:taskRealloc3}}. 
Among all re-allocations with the lowest penalty, Alg. \ref{alg:bfs} selects the one with the minimum number of re-assignments.
%\textcolor{red}{[I think the `or with the lowest penalty' is not very accurate. I think you mean with the lowest penalty and with the min number of re-assignments]}
%{Yes you are right... or is not needed}
\end{prop}
%\begin{proof} %completeness
%\textcolor{blue}{This result is due to completeness and optimality properties of the BFS algorithm. The graph $\ccalG$ captures all possible re-assignments by construction and as our proposed algorithm relies on BFS to search the whole graph, we can keep track of the closest node to the root with the lowest penalty. Thus, even if there are more than one nodes with same lowest value, we will return the node that will result in minimum number of re-assignments.}
%\end{proof}

\begin{proof} %completeness
If Alg. \ref{alg:bfs} cannot find an available robot (no penalty), it exhaustively searches all possible reassignment options in $\ccalG$ and then returns a path $p=p(0),p(1),\dots,p(P)$ over $\ccalG$, where $p(0)=a_{\text{root}}$ is the failed robot, and $p(P)=a^*$.
Since $a^*$ is always updated to point to the node with the lowest penalty ($F(g_{q_B',q_B''}^d(a^*))$ (line \ref{bfs:penaltyConditions}-\ref{bfs:reassign2ndBest}, Alg. \ref{alg:bfs})), we are guaranteed to find the re-allocation with the lowest penalty.

% \textcolor{blue}{This result is due to completeness and optimality properties of the BFS algorithm. 
% The algorithm searches for possible reassignments among the nodes in graph $\ccalG$ and stops searching either if it finds a robot that is available (no penalty), or has searched all possible reassignment options in $\ccalG$. Since we keep track of the node ($a^*$) with the lowest penalty ($F(g_{q_B',q_B''}^d(a^*))$ (line \ref{bfs:penaltyConditions}-\ref{bfs:reassign2ndBest}, Alg. \ref{alg:bfs})), when we search the complete graph $\ccalG$, we are guaranteed to find the re-allocation with the lowest penalty.}



Furthermore, Alg. \ref{alg:bfs} guarantees minimum number of re-assignments because we search with a breadth-first approach. \textcolor{blue}{If there is more than one node $a'$ with the lowest penalty, the first such node that Alg. \ref{alg:bfs} finds would be set as $a^*$ and this node will be closest to the root, i.e., the sum of the costs of edges, $w_{\ccalG}$, from $a_{root}$ to $a^*$ will be the lowest}. Then $a^*$ will not be set to any subsequent node with the same penalty that Alg. \ref{alg:bfs} finds, because we only update the node $a^*$ if its penalty $F(g_{q_B',q_B''}^d(a^*))$ is strictly lower than the other nodes (line \ref{bfs:penaltyConditions}-\ref{bfs:reassign2ndBest}, Alg. \ref{alg:bfs}). Thus, the path from $a_{root}$ to $a^*$ will result in the minimum number of re-assignments, \textcolor{blue}{as $a^*$ being the closest to the root, it can be reached with the minimum number of hops.}

% \textcolor{blue}{If there are more than one re-allocations with the lowest penalty, due to the breadth-first nature of search, and because we only update the lowest penalty node if it is strictly lower than the previous lowest node (line \ref{bfs:penaltyConditions}-\ref{bfs:reassign2ndBest}, Alg. \ref{alg:bfs}) we are guaranteed to find the node closest to the root and with the lowest penalty, even if there are more nodes in the tree with the same lowest penalty value. Thus we will return the node that will result in the minimum number of re-assignments.}

\end{proof}

% This result is due to completeness and optimality properties of the BFS algorithm. If the search on graph $\ccalG$ does not find a free robot (0 penalty), the algorithm searches the complete graph. Since we keep track of the node with the lowest penalty ($F(g_{q_B',q_B''}^d(a^*))$ (line \ref{bfs:penaltyConditions}-\ref{bfs:reassign2ndBest}, Alg. \ref{alg:bfs})), when we search the complete graph $\ccalG$, we are guaranteed to find the re-allocation with the lowest penalty.

% If there are more than one re-allocations with the lowest penalty, due to the breadth-first nature of search, and because we only update the lowest penalty node if it is strictly lower than the previous lowest node (line \ref{bfs:penaltyConditions}-\ref{bfs:reassign2ndBest}, Alg. \ref{alg:bfs}) we are guaranteed to find the node closest to the root and with the lowest penalty, even if there are more nodes in the tree with the same lowest penalty value. Thus we will return the node that will result in the minimum number of re-assignments.


% \textcolor{blue}{This result is due to completeness and optimality properties of the BFS algorithm. \textcolor{red}{[In the following text, you need to mention explicitly where optimality/completeness of BFS is used otherwise that sentence seems to be out of place. ]}The graph $\ccalG$ captures all possible re-assignments by construction thus enabling it \textcolor{red}{[I dont understand who enables whom here]} to find the task with the lowest penalty \textcolor{red}{[who finds the task with the lowest penalty? be specific. Is there a symbol for this penalty given a path? Introduce some math here, based on previously defined notations, so that it is easier to follow this text. Say here explicitly that this completes the first part of the proof (ie finding the reallocation with the lowest penalty)]}.
% %
% \textcolor{red}{[In the following text, you focus on the second part of the proof. Mention this explicitly and start a new paragraph.]}
% Furthermore, since our proposed algorithm relies on BFS to search the whole graph, we can keep track of the closest node to the root with the lowest penalty. Thus, even if there are more than one nodes with same lowest value \textcolor{red}{[you mean penalty?]}, we will return the node that will result in minimum number of re-assignments.}



\begin{prop}[Optimality of Re-planning]\label{prop:optiLVP}
Given the reassignments of predicates over the failed edges (Algorithm \ref{alg:RP}), our planner, as elaborated in Sec. \ref{sec:onlineReplan}, is guaranteed to find the path with the smallest violation score. 
% Consider one or more failures that occur during a mission, then the least violation path, as discussed in Sec. \ref{sec:onlineReplan}, is optimal with respect to the violation score. That is, if there exist multiple paths, then our approach will find the path with the lowest penalty possible.
\end{prop}

\begin{proof} %completeness
\textcolor{red}{[The proof needs to be updated. Currently it is written as if we replan globally. ]}
\textcolor{blue}{First, we prove optimality in case of global re-planning.}
To satisfy $b_{q_B',q_B''}^d$, proposition \ref{prop:optiAlg1} guarantees that the re-allocation of predicates in a failed edge ($q_B',q_B''$) will sacrifice (if needed) the predicate with the lowest penalty. Thus the violation score for the transition in the edge ($q_B',q_B''$) will be the minimum possible. This, combined with the optimality property of the sampling-based planner \cite{luo2021abstraction}, guarantees that the planner will exhaustively search all possible paths and thus will find a path $\tau$ such that the sequence of state transitions will result in the smallest violation score  $\mathbb{C}_\tau(t)$.

\textcolor{blue}{In case of local re-planning, as presented in Sec. \ref{sec:onlineReplan}, we first determine the sequence of states in the NBA that will yield the lowest violation score. We then implement our sampling-based planner by choosing start and end points between these states. Thus locally our planner is optimal due to optimality of our planner, and globally the planner is optimal by construction because we are building the plan that reaches the states in the NBA which will result in minimum violation.}

% \textcolor{blue}{This result is due to the optimality property of the sampling-based planner \cite{luo2021abstraction} and the guarantees of the lowest penalty re-allocation for each failed predicate (Proposition \ref{prop:optiAlg1}). Due to the optimality of the sampling-based planner, we are bound to search all possible combinations, thus guaranteeing that we will find the path that will accrue the smallest violation score.}
\end{proof}

%\begin{proof} %completeness
%\textcolor{blue}{This result is due to the optimality property of the sampling-based planner \cite{luo2021abstraction} and the guarantees of the lowest penalty re-allocation for each failed predicate (Proposition \ref{prop:optiLVP}). Due to the optimality of the planner, we are bound to search all possible combinations, thus guaranteeing th}at we will find the path that will accrue the smallest violation score. 
%\end{proof}

% A straightforward solution to revise the robot paths is to apply the sampling-based planner, discussed in Section \ref{sec:samplingAlg}, to build a new prefix-suffix plan from scratch.
% Nevertheless, re-planning from scratch for \textit{all} robots may be unnecessary given the `local' task re-allocations made by  Alg. \ref{alg:RP} while it may be impractical for large robot teams. Inspired by \cite{guo2013revising}, we propose an alternative re-planning approach that aims to locally revise the multi-robot plans. \textcolor{blue}{The idea is to use the sampling-based planner discussed in Section \ref{sec:samplingAlg}, to replan paths for the robots only in parts of the mission affected by the failure. These paths will rejoin the original paths wherever feasible and then the robots will continue to follow the original paths. Only in case no feasible local solution is found, the planner continues to sample till it finds a whole new plan. Details of this approach are beyond the scope of this paper and have been elaborated in \cite{kalluraya2023resilient_arxiv}. }


% Assume that the multi-robot system is at state $\tau_H(t)=[\bbp(t), \bbs(t), q_B(t)]$ when capability failures occurred and that Alg. \ref{alg:RP} has re-assigned tasks to robots. A straightforward solution to revise the robot paths is to apply the sampling-based planner, discussed in Section \ref{sec:samplingAlg}, to build a new prefix-suffix plan from scratch.
% %a new tree rooted at $\tau_H(t)$, to extract a . %If $\tau_H(t)$ belongs to the prefix part of the previous plan
% Nevertheless, re-planning from scratch for \textit{all} robots may be unnecessary given the `local' task re-allocations made by  Alg. \ref{alg:RP} while it may be impractical for large robot teams. Inspired by \cite{guo2013revising}, we propose an alternative re-planning approach that aims to locally revise the multi-robot plans; see also Fig. \ref{fig:revise}.



% First, we define the path $\hat{\tau}_H=\tau_H^{\text{pre}}\tau_H^{\text{suf}}=[\bbq(1),\dots,\bbq(T)],[\bbq(T+1),\dots, \bbq(T+K)]$ that concatenate the prefix and the suffix part of the current plan $\tau_H$ (without repeating  $\tau_H^{\text{suf}}$); see also Section \ref{sec:samplingAlg}.
% %
% Second, we compute the state $\hat{\tau}_H(k)$ for which it holds $\hat{\tau}_H(k)=\tau_H(t)$. \footnote{It is possible that $t>T+K$ since the state $\tau_H(t)$ may belong to the suffix part and $\tau_H$ contains an infinite repetition of the suffix part. In $\hat{\tau}_H(k)$, $k$ points to the $k$-th entry in $\hat{\tau}_H$ where   $\hat{\tau}_H(k)=\tau_H(t)$. } Third, we define the ordered set $\ccalT_{\text{pre}}$ collecting all states $\hat{\tau}_H(k')=[\bbp(k'), \bbs(k'), q_B(k')]$ in $\hat{\tau}_H$ that satisfy the following requirements: i) $k' \geq k$; ii) ($q_B(k')\neq q_B(k'+1)$ and $(q_B(k'),q_B(k'+1))\in\ccalE$) or ($q_B(k')\neq q_B(k'-1)$ and $(q_B(k'-1),q_B(k'))\in\ccalE$); and iii) $k'\leq T$. We denote by $\ccalT_{\text{pre}}(e)$ the $e$-th entry in $\ccalT_{\text{pre}}$. %We also include the current state $\hat{\tau}_H(k)$. 
% We similarly define $\ccalT_{\text{suf}}$ where the third requirement is replaced by $T+1\leq k'\leq T+K$. The entries in these sets appear in increasing order of the indices $k'$ (i.e., $\hat{\tau}_H(k)$ always appear first).  %; the same notation extends to $\ccalT_{\text{suf}}$.

\begin{figure}[t]
  \centering
    \includegraphics[width=0.75\linewidth]{figures/Tree3.png}
 \vspace{-0.2cm}
  \caption{Consider in Example \ref{ex:LTL} the case where skill $c_3$ of robot $2$ fails, i.e., the failed predicate is $\pi_2$. We present the BFS tree (Alg. \ref{alg:bfs}) built to fix $\pi_2$ for the NBA transition enabled by  $b_{q_B',q_B''}^{d}=\pi_1\wedge\pi_2\wedge\pi_3\wedge\neg\pi_4$. The set $\ccalA$ is defined as $\ccalA=\{4\}$ and the root of the tree is robot $2$. Robots $3$, and $4$ are adjacent to robot $2$ in $\ccalG$. Robot $4$ is not connected to robot $2$ because it does not satisfy $g_{q_B',q_B''}^d(2)\notin V^{d}_{q_B',q_B''}(4)=\{\pi_2,\pi_4,\pi_2\pi_4\}$. %where \textcolor{black}{$V^{d}_{q_B',q_B''}(a')$=$\{\pi_2$,$\pi_4$,$\pi_2$$\pi_4$\}, }.
  Robot $3$ is connected to robot $2$ and subsequently, robot $1$ is connected to robot $3$. Since we did not find a feasible path from $a_{\text{root}}$ to $\ccalA$, we pick the node $a^*=3$ which has the lowest predicate penalty, $F(g_{q_B',q_B''}^d(a^*))=15$. The blue dashed arrows show the re-assignment process along the computed path $p$, i.e., robot $3$ will take over the failed predicate and $\pi_3$ will be sacrificed resulting in an assignment cost/penalty of 15. In an alternate case if $\pi_1$ had the lowest penalty, then we would have seen robot $1$ replace robot $3$, and robot $3$ replace failed robot $2$, thus sacrificing $\pi_1$. %As robot $4\in\ccalA$, the path is returned from robot $4$ to the root, robot $2$.  
  }
\vspace{-0.05cm}
  \label{fig:bfs}
\end{figure}

% Assume that the failures occurred while the robots were executing the prefix part in $\tau_H$. %In what follows, we show how to compute a new prefix path using the sampling-based planner discussed in Section \ref{sec:samplingAlg}. %; the prefix part is constructed even if $\tau_H(t)$ belonged to the suffix part of $\tau_H$. 
% %The following process is repeated for each state $\ccalT_{\text{pre}}(e)$. 
% %
% To locally revise the prefix part, we build a tree, using the sampling-based planner discussed in Section \ref{sec:samplingAlg}, rooted at $\ccalT_{\text{pre}}(r)$, with $r=1$ and the goal region is defined as  
% $\ccalR_{\text{pre}}^{\text{rev}}=\{\bbq(T)\}\cup \{\ccalT_{\text{pre}}(s)\}_{s=r+1}^{|\ccalT_{\text{pre}}|}\cup \ccalR_{\text{pre}}$, i.e., the goal is to reach either any subsequent state in $\ccalT_{\text{pre}}$ along  the current path $\hat{\tau}_H$, or reach the final state $\bbq(T)$ associated with the current path $\hat{\tau}_H$, or reach any final state in the set $\ccalR_{\text{pre}}$ defined in Section \ref{sec:samplingAlg}. We terminate the sampling-based planner as soon as it returns the first feasible path. If that path connects the root to either $\ccalR_{\text{pre}}$ or $\hat{\tau}_H(T)$ then this path corresponds to the new/revised prefix part; %(i.e., the final state $\bbq(T)$) 
% construction of all other trees terminates. Otherwise, if it finds a path towards a state $\ccalT_{\text{pre}}(s)$, $s>r$, then we build a new tree, exactly as before, rooted at $\ccalT_{\text{pre}}(r)$ where $r$ is re-defined to be $r=s$. Then, the above process is repeated until a path towards either  $\ccalR_{\text{pre}}$ or $\hat{\tau}_H(T)$ is found. The revised prefix path is constructed by replacing the affected parts in $\tau_{H}^{\text{pre}}$, as captured by $\ccalT_{\text{pre}}$, with the revised ones; see also Fig. \ref{fig:revise}. 
% %Note that this process aims to revise only parts of the current prefix part. 
% If no prefix path can be found, global re-planning is triggered where a new-prefix suffix plan is designed from scratch as discussed in Section \ref{sec:samplingAlg}; the only difference is that the root for the prefix tree is based on the current robot position $\bbp(t)$ and current NBA state $q_B(t)$.
% %by building a new tree where the root consists of the current robot position $\bbp(t)$ and current NBA state $q_B(t)$ as discussed in Section \ref{sec:samplingAlg}.
% %
% Once the prefix part is designed, construction of the suffix part follows. If the revised prefix part ends in the state $\hat{\tau}_H(T)$, then the suffix part is constructed by following a similar logic as above. Otherwise, if it ends in a state $\ccalR_{\text{pre}}\setminus\hat{\tau}_H(T)$, the suffix part needs to be constructed from scratch by building a new tree rooted at the end state of the prefix path. 
% %
% If the failures occur when the robots are executing the suffix part in $\tau_H^{\text{suf}}$, then a similar approach is applied as before aiming to locally revise the suffix part i.e., the loop around $\hat{\tau}_H(T)$. If such a cyclic path around $\hat{\tau}_H(T)$ cannot be found, then a new prefix-suffix path is constructed from scratch as discussed earlier.

% \begin{figure}[t]
%   \centering
%     %\subfigure[$t=190$]{
%     %\label{fig:190}
%   %\includegraphics[width=0.485\linewidth]{figures/190.png}}
%       \subfigure[Current Path]{
%     \label{fig:curPath}
%   \includegraphics[width=0.9\linewidth]{figures/currentPrefix.png}}
%   \vspace{3pt}
%   \subfigure[Revised Path]{
%     \label{fig:revPath}
%   \includegraphics[width=0.9\linewidth]{figures/RevisedPrefix.png}}
% \vspace{-0.1cm}
%   \caption{Example of online revision of the prefix path. The disks capture states in $\hat{\tau}_H$.
%   Yellow states $\hat{\tau}_H(k')$ model states for which it holds $q_B(k')\neq q_B(k'-1)$. The red state corresponds to a final state around which a suffix part is designed. The part of $\hat{\tau}_H$ connecting  NBA states $q_B$ and $q_B'$, where $e=(q_B,q_B')\in\ccalE$ (see Alg. \ref{alg:RP}) is marked with a red color and a red `X' denoting that it requires revision. In this example, a path was found when a tree was built rooted at $\ccalT_{\text{pre}}(1)=\hat{\tau}_H(k)$. The computed path connects $\hat{\tau}_H(k)$ to $\ccalT_{\text{pre}}(2)$. The revised prefix part is constructed by replacing the red marked edges in $\hat{\tau}_H(k)$ with the previously computed path. 
%   }
% \vspace{0.2cm}
%   \label{fig:revise}
% \end{figure}
























%similar approach is applied to revise the suffix part if




%\textcolor{black}{
%The sampling-based planner builds a tree by sampling nodes in the form $\bbq(t)=[\bbp(t), \bbs(t), q_B(t)]$. Thus every node $\tau(t)$ in the resulting path $\tau$ corresponds to a node $\bbq(t)$ in the tree and a state  $q_B(t)$ in the NBA. The run $\rho_B=q_B^1\dotsq_B^k\dots$ corresponding to path $\tau$ is the sequence of NBA states that are visited when the robots follow $\tau$. Every time we visit a new state in the NBA while following $\tau$,  we add the node in the tree $\bbq(t)=[\bbp(t), \bbs(t), q_B(t)]$ at that time instant to a set $\mathbb{T}$. In other words $\mathbb{T}$ consists of nodes in the tree at which point we have transitioned to a new state $q_B$ in the NBA. }

%\textcolor{black}{
%At any time $t$, if one or more abilities of robots fail during the mission, Algorithm \ref{alg:RP} is executed. If the failure affects the mission in any way, the necessary robot reassignments will be reflected in the NBA. Thus at the end of the reassignment, if a transition is affected then it will result in different robots enabling the transition to the next state. We then compare for each node in $\mathbb{T}$ the corresponding state in the new NBA and determine the change in the transition needed. If the robots that satisfy the transition at the start state and end state are different, then we run the sampling-based planner from the positions in the start state to (i) the new satisfying positions for the replaced robots and (ii) the positions of other robots according to their original positions in $\mathbb{T}$. This way, we only replan where needed thus avoiding the need to replan for unaffected transitions. In case a transition in our previous path is unfeasible due to the failures, then we determine the next closest state in the path to which we could have a multi-hop transition through the NBA and then plan a path to that state.   }

%\textcolor{black}{
%Alternately, we could also run the sampling-based planner from the current robot positions (\bbp(t)) and the current state in the NBA ($q_{curr}$) to an accepting state so as to generate a new path $\tau=\tau(t)\dots\textcolor{black}{\tau(\infty)}$, that satisfy $\phi$.}
% \textcolor{green}{[IMPORTANT:} \textcolor{red}{I suggest here we explain how we can possibly leverage the previous tree (or the previous paths). This text implies that we do local task allocation but we do global re-planning which somehow makes us similar to [32] (in some sense the global replanning defeats the purpose of local task reallocation). For example, here: use the previous tree to initialize the planner as follows. For every node $\bbq(t)=[\bbp(t),\bbs(t),q_B(t)]$ in the previous tree, switch the abilities in $\bbs(t)$ from $c$ to $\varnothing$ if they have failed. Then, after you do this, recompute the NBA states associated with these tree nodes. Then use that tree to initialize your planner. OR: you could possibly use the planner to locally revise the paths. e.g., to fix the path connecting $q_B$ to $q_B'$ if this an affected transition. I thought that you were doing the latter. Possibly we could describe both or the one that is easier to explain]}

% % At any time $t$, if one or more abilities of robots fail during the mission, Algorithm \ref{alg:RP} is executed. If the failure affects the mission in any way, the necessary robot reassignments will be reflected in the NBA. We then run the sampling-based planner again from the current robot positions (\bbp(t)) and the current state in the NBA ($q_{curr}$)to generate a new path $\tau=\tau(t)\dots\textcolor{black}{\tau(\infty)}$, that satisfy $\phi$
% sequence $\bbu_{t:H}$ of control inputs $\bbu(\hat{t})$, for all $\hat{t}\in\set{t,\dots,H}$, that satisfy $\phi$. 
% \textcolor{black}{[self note: maybe mention here that planner picks $\hat\sigma$ such that $\hat\sigma$ has a valid assignment. For example, in Example \ref{ex:LTL_trans} if originally $\hat{\sigma}=\sigma_2$ and say robot $2$ and robot $3$ failed, then BFS will be able to find a solution only for $\sigma_1$, by replacing robot $2$ with robot $5$. In that case, when we recall the sampling-based planner, the planner picks $\hat{\sigma}=\sigma_1$.]}








% \vspace{-0.3cm}
% \subsection{Algorithm Analysis}\label{sec:analysis}
% \vspace{-0.1cm}

% In this section, we discuss correctness, completeness and optimality of the proposed algorithm. The proofs are omitted due to space limitations; they rely on completeness properties of the BFS and the sampling-based planner \cite{luo2021abstraction}. 

% \begin{prop}[Completeness/Optimality of Alg. \ref{alg:bfs}]\label{bfsCompl}
% Consider a failed predicate $\pi\in\mathcal{AP}_F$ and Boolean formula $b_{q_B',q_B''}^d$ that contains $\pi$. %where $e=(q_B',q_B'')\in\ccalE$. 
% Alg. \ref{alg:bfs} is complete, i.e., if there exists a re-allocation of all predicates (i.e., path $p$) that appear in $b_{q_B',q_B''}^d$ satisfying the constraints discussed in Section \ref{sec:taskRealloc2}, then Alg. \ref{alg:bfs} will find it. Algorithm \ref{alg:bfs} is also optimal,
% i.e., if there exist multiple feasible re-allocations it will find the re-allocation with the minimum number of re-assignments.
% %
% \end{prop}

% \begin{prop}[Completeness/Optimality of Alg. \ref{alg:RP}]\label{prop:ComplOpt}
% Consider a failed predicate $\pi\in\mathcal{AP}_F$ and a set of NBA edges $\ccalE$ depending on the $\pi$. If there exists feasible re-allocations(i.e., paths $p$) of all predicates for all Boolean formulas $b_{q_B',q_B''}^d$ for a given edge $e\in\ccalE$ and for all $e\in\ccalE$, then Alg. \ref{alg:RP} will find them. It will also find the solution with the minimum number of re-assignments across all sub-formulas and edges.
% \end{prop}


% \begin{prop}[Soundness/Completeness of Replanning]
% Consider a re-allocation of predicates to robots by Alg. \ref{alg:RP}. If the re-planning algorithm (Section \ref{sec:onlineReplan}) returns a new prefix-suffix plan, then this plan satisfies $\phi$. Also, if there exists a feasible prefix-suffix plan satisfying the revised formula, then the re-planning algorithm will find it.
% \end{prop}

%\begin{rem}[Limitations]\label{rem:limitations}
%\textcolor{cyan}{do we need this?}
%The constraints defined in Section \ref{sec:taskRealloc2} cannot ensure feasibility of the revised LTL formula. In fact, satisfying these constraints is necessary, but not sufficient, to ensure the existence of robot paths that can result in accepting NBA runs. %Additional  constraints can be introduced in the task re-allocation process, modeling necessary conditions to ensure that a transition is physically realizable; see e.g., Def. 3.4 in \cite{kantaros2020reactive}.
%\end{rem}






















% \subsection{BFS algorithm}\label{bfs_explanation}
% This algorithm builds a tree such that each node in the tree represents a robot and the children of that node are those robots that can do the task of the parent robot. We start the tree with the root node representing the failed robot. We build the tree in a breadth-first manner, and if there exists a solution, the tree will stop building when it finds a robot that is currently unassigned. While this robot may not necessarily directly replace the failed robot, the path in the tree from this robot to the root is the sequence of reassignments that need to be done to fix the failed task.

% The input for the algorithm is the failed task $\pi_{\ccalT_c}^p$, failed robot $rob_j$, sets $\mathcal{U}$ and $\mathcal{A}$, and the atomic predicates that need to be satisfied ($\sigma_b$) for the NBA transition to happen. The first step is to add the failed robot and failed task to the root node called $root$ and add the $root$ to a queue $\mathcal{Q}$ (lines \ref{bfs:root}-\ref{bfs:queue}, Alg. \ref{alg:bfs}). We initialize an empty set $\mathcal{V}$ which will keep track of all the nodes that we visit (line \ref{bfs:visited}, Alg. \ref{alg:bfs}). $\mathcal{V}$ helps us avoid expanding the tree for a particular robot more than once. Intuitively a robot cannot be in the tree more than once as that could lead to a solution where that robot might need to do two tasks at the same time which is infeasible. The only robot allowed to appear in the tree a second time is the robot with the failed ability ($root$). This can happen if that robot has another active ability and thus can take over another task giving up on the current failed task.

% We then keep building the tree until $\mathcal{Q}$ is not empty. To do so the node $parent$ is set to the first node in $\mathcal{Q}$ and that node is removed from $\mathcal{Q}$ (line \ref{bfs:pop}, Alg. \ref{alg:bfs}). If we haven't previously visited this node and if this is not the root node, we add $parent$ to $\mathcal{V}$ (line \ref{bfs:add2visited}, Alg. \ref{alg:bfs}). If there are unassigned robots that can accomplish the task of the robot in $parent$, we choose one of the unassigned robots $rob_g$ using the function PICK (line \ref{bfs:pick}, Alg. \ref{alg:bfs}). This function can choose an unassigned robot based on some optimization criteria. In our implementation, for simplicity, we pick the first robot in the set. We then add the $rob_g$ and the $parent$ to a new node called $answer$ and return $answer$ and a flag set to True as the solution of the algorithm (lines \ref{bfs:answer1}-\ref{bfs:return1}, Alg. \ref{alg:bfs}). If there are no unassigned robots, then for every robot $rob_g$ in $\mathcal{A}$ we first check if this $rob_g$ is the same as the $root$ robot or in other words the robot with the failed task. If that is the case we add $rob_g$ and the $parent$ to a new node called $answer$ and return  $answer$  and a flag set to True (lines \ref{bfs:answer1}-\ref{bfs:return1}, Alg. \ref{alg:bfs}) (we call this type of replacement ``looped-reassignment" and we will see an example of this in Section \ref{sec:looped}). Otherwise, if we have not visited $rob_g$ before, we create a child node with $rob_g$, the task $rob_g$ is currently assigned to (using function TASK($rob_g$,$\sigma_b$) that returns the task  $rob_g$ needs to do to satisfy $\sigma_b$), and $parent$, and add this node to $\mathcal{Q}$. (lines \ref{bfs:child}-\ref{bfs:add2q}, Alg. \ref{alg:bfs}). If we empty $\mathcal{Q}$ without finding a solution, then we return an empty node and  flag that is set to false indicating that the algorithm could not find any feasible solution.  

% When we build this tree, we search all possible robots that can replace each task. Thus if there exists a solution, that is if there exists a particular order of robot-task re-assignments, we are guaranteed to find it. Furthermore, since the tree is built in a breadth-first manner, the first solution that we find is guaranteed to have the least number of robot-task re-assignments.

% \begin{algorithm}[t]
% %\footnotesize
% \caption{Breadth First Search}
% \LinesNumbered
% \label{alg:bfs}
% \KwIn{ (i) Failed robot and task: $\pi_{\ccalT_c}^p(rob_j, \zeta_c, l_i)$, (ii)$\mathcal{U}$, (iii)$\mathcal{A}$, (iv) $\sigma_b$}
% \KwOut{answer node}
% $root$ = [$rob_j$, $\pi_{\ccalT_c}^p$,parent=None]\;\label{bfs:root}
% $\mathcal{Q}$ = [$root$]\;\label{bfs:queue}
% $\mathcal{V}=\emptyset$\;\label{bfs:visited}
% $first\_time$ = True\;\label{bfs:first_time}
% \While{$\sim$empty($\mathcal{Q}$)}{
%     $parent\leftarrow$ POP($\mathcal{Q}$)\;\label{bfs:pop}
%     \If{$parent\notin \mathcal{V}$}{
%         \If{$\sim first\_time$}{
%             $\mathcal{V}\leftarrow parent$\;\label{bfs:add2visited}
%         }
%         $first\_time$ = False\;
%         \If{$\sim$empty($\mathcal{U}[parent.task]$}{
%             $rob_g$ = PICK($\mathcal{U}[parent.task]$)\;\label{bfs:pick}
%             $answer$ = [$rob_g$, parent=$parent$]\;\label{bfs:answer1}
%             return ($answer$, True)\;\label{bfs:return1}
%         }
%         \For{$rob_g \in \mathcal{A}[parent.task]$}{
%             \If{$rob_g$ = $root.robot$}{
%                 $answer$ = [$root.robot$, parent=$parent$]\;\label{bfs:answer2}
%                 return ($answer$, True)\;\label{bfs:return2}
%             }
%             \ElseIf{$rob_g\notin \mathcal{V}$}{
%                 \small$child$ = [$rob_g$,TASK($rob_g,\sigma_b$),parent=$parent$]\;\label{bfs:child}
%                 $\mathcal{Q}\leftarrow child$\;\label{bfs:add2q}
%             }
%         }
%     }
% }
% return ($\emptyset$, False)
% \end{algorithm}





%\textcolor{red}{[You are still missing a theoretical result here. As we discussed last time, you need to have a proposition here discussing that if a single failure happens then you can find a re-assignment that satisfies all the imposed constraints. Provide a short proof on this. then, discuss what happens if you have multiple failures. Not as a theorem (if you don't have a proof for this) but at least a discussion is needed. Then, provide at least a discussion on under what conditions there exist feasible paths for the new assignment.]}
